On the use of Sulphur as a tracer for abundances in galaxies

We present a methodology for the use of sulphur as global metallicity tracer in galaxies, allowing performing a complete abundance analysis using only the red-to-near infrared spectral region. We have applied it to a compilation of high-quality data split into two samples: HII regions (DHR) in spiral and irregular galaxies, and dwarf galaxies dominated by a strong starburst (HIIGal). Sulphur abundances have been derived by direct methods under the assumption of an ionisation structure composed of two zones: an intermediate one where S{++} is originated and a low ionisation one where S{+} is formed. Ionisation correction factors (ICF) have been calculated from the Ar{2+}/Ar{3+} ratio and are shown to correlate with the hardness of the radiation field. Only about 10% of the objects show S{3+} contributions to the total abundance larger than 30%. A good correlation exists between sulphur abundance and ionising temperature with low metallicity objects being ionised by hotter stars. No correlation is found between ionisation parameter and total S/H abundance. Most of the HIIGal objects show S/O ratios below the solar value and a trend for increasing S/O ratios with increasing sulphur abundances while DHR objects show S/O ratios larger than solar and a tendency for lower S/O ratios for higher metallicities. Finally, we present a calibration of the sulphur abundance through the S{23} parameter that remains single valued up to sulphur abundances well beyond the solar value. S{23} is independent of the ionisation parameter and only weakly dependent on ionising temperature.

==> Tables/Tabla_DHR_lines.tex <==
\begin{table*}
\centering
\caption{Reddening corrected emission line intensities, relative to H$\beta$ = 100 for objects in the DHR sub-sample. }
\label{linesDHR}
\begin{tabular}{cccccccc}
\cline{1-8}
  & Line & [OII] & [OIII] & [OIII] & [SIII] & [SII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 &4959, 5007 & 6312  & 6717, 6731 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{6}{c}{I($\lambda $)$^{a}$} \\ \hline


1 & N604D (M33) & 161.4 $\pm$ 2.0 & -& 340.4 $\pm$ 10.0 & 0.9 $\pm$ 0.4 & 23.4 $\pm$ 1.5 & 123.5 $\pm$ 2.5\\ 
2 & N604E & 257.0 $\pm$ 2.0 & -& 204.9 $\pm$ 3.3 & 1.1 $\pm$ 0.4 & 51.3 $\pm$ 2.9 & 127.5 $\pm$ 6.9\\ 
3 & NGC595 (M33) & 213.8 $\pm$ 10.01 & -& 189.6 $\pm$ 6.0 & 0.8 $\pm$ 0.15 & 24.9 $\pm$ 1.0 & 97.2 $\pm$ 1.6\\ 
4 & NGC3310-A & 259.0 $\pm$ 4.0 & 1.8 $\pm$ 0.5 & 305.0 $\pm$ 1.6 & 1.1 $\pm$ 0.3 & 49.0 $\pm$ 1.2 & 43.0 $\pm$ 0.7\\ 
5 & NGC3310-C & 316.0 $\pm$ 10.0 & 2.5 $\pm$ 0.7 & 326.0 $\pm$ 2.4 & 1.4 $\pm$ 0.2 & 55.0 $\pm$ 0.4 & 81.0 $\pm$ 0.9\\ 
6 & NGC3310-E & 313.0 $\pm$ 4.5 & -& 271.0 $\pm$ 1.5 & 1.4 $\pm$ 0.7 & 62.0 $\pm$ 2.7 & 76.0 $\pm$ 2.4\\ 
7 & NGC3310-L & 469.0 $\pm$ 19.0 & -& 225.0 $\pm$ 8.0 & 1.1 $\pm$ 0.5 & 85.0 $\pm$ 2.0 & 67.0 $\pm$ 3.5\\ 
8 & N2363A2 & 43.2 $\pm$ 0.5 & 16.5 $\pm$ 0.4 & 994.0 $\pm$ 8.0 & 1.0 $\pm$ 0.1 & 6.7 $\pm$ 0.2 & 31.3 $\pm$ 1.2\\ 
9 & N2363-B1 & 150.0 $\pm$ 10.0 & 11.0 $\pm$ 0.2 & 710.0 $\pm$ 40.0 & 1.7 $\pm$ 0.6 & 22.0 $\pm$ 2.0 & 40.0 $\pm$ 7.0\\ 
10 & N2363-B2 & 89.0 $\pm$ 1.4 & 12.5 $\pm$ 0.2 & 840.0 $\pm$ 8.0 & 1.7 $\pm$ 0.1 & 12.6 $\pm$ 0.2 & 37.8 $\pm$ 1.4\\ 
11 & N2363-B3 & 60.0 $\pm$ 3.0 & 13.0 $\pm$ 0.5 & 905.0 $\pm$ 14.0 & 1.5 $\pm$ 0.1 & 9.2 $\pm$ 0.4 & 34.4 $\pm$ 6.9\\ 
12 & N2363-B4 & 42.0 $\pm$ 0.6 & 14.0 $\pm$ 2.0 & 920.0 $\pm$ 50.0 & 1.6 $\pm$ 0.3 & 7.8 $\pm$ 0.7 & 39.0 $\pm$ 12.0\\ 
13 & H681 & 244.2 $\pm$ 15.8 & 5.0 $\pm$ 0.5 & 417.8 $\pm$ 18.5 & 1.7 $\pm$ 0.1 & 26.9 $\pm$ 3.9 & 36.4 $\pm$ 5.4\\ 
14 & N7714-A-110 & 245.0 $\pm$ 2.0 & 1.7 $\pm$ 0.2 & 179.4 $\pm$ 1.2 & 0.8 $\pm$ 0.1 & 74.4 $\pm$ 0.7 & 79.8 $\pm$ 1.4\\ 
15 & N7714-B-110 & 242.0 $\pm$ 4.0 & 3.1 $\pm$ 0.5 & 476.0 $\pm$ 3.0 & 1.4 $\pm$ 0.1 & 53.0 $\pm$ 1.1 & 49.2 $\pm$ 2.5\\ 
16 & N7714-C-216 & 280.0 $\pm$ 30.0 & 1.7 $\pm$ 0.4 & 343.0 $\pm$ 4.0 & 1.0 $\pm$ 0.1 & 57.0 $\pm$ 7.0 & 42.0 $\pm$ 1.0\\ 
17 & VS35 (2403) & 246.0 $\pm$ 38.0 & -& 184.0 $\pm$ 19.0 & 1.1 $\pm$ 0.3 & 47.8 $\pm$ 9.7 & 79.0 $\pm$ 6.6\\ 
18 & VS24 & 242.0 $\pm$ 22.0 & -& 176.0 $\pm$ 18.0 & 0.4 $\pm$ 0.1 & 34.7 $\pm$ 1.1 & 90.7 $\pm$ 8.8\\ 
19 & VS38 & 192.0 $\pm$ 24.0 & -& 134.0 $\pm$ 14.0 & 0.7 $\pm$ 0.1 & 30.2 $\pm$ 1.0 & 84.4 $\pm$ 4.6\\ 
20 & VS44 & 280.0 $\pm$ 110.0 & -& 199.0 $\pm$ 20.0 & 1.1 $\pm$ 0.1 & 39.2 $\pm$ 1.3 & 71.3 $\pm$ 3.9\\ 
21 & VS51 & 228.0 $\pm$ 80.0 & -& 237.0 $\pm$ 23.0 & 1.0 $\pm$ 0.2 & 34.0 $\pm$ 2.0 & 80.0 $\pm$ 13.0\\ 
22 & VS3 & 226.0 $\pm$ 55.0 & 1.0 $\pm$ 0.2 & 214.0 $\pm$ 22.0 & 1.2 $\pm$ 0.1 & 32.5 $\pm$ 1.1 & 77.7 $\pm$ 5.3\\ 
23 & VS49 & 219.0 $\pm$ 24.0 & 2.9 $\pm$ 0.4 & 325.0 $\pm$ 33.0 & 1.2 $\pm$ 0.2 & 40.7 $\pm$ 1.4 & 74.2 $\pm$ 11.5\\ 
24 & VS48 & 252.0 $\pm$ 25.0 & 3.8 $\pm$ 0.6 & 423.0 $\pm$ 42.0 & 1.6 $\pm$ 0.1 & 36.8 $\pm$ 1.4 & 82.1 $\pm$ 22.5\\ 
25 & N4258-74C    & 210.0 $\pm$ 4.0 & -& 151.8 $\pm$ 1.5 & 0.9 $\pm$ 0.1 & 44.8 $\pm$ 1.3 & 92.6 $\pm$ 2.0\\ 
26 & N4258-69C    & 228.0 $\pm$ 9.0 & -& 122.0 $\pm$ 4.0 & 0.7 $\pm$ 0.1 & 61.6 $\pm$ 1.5 & 65.4 $\pm$ 4.0\\ 
27 & N1232CDT3  & 318.0 $\pm$ 15.0 & -& 112.6 $\pm$ 1.9 & 0.7 $\pm$ 0.1 & 60.5 $\pm$ 1.9 & 84.3 $\pm$ 4.0\\ 
28 & N1232CDT4 & 253.0 $\pm$ 12.0 & -& 155.5 $\pm$ 1.1 & 0.7 $\pm$ 0.1 & 54.0 $\pm$ 3.5 & 91.4 $\pm$ 3.0\\ 
29 & N1232-CDT1 & 149.0 $\pm$ 7.0 & -& 30.6 $\pm$ 0.6 & 0.2 $\pm$ 0.1 & 63.1 $\pm$ 1.4 & 65.2 $\pm$ 4.7\\ 
30 & N628H13 & 296.0 $\pm$ 11.0 & 1.0 $\pm$ 0.2 & 208.3 $\pm$ 1.5 & 1.2 $\pm$ 0.1 & 35.5 $\pm$ 0.9 & 54.2 $\pm$ 2.5\\ 
31 & H1013 & 188.0 $\pm$ 10.0 & -& 137.3 $\pm$ 0.7 & 0.8 $\pm$ 0.1 & 28.8 $\pm$ 1.5 & 131.6 $\pm$ 7.0\\ 
32 & H1105 & 185.0 $\pm$ 10.0 & 1.4 $\pm$ 0.1 & 421.3 $\pm$ 22.7 & 1.3 $\pm$ 0.1 & 24.1 $\pm$ 1.3 & 126.1 $\pm$ 6.1\\ 
33 & H1159 & 198.0 $\pm$ 10.0 & 1.9 $\pm$ 0.4 & 422.7 $\pm$ 22.7 & 1.6 $\pm$ 0.2 & 29.8 $\pm$ 1.6 & 97.0 $\pm$ 5.4\\ 
34 & H1170 & 308.0 $\pm$ 16.0 & 1.6 $\pm$ 0.2 & 268.0 $\pm$ 14.7 & 1.7 $\pm$ 0.2 & 56.7 $\pm$ 3.0 & 170.0 $\pm$ 9.3\\ 
35 & H1176 & 160.0 $\pm$ 8.0 & 2.4 $\pm$ 0.3 & 492.0 $\pm$ 26.7 & 1.5 $\pm$ 0.1 & 23.0 $\pm$ 1.2 & 113.5 $\pm$ 6.1\\ 
36 & H1216 & 151.0 $\pm$ 8.0 & 4.7 $\pm$ 0.3 & 630.7 $\pm$ 33.3 & 1.6 $\pm$ 0.1 & 18.9 $\pm$ 1.0 & 83.0 $\pm$ 4.6\\ 
37 & H128 & 145.0 $\pm$ 8.0 & 1.7 $\pm$ 0.2 & 521.3 $\pm$ 37.3 & 1.3 $\pm$ 0.1 & 23.3 $\pm$ 1.2 & 104.4 $\pm$ 5.7\\ 
38 & H143 & 219.0 $\pm$ 12.0 & 2.3 $\pm$ 0.4 & 378.7 $\pm$ 20.0 & 1.4 $\pm$ 0.2 & 40.2 $\pm$ 2.1 & 93.8 $\pm$ 5.2\\ 
39 & H149 & 212.0 $\pm$ 11.0 & 1.8 $\pm$ 0.4 & 424.0 $\pm$ 22.7 & 1.4 $\pm$ 0.1 & 37.2 $\pm$ 1.9 & 95.4 $\pm$ 5.0\\ 
40 & H409 & 218.0 $\pm$ 12.0 & 2.3 $\pm$ 0.2 & 493.3 $\pm$ 29.3 & 0.6 $\pm$ 0.1 & 31.2 $\pm$ 2.2 & 90.4 $\pm$ 4.9\\ 
41 & H67 & 244.0 $\pm$ 13.0 & 3.5 $\pm$ 0.2 & 456.0 $\pm$ 24.0 & 1.7 $\pm$ 0.1 & 26.3 $\pm$ 1.9 & 92.1 $\pm$ 5.7\\ 
42 & N5471A & 106.0 $\pm$ 6.0 & 9.5 $\pm$ 0.5 & 858.7 $\pm$ 45.3 & 1.8 $\pm$ 0.4 & 15.8 $\pm$ 0.9 & 61.4 $\pm$ 3.4\\ 
43 & N5471B & 213.0 $\pm$ 11.0 & 6.6 $\pm$ 0.4 & 526.7 $\pm$ 28.0 & 1.6 $\pm$ 0.1 & 54.7 $\pm$ 2.8 & 50.9 $\pm$ 3.1\\ 
44 & N5471C & 174.0 $\pm$ 9.0 & 5.4 $\pm$ 0.3 & 554.7 $\pm$ 29.3 & 1.3 $\pm$ 0.1 & 114.1 $\pm$ 1.2 & 65.9 $\pm$ 3.7\\ 
45 & N5471D & 137.0 $\pm$ 7.0 & 8.0 $\pm$ 0.4 & 770.7 $\pm$ 41.3 & 1.4 $\pm$ 0.1 & 20.6 $\pm$ 1.1 & 75.7 $\pm$ 4.3\\ 
46 & LMC-30Dor & 123.47 $\pm$ 1.48 & 3.209 $\pm$ 0.048135 & 678.8 $\pm$ 6.79 & 1.805 $\pm$ 0.044 & 13.68 $\pm$ 0.19 & 93.76 $\pm$ 1.31\\ 
47 & M51CCM10 & 126.0 $\pm$ 9.0 & -& 16.5 $\pm$ 1.0 & 0.3 $\pm$ 0.03 & 46.0 $\pm$ 3.0 & 58.5 $\pm$ 10.3\\ 
48 & M51CCM53 & 129.0 $\pm$ 9.0 & -& 45.1 $\pm$ 2.7 & 0.31 $\pm$ 0.06 & 41.0 $\pm$ 3.0 & 61.9 $\pm$ 13.7\\ 
49 & M51CCM54 & 115.0 $\pm$ 8.0 & -& 55.7 $\pm$ 3.3 & 0.44 $\pm$ 0.06 & 63.0 $\pm$ 5.0 & 58.5 $\pm$ 10.3\\ 
50 & M51CCM55 & 78.0 $\pm$ 5.0 & -& 25.7 $\pm$ 1.5 & 0.31 $\pm$ 0.03 & 41.0 $\pm$ 3.0 & 72.2 $\pm$ 13.7\\ 
51 & M51CCM57 & 114.0 $\pm$ 8.0 & -& 21.6 $\pm$ 1.2 & 0.31 $\pm$ 0.07 & 45.0 $\pm$ 3.0 & 48.2 $\pm$ 10.3\\ 
52 & M51CCM72 & 63.0 $\pm$ 6.0 & -& 9.0 $\pm$ 0.5 & 0.16 $\pm$ 0.03 & 46.0 $\pm$ 4.0 & 48.2 $\pm$ 10.3\\ 
53 & MWG-Orion   & 82.674 $\pm$ 3.30696 & 1.301 $\pm$ 0.02602 & 512.006 $\pm$ 3.584042 & 1.853 $\pm$ 0.07412 & 5.456 $\pm$ 0.32736 & 102.766 $\pm$ 15.4149\\ 
54 & MWG-N3576 & 132.635 $\pm$ 5.3054 & 1.279 $\pm$ 0.02558 & 474.358 $\pm$ 3.320506 & 1.544 $\pm$ 0.0757 & 13.132 $\pm$ 0.78792 & 113.068 $\pm$ 12.43748\\ 
55 & N1232-4         & 207.0 $\pm$ 17.0 & -& 536.0 $\pm$ 32.0 & 1.47 $\pm$ 0.19 & 23.0 $\pm$ 2.0 & 65.4 $\pm$ 14.0\\ 
56 & N1232-5        & 253.0 $\pm$ 16.0 & -& 134.0 $\pm$ 8.0 & 0.66 $\pm$ 0.11 & 59.0 $\pm$ 4.0 & 86.0 $\pm$ 17.0\\ 
57 & N1232-7        & 163.0 $\pm$ 10.0 & -& 29.0 $\pm$ 1.0 & 0.36 $\pm$ 0.15 & 62.0 $\pm$ 5.0 & 58.5 $\pm$ 10.0\\ 
58 & N1232-14       & 305.0 $\pm$ 19.0 & -& 107.0 $\pm$ 7.0 & 0.8 $\pm$ 0.12 & 78.0 $\pm$ 5.0 & 65.4 $\pm$ 14.0\\ 
59 & N1365-5        & 169.0 $\pm$ 11.0 & -& 34.0 $\pm$ 2.0 & 0.32 $\pm$ 0.11 & 66.0 $\pm$ 5.0 & 55.0 $\pm$ 10.0\\ 
60 & N1365-8        & 172.0 $\pm$ 11.0 & -& 80.0 $\pm$ 5.0 & 0.63 $\pm$ 0.13 & 55.0 $\pm$ 4.0 & 65.4 $\pm$ 14.0\\ 

 
\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{cccccccc}
\cline{1-8}
  & Line & [OII] & [OIII] & [OIII] & [SIII] & [SII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 &4959, 5007 & 6312  & 6717, 6731 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{6}{c}{I($\lambda $)$^{a}$} \\ \hline

 
 
61 & N1365-14      & 209.0 $\pm$ 13.0 & -& 52.0 $\pm$ 3.0 & 0.38 $\pm$ 0.16 & 61.0 $\pm$ 5.0 & 51.6 $\pm$ 10.0\\ 
62 & N1365-15      & 221.0 $\pm$ 18.0 & -& 100.0 $\pm$ 6.0 & 1.0 $\pm$ 0.12 & 56.0 $\pm$ 5.0 & 113.5 $\pm$ 24.0\\ 
63 & N1365-16       & 244.0 $\pm$ 16.0 & -& 127.0 $\pm$ 8.0 & 0.78 $\pm$ 0.28 & 43.0 $\pm$ 3.0 & 65.4 $\pm$ 14.0\\ 
64 & N2997-4        & 383.0 $\pm$ 31.0 & -& 204.0 $\pm$ 12.0 & 0.96 $\pm$ 0.18 & 63.0 $\pm$ 7.0 & 89.0 $\pm$ 17.0\\ 
65 & N2997-5        & 213.0 $\pm$ 17.0 & -& 110.0 $\pm$ 7.0 & 0.54 $\pm$ 0.11 & 65.0 $\pm$ 7.0 & 86.0 $\pm$ 17.0\\ 
66 & N2997-6        & 215.0 $\pm$ 13.0 & -& 109.0 $\pm$ 7.0 & 0.96 $\pm$ 0.12 & 36.0 $\pm$ 7.0 & 103.0 $\pm$ 21.0\\ 
67 & N2997-7        & 203.0 $\pm$ 16.0 & -& 69.0 $\pm$ 4.0 & 0.61 $\pm$ 0.13 & 56.0 $\pm$ 5.0 & 79.0 $\pm$ 17.0\\ 
68 & N2997-13      & 118.0 $\pm$ 7.0 & -& 25.0 $\pm$ 2.0 & 0.28 $\pm$ 0.09 & 51.0 $\pm$ 4.0 & 89.4 $\pm$ 17.0\\ 
69 & N5236-3        & 208.0 $\pm$ 17.0 & -& 157.0 $\pm$ 9.0 & 0.72 $\pm$ 0.13 & 43.0 $\pm$ 4.0 & 89.4 $\pm$ 17.0\\ 
70 & N5236-6        & 123.0 $\pm$ 8.0 & -& 28.0 $\pm$ 2.0 & 0.5 $\pm$ 0.17 & 49.0 $\pm$ 4.0 & 82.6 $\pm$ 17.0\\ 
71 & N5236-11       & 47.0 $\pm$ 3.0 & -& 12.0 $\pm$ 2.0 & 0.23 $\pm$ 0.05 & 59.0 $\pm$ 4.0 & 141.0 $\pm$ 27.0\\ 
72 & N5236-16      & 144.0 $\pm$ 9.0 & -& 31.0 $\pm$ 2.0 & 0.35 $\pm$ 0.1 & 51.0 $\pm$ 4.0 & 127.0 $\pm$ 24.0\\ 
73 & MWG-S311    & 359.29 $\pm$ 14.3716 & 0.562 $\pm$ 0.02248 & 169.026 $\pm$ 5.07078 & 1.348 $\pm$ 0.05392 & 50.186 $\pm$ 2.00744 & 84.604 $\pm$ 4.2302\\ 
74 & MWG-M16    & 276.56 $\pm$ 11.0624 & 0.192 $\pm$ 0.015 & 110.093 $\pm$ 3.30279 & 1.024 $\pm$ 0.04096 & 52.372 $\pm$ 2.09488 & 83.676 $\pm$ 6.69408\\ 
75 & MWG-N3603 & 65.35 $\pm$ 3.2675 & 2.483 $\pm$ 0.12415 & 713.581 $\pm$ 21.40743 & 1.849 $\pm$ 0.09245 & 5.259 $\pm$ 0.26295 & 124.421 $\pm$ 11.19789\\ 
76 & MWG-M20     & 319.911 $\pm$ 9.59733 & 0.148 $\pm$ 0.0192 & 77.937 $\pm$ 2.33811 & 0.941 $\pm$ 0.03764 & 45.421 $\pm$ 1.81684 & 80.244 $\pm$ 4.81464\\ 
77 & M101-H493   & 84.0 $\pm$ 4.0 & -& 11.0 $\pm$ 1.0 & 0.27 $\pm$ 0.07 & 51.4 $\pm$ 3.0 & 34.4 $\pm$ 7.0\\ 
78 & M101-H1013 & 221.0 $\pm$ 11.0 & 0.24 $\pm$ 0.03 & 135.0 $\pm$ 5.0 & 0.77 $\pm$ 0.05 & 29.8 $\pm$ 1.7 & 83.0 $\pm$ 17.0\\ 
79 & MWG-M8       & 209.487 $\pm$ 16.75896 & 0.286 $\pm$ 0.01144 & 128.998 $\pm$ 3.86994 & 1.344 $\pm$ 0.04032 & 21.191 $\pm$ 0.63573 & 89.579 $\pm$ 3.58316\\ 
80 & MWG-M17     & 91.792 $\pm$ 3.67168 & 0.953 $\pm$ 0.04765 & 449.449 $\pm$ 13.48347 & 1.203 $\pm$ 0.04812 & 8.902 $\pm$ 0.4451 & 109.818 $\pm$ 7.68726\\ 
81 & NGC300-2 & 166.7 $\pm$ 12.0 & 5.59 $\pm$ 0.35 & 670.32 $\pm$ 38.57 & 1.85 $\pm$ 0.13 & 17.4 $\pm$ 0.8 & 67.424 $\pm$ 5.848\\ 
82 & NGC300-4 & 286.0 $\pm$ 20.0 & 2.14 $\pm$ 0.17 & 336.49 $\pm$ 19.95 & 1.73 $\pm$ 0.16 & 33.2 $\pm$ 1.6 & 71.208 $\pm$ 4.816\\ 
83 & NGC300-5 & 296.0 $\pm$ 21.0 & 1.1 $\pm$ 0.15 & 300.58 $\pm$ 17.29 & 1.34 $\pm$ 0.16 & 52.7 $\pm$ 2.5 & 90.816 $\pm$ 5.848\\ 
84 & NGC300-6 & 225.0 $\pm$ 20.0 & 1.16 $\pm$ 0.14 & 327.18 $\pm$ 18.62 & 1.38 $\pm$ 0.16 & 38.6 $\pm$ 1.8 & 69.832 $\pm$ 4.816\\ 
85 & NGC300-8 & 307.0 $\pm$ 22.0 & 0.77 $\pm$ 0.1 & 191.52 $\pm$ 10.64 & 1.32 $\pm$ 0.12 & 44.2 $\pm$ 2.1 & 70.864 $\pm$ 4.816\\ 
86 & NGC300-9 & 172.0 $\pm$ 12.0 & 0.89 $\pm$ 0.08 & 312.55 $\pm$ 18.62 & 1.09 $\pm$ 0.08 & 33.1 $\pm$ 1.5 & 93.568 $\pm$ 6.192\\ 
87 & NGC300-10 & 180.0 $\pm$ 13.0 & 0.91 $\pm$ 0.07 & 313.88 $\pm$ 18.62 & 1.11 $\pm$ 0.08 & 16.3 $\pm$ 0.8 & 91.16 $\pm$ 5.848\\ 
88 & NGC300-11 & 258.0 $\pm$ 19.0 & 1.11 $\pm$ 0.18 & 267.33 $\pm$ 15.96 & 1.34 $\pm$ 0.12 & 41.8 $\pm$ 2.0 & 81.872 $\pm$ 5.504\\ 
89 & NGC300-12 & 262.0 $\pm$ 19.0 & -& 39.9 $\pm$ 2.66 & 0.73 $\pm$ 0.07 & 72.5 $\pm$ 3.4 & 75.68 $\pm$ 4.816\\ 
90 & NGC300-13 & 246.0 $\pm$ 18.0 & -& 158.27 $\pm$ 9.31 & 1.04 $\pm$ 0.09 & 37.5 $\pm$ 1.8 & 72.928 $\pm$ 4.816\\ 
91 & NGC300-14 & 248.0 $\pm$ 18.0 & 0.75 $\pm$ 0.06 & 240.73 $\pm$ 14.63 & 1.4 $\pm$ 0.1 & 41.6 $\pm$ 1.7 & 101.824 $\pm$ 6.536\\ 
92 & NGC300-15 & 185.0 $\pm$ 13.0 & -& 122.36 $\pm$ 6.65 & 1.1 $\pm$ 0.1 & 48.0 $\pm$ 2.3 & 96.664 $\pm$ 6.192\\ 
93 & NGC300-16 & 264.0 $\pm$ 19.0 & -& 255.36 $\pm$ 14.63 & 0.99 $\pm$ 0.12 & 53.0 $\pm$ 2.5 & 83.592 $\pm$ 5.504\\ 
94 & NGC300-17 & 213.0 $\pm$ 15.0 & 0.59 $\pm$ 0.05 & 156.94 $\pm$ 9.31 & 1.32 $\pm$ 0.11 & 27.3 $\pm$ 1.3 & 93.912 $\pm$ 6.192\\ 
95 & NGC300-18 & 259.0 $\pm$ 18.0 & -& 219.45 $\pm$ 13.3 & 1.26 $\pm$ 0.1 & 57.2 $\pm$ 2.7 & 89.096 $\pm$ 5.848\\ 
96 & NGC300-19 & 194.0 $\pm$ 14.0 & 0.61 $\pm$ 0.5 & 301.91 $\pm$ 17.29 & 0.95 $\pm$ 0.07 & 30.6 $\pm$ 1.4 & 79.464 $\pm$ 5.16\\ 
97 & NGC300-20 & 146.0 $\pm$ 10.0 & 0.71 $\pm$ 0.06 & 136.99 $\pm$ 7.98 & 1.15 $\pm$ 0.08 & 20.0 $\pm$ 0.9 & 98.384 $\pm$ 6.536\\ 
98 & NGC300-21 & 217.0 $\pm$ 16.0 & -& 102.41 $\pm$ 5.32 & 1.09 $\pm$ 0.12 & 55.5 $\pm$ 2.6 & 99.072 $\pm$ 6.536\\ 
99 & NGC300-22 & 270.0 $\pm$ 19.0 & -& 263.34 $\pm$ 15.96 & 0.82 $\pm$ 0.08 & 71.6 $\pm$ 3.3 & 76.712 $\pm$ 5.16\\ 
100 & NGC300-23 & 176.0 $\pm$ 13.0 & 0.57 $\pm$ 0.07 & 239.4 $\pm$ 13.3 & 0.99 $\pm$ 0.09 & 28.0 $\pm$ 1.3 & 82.56 $\pm$ 5.504\\ 
101 & NGC300-25 & 287.0 $\pm$ 21.0 & -& 176.89 $\pm$ 10.64 & 1.07 $\pm$ 0.13 & 45.0 $\pm$ 2.1 & 84.624 $\pm$ 5.504\\ 
102 & NGC300-26 & 160.0 $\pm$ 11.0 & 1.19 $\pm$ 0.1 & 344.47 $\pm$ 19.95 & 1.43 $\pm$ 0.1 & 22.1 $\pm$ 1.0 & 97.008 $\pm$ 6.192\\ 
103 & NGC300-27 & 357.0 $\pm$ 25.0 & 1.59 $\pm$ 0.11 & 236.74 $\pm$ 13.3 & 1.5 $\pm$ 0.11 & 81.7 $\pm$ 3.8 & 59.512 $\pm$ 3.784\\ 
104 & NGC300-28 & 314.0 $\pm$ 22.0 & 1.89 $\pm$ 0.13 & 324.52 $\pm$ 18.62 & 1.51 $\pm$ 0.19 & 37.2 $\pm$ 1.7 & 72.928 $\pm$ 4.816\\ 
105 & M31-2            & 210.0 $\pm$ 20.0 & -& 80.0 $\pm$ 6.0 & 0.6 $\pm$ 0.07 & 40.0 $\pm$ 4.0 & 79.0 $\pm$ 10.0\\ 
106 & M31-17          & 143.0 $\pm$ 13.0 & 0.34 $\pm$ 0.03 & 154.0 $\pm$ 11.0 & 0.97 $\pm$ 0.11 & 26.0 $\pm$ 3.0 & 79.0 $\pm$ 10.0\\ 
107 & M31-25          & 158.0 $\pm$ 10.0 & 1.3 $\pm$ 0.08 & 337.0 $\pm$ 19.0 & 1.21 $\pm$ 0.08 & 19.0 $\pm$ 1.0 & 72.0 $\pm$ 7.0\\ 
108 & M31-26          & 230.0 $\pm$ 20.0 & 1.2 $\pm$ 0.1 & 295.0 $\pm$ 26.0 & 1.37 $\pm$ 0.1 & 30.0 $\pm$ 2.0 & 76.0 $\pm$ 7.0\\ 
109 & M31-35          & 150.0 $\pm$ 10.0 & 1.35 $\pm$ 0.08 & 424.0 $\pm$ 26.0 & 1.45 $\pm$ 0.14 & 22.0 $\pm$ 2.0 & 72.0 $\pm$ 7.0\\ 
110 & NGC628+49.8+48.7 & 165.3 $\pm$ 3.8 & -& 67.6 $\pm$ 1.3 & 0.7 $\pm$ 0.1 & 42.6 $\pm$ 0.9 & 133.6 $\pm$ 2.6\\ 
111 & NGC628-73.1-27.3 & 113.4 $\pm$ 2.3 & -& 19.3 $\pm$ 0.4 & 0.4 $\pm$ 0.1 & 69.0 $\pm$ 1.4 & 74.6 $\pm$ 1.5\\ 
112 & NGC628-76.2+22.9 & 116.5 $\pm$ 4.4 & -& 23.2 $\pm$ 0.8 & 0.4 $\pm$ 0.1 & 49.2 $\pm$ 1.0 & 94.4 $\pm$ 2.0\\ 
113 & NGC628+68.5+53.4 & 141.0 $\pm$ 2.9 & -& 44.9 $\pm$ 0.9 & 0.7 $\pm$ 0.1 & 58.6 $\pm$ 1.2 & 113.0 $\pm$ 2.3\\ 
114 & NGC628+81.6-32.3 & 93.2 $\pm$ 1.9 & -& 20.1 $\pm$ 0.4 & 0.3 $\pm$ 0.1 & 41.3 $\pm$ 0.8 & 107.2 $\pm$ 2.2\\ 
115 & NGC628-68.5+61.7 & 139.0 $\pm$ 3.3 & -& 32.5 $\pm$ 0.7 & 0.4 $\pm$ 0.1 & 51.8 $\pm$ 1.0 & 108.6 $\pm$ 2.2\\ 
116 & NGC628+76.9-49.6 & 134.8 $\pm$ 2.9 & -& 18.8 $\pm$ 1.2 & 0.4 $\pm$ 0.1 & 79.9 $\pm$ 1.6 & 119.9 $\pm$ 2.7\\ 
117 & NGC628-13.1+107.5 & 186.2 $\pm$ 3.8 & -& 93.1 $\pm$ 1.9 & 0.7 $\pm$ 0.1 & 48.6 $\pm$ 1.0 & 119.0 $\pm$ 2.3\\ 
118 & NGC628-35.7+119.6 & 176.4 $\pm$ 3.5 & -& 119.2 $\pm$ 2.4 & 0.6 $\pm$ 0.1 & 62.1 $\pm$ 1.2 & 113.4 $\pm$ 2.3\\ 
119 & NGC628-20.3+124.6 & 216.5 $\pm$ 4.3 & -& 147.2 $\pm$ 2.9 & 1.1 $\pm$ 0.1 & 47.5 $\pm$ 0.9 & 156.9 $\pm$ 3.2\\ 
120 & NGC628-59.6-111.6 & 153.7 $\pm$ 8.6 & -& 50.7 $\pm$ 1.1 & 0.5 $\pm$ 0.1 & 60.6 $\pm$ 1.2 & 100.1 $\pm$ 2.9\\ 
121 & NGC628+61.2+113.5 & 220.8 $\pm$ 4.4 & -& 51.4 $\pm$ 1.1 & 0.5 $\pm$ 0.1 & 55.0 $\pm$ 1.1 & 93.9 $\pm$ 1.9\\ 

 \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{cccccccc}
\cline{1-8}
  & Line & [OII] & [OIII] & [OIII] & [SIII] & [SII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 &4959, 5007 & 6312  & 6717, 6731 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{6}{c}{I($\lambda $)$^{a}$} \\ \hline


 
 
122 & NGC628+42.6-120.7 & 203.6 $\pm$ 8.4 & -& 82.6 $\pm$ 1.6 & 0.8 $\pm$ 0.1 & 54.6 $\pm$ 1.1 & 133.4 $\pm$ 2.7\\ 
123 & NGC628+131.9+18.5 & 211.0 $\pm$ 4.2 & 0.8 $\pm$ 0.1 & 128.8 $\pm$ 2.5 & 0.7 $\pm$ 0.1 & 62.1 $\pm$ 1.3 & 110.7 $\pm$ 2.2\\ 
124 & NGC628+125.4-62.4 & 251.2 $\pm$ 18.9 & -& 103.3 $\pm$ 2.4 & 0.8 $\pm$ 0.2 & 60.7 $\pm$ 1.6 & 102.4 $\pm$ 3.9\\ 
126 & NGC628+131.7-70.2 & 336.5 $\pm$ 52.7 & -& 91.0 $\pm$ 2.0 & 0.9 $\pm$ 0.1 & 58.1 $\pm$ 1.9 & 91.0 $\pm$ 4.4\\ 
127 & NGC628+151.0+22.3 & 181.1 $\pm$ 8.5 & 0.8 $\pm$ 0.2 & 217.7 $\pm$ 4.4 & 1.2 $\pm$ 0.2 & 35.7 $\pm$ 0.7 & 158.7 $\pm$ 4.2\\ 
128 & NGC628-157.9-0.3 & 211.1 $\pm$ 8.5 & -& 115.2 $\pm$ 2.3 & 0.9 $\pm$ 0.2 & 33.0 $\pm$ 0.7 & 123.7 $\pm$ 2.6\\ 
129 & NGC628-24.5-155.6 & 193.2 $\pm$ 11.6 & -& 109.1 $\pm$ 2.2 & 0.6 $\pm$ 0.1 & 50.7 $\pm$ 1.0 & 97.5 $\pm$ 2.4\\ 
130 & NGC628-129.8+94.7 & 190.1 $\pm$ 3.8 & -& 99.9 $\pm$ 2.0 & 0.6 $\pm$ 0.1 & 59.2 $\pm$ 1.2 & 110.1 $\pm$ 2.2\\ 
131 & NGC628+78.6-137.6 & 150.4 $\pm$ 3.0 & -& 170.8 $\pm$ 3.4 & 0.7 $\pm$ 0.1 & 30.6 $\pm$ 0.7 & 122.9 $\pm$ 2.4\\ 
125 & NGC628-130.9+71.8 & 218.6 $\pm$ 4.4 & -& 81.5 $\pm$ 1.6 & 0.8 $\pm$ 0.1 & 52.2 $\pm$ 1.0 & 116.0 $\pm$ 2.3\\ 
132 & NGC628+140.3+82.0 & 229.7 $\pm$ 4.6 & -& 124.1 $\pm$ 2.5 & 1.1 $\pm$ 0.1 & 41.5 $\pm$ 0.8 & 92.1 $\pm$ 1.8\\ 
133 & NGC628-42.8-158.2 & 189.3 $\pm$ 12.4 & 1.0 $\pm$ 0.2 & 199.3 $\pm$ 4.0 & 1.0 $\pm$ 0.1 & 34.9 $\pm$ 0.7 & 130.3 $\pm$ 3.2\\ 
134 & NGC628+163.5+64.4 & 251.0 $\pm$ 13.5 & -& 116.6 $\pm$ 2.3 & 0.8 $\pm$ 0.1 & 79.7 $\pm$ 1.6 & 126.0 $\pm$ 2.9\\ 
135 & NGC628-4.5+185.6 & 213.6 $\pm$ 4.3 & -& 156.2 $\pm$ 3.1 & 1.0 $\pm$ 0.1 & 34.9 $\pm$ 0.7 & 89.2 $\pm$ 1.8\\ 
136 & NGC628+176.7-50.0 & 146.8 $\pm$ 15.2 & -& 130.8 $\pm$ 2.7 & 0.8 $\pm$ 0.2 & 44.0 $\pm$ 0.9 & 83.6 $\pm$ 2.3\\ 
137 & NGC628-76.2-171.8 & 209.5 $\pm$ 15.9 & 1.0 $\pm$ 0.2 & 229.1 $\pm$ 4.6 & 0.7 $\pm$ 0.1 & 63.8 $\pm$ 1.4 & 88.9 $\pm$ 3.3\\ 
138 & NGC628+31.6-191.1 & 234.4 $\pm$ 5.0 & 0.5 $\pm$ 0.1 & 189.4 $\pm$ 3.8 & 1.1 $\pm$ 0.1 & 40.2 $\pm$ 0.8 & 103.2 $\pm$ 2.0\\ 
139 & NGC628-200.6-4.2 & 239.3 $\pm$ 8.9 & 0.6 $\pm$ 0.1 & 177.0 $\pm$ 3.5 & 0.9 $\pm$ 0.2 & 41.6 $\pm$ 0.8 & 118.8 $\pm$ 2.7\\ 
140 & NGC628-184.7+83.4 & 286.6 $\pm$ 5.7 & 0.7 $\pm$ 0.1 & 173.6 $\pm$ 3.5 & 1.0 $\pm$ 0.1 & 62.6 $\pm$ 1.2 & 134.5 $\pm$ 2.7\\ 
141 & NGC628-206.5-25.7 & 172.3 $\pm$ 6.8 & 1.0 $\pm$ 0.1 & 406.3 $\pm$ 8.2 & 1.1 $\pm$ 0.3 & 25.1 $\pm$ 0.6 & 113.2 $\pm$ 2.6\\ 
142 & NGC628-90.1+190.2 & 280.4 $\pm$ 5.6 & 0.6 $\pm$ 0.1 & 192.5 $\pm$ 3.9 & 1.1 $\pm$ 0.1 & 40.4 $\pm$ 0.8 & 101.9 $\pm$ 2.0\\ 
143 & NGC628+232.7+6.6 & 224.4 $\pm$ 12.6 & 1.5 $\pm$ 0.5 & 285.7 $\pm$ 5.7 & 1.0 $\pm$ 0.3 & 53.8 $\pm$ 1.1 & 95.1 $\pm$ 2.4\\ 
144 & NGC628+237.6+3.0 & 280.4 $\pm$ 20.7 & 0.9 $\pm$ 0.3 & 184.0 $\pm$ 3.6 & 1.0 $\pm$ 0.3 & 56.7 $\pm$ 1.2 & 89.6 $\pm$ 2.9\\ 
145 & NGC628+254.3-42.8 & 322.2 $\pm$ 38.5 & 2.0 $\pm$ 0.4 & 250.8 $\pm$ 5.0 & 1.9 $\pm$ 0.3 & 94.6 $\pm$ 1.9 & 104.3 $\pm$ 3.4\\ 
146 & NGC628+252.1-92.1 & 258.8 $\pm$ 11.6 & 2.7 $\pm$ 0.5 & 323.7 $\pm$ 6.5 & 1.6 $\pm$ 0.3 & 39.4 $\pm$ 0.9 & 91.5 $\pm$ 2.8\\ 
147 & NGC628+289.9-17.4 & 151.9 $\pm$ 3.2 & 2.9 $\pm$ 0.2 & 556.8 $\pm$ 11.1 & 1.6 $\pm$ 0.1 & 18.7 $\pm$ 0.4 & 101.8 $\pm$ 2.1\\ 
148 & NGC628+298.4+12.3 & 111.4 $\pm$ 2.2 & 4.0 $\pm$ 0.2 & 681.2 $\pm$ 13.6 & 1.5 $\pm$ 0.1 & 12.0 $\pm$ 0.2 & 85.7 $\pm$ 1.8\\ 
149 & NGC5194+30.2+2.2 & 151.0 $\pm$ 4.7 & -& 47.1 $\pm$ 1.0 & 0.247 $\pm$ 0.063 & 51.2 $\pm$ 1.02 & 27.45 $\pm$ 0.55\\ 
150 & NGC5194+91.0+69.0 & 87.0 $\pm$ 7.6 & -& 19.5 $\pm$ 0.8 & 0.295 $\pm$ 0.098 & 64.2 $\pm$ 1.29 & 101.1 $\pm$ 2.04\\ 
151 & NGC5194-86.5-79.4 & 53.4 $\pm$ 1.34 & -& 9.45 $\pm$ 0.199 & 0.117 $\pm$ 0.019 & 46.9 $\pm$ 0.94 & 46.3 $\pm$ 0.92\\ 
152 & NGC5194-97.0-78.4 & 94.0 $\pm$ 2.3 & -& 25.33 $\pm$ 0.63 & 0.257 $\pm$ 0.034 & 49.2 $\pm$ 0.98 & 84.6 $\pm$ 1.69\\ 
153 & NGC5194-3.0+131.9 & 149.0 $\pm$ 8.4 & -& 49.6 $\pm$ 1.07 & 0.46 $\pm$ 0.11 & 51.2 $\pm$ 1.03 & 51.2 $\pm$ 1.59\\ 
154 & NGC5194-57.2+118.2 & 134.0 $\pm$ 5.3 & -& 47.6 $\pm$ 0.95 & 0.312 $\pm$ 0.074 & 53.1 $\pm$ 1.07 & 48.2 $\pm$ 1.13\\ 
155 & NGC5194-66.6+122.9 & 206.4 $\pm$ 11.7 & -& 46.3 $\pm$ 0.96 & 0.328 $\pm$ 0.085 & 43.4 $\pm$ 0.87 & 50.6 $\pm$ 1.35\\ 
156 & NGC5194+30.8+139.0 & 109.0 $\pm$ 5.4 & -& 20.55 $\pm$ 0.44 & 0.267 $\pm$ 0.055 & 73.9 $\pm$ 1.47 & 36.5 $\pm$ 0.81\\ 
157 & NGC5194+104.1-105.5 & 128.0 $\pm$ 4.9 & -& 43.4 $\pm$ 0.87 & 0.444 $\pm$ 0.042 & 36.3 $\pm$ 0.73 & 95.7 $\pm$ 1.95\\ 
158 & NGC5194+98.1-113.8 & 90.0 $\pm$ 2.4 & -& 25.01 $\pm$ 0.5 & 0.289 $\pm$ 0.021 & 43.7 $\pm$ 0.87 & 82.6 $\pm$ 2.65\\ 
159 & NGC5194+71.2+135.9 & 110.0 $\pm$ 8.0 & -& 17.43 $\pm$ 0.37 & 0.224 $\pm$ 0.04 & 48.6 $\pm$ 0.97 & 42.9 $\pm$ 1.1\\ 
160 & NGC5194+83.4-133.1 & 115.0 $\pm$ 4.6 & -& 19.45 $\pm$ 0.43 & 0.308 $\pm$ 0.045 & 52.2 $\pm$ 1.04 & 79.7 $\pm$ 2.55\\ 
161 & NGC5194+109.9-121.4 & 138.0 $\pm$ 4.5 & -& 51.7 $\pm$ 1.03 & 0.427 $\pm$ 0.089 & 66.9 $\pm$ 1.33 & 87.9 $\pm$ 2.7\\ 
162 & NGC5194+150.6+99.0 & 194.1 $\pm$ 16.1 & -& 70.4 $\pm$ 1.46 & 0.67 $\pm$ 0.15 & 53.7 $\pm$ 1.08 & 102.5 $\pm$ 2.83\\ 
163 & NGC5194-159.5-116.4 & 199.6 $\pm$ 4.5 & -& 28.31 $\pm$ 0.84 & 0.47 $\pm$ 0.11 & 80.2 $\pm$ 1.6 & 80.7 $\pm$ 1.57\\ 
164 & NGC5194-135.4-181.4 & 194.3 $\pm$ 10.8 & -& 76.2 $\pm$ 1.48 & 0.515 $\pm$ 0.083 & 50.7 $\pm$ 1.01 & 93.3 $\pm$ 1.93\\ 
165 & NGC5194+114.5+230.8 & 245.0 $\pm$ 30.0 & -& 76.8 $\pm$ 1.51 & 0.84 $\pm$ 0.11 & 53.7 $\pm$ 1.14 & 98.8 $\pm$ 3.35\\ 
166 & NGC5457-75.0+29.3 & 75.0 $\pm$ 2.2 & -& 8.98 $\pm$ 0.4 & 0.218 $\pm$ 0.067 & 55.3 $\pm$ 1.97 & 62.3 $\pm$ 3.14\\ 
167 & NGC5457+138.9+30.6 & 153.0 $\pm$ 4.0 & -& 38.34 $\pm$ 0.77 & 0.531 $\pm$ 0.056 & 39.6 $\pm$ 1.38 & 89.0 $\pm$ 3.9\\ 
168 & NGC5457+134.4-58.8 & 202.0 $\pm$ 6.5 & -& 38.72 $\pm$ 0.77 & 0.462 $\pm$ 0.098 & 66.0 $\pm$ 3.2 & 45.6 $\pm$ 2.95\\ 
169 & NGC5457+164.6+9.9 & 194.7 $\pm$ 5.8 & 0.203 $\pm$ 0.022 & 130.6 $\pm$ 2.65 & 0.785 $\pm$ 0.029 & 27.7 $\pm$ 1.18 & 117.0 $\pm$ 6.8\\ 
170 & NGC5457-70.2+162.2 & 190.0 $\pm$ 6.1 & -& 90.8 $\pm$ 1.86 & 0.89 $\pm$ 0.14 & 38.8 $\pm$ 1.5 & 127.0 $\pm$ 6.4\\ 
171 & NGC5457+166.4+86.3 & 162.0 $\pm$ 5.5 & -& 43.8 $\pm$ 0.95 & 0.485 $\pm$ 0.075 & 52.6 $\pm$ 2.21 & 52.0 $\pm$ 2.9\\ 
172 & NGC5457+177.2-42.8 & 154.0 $\pm$ 4.2 & -& 75.9 $\pm$ 1.48 & 0.441 $\pm$ 0.052 & 33.2 $\pm$ 1.37 & 54.7 $\pm$ 2.98\\ 
173 & NGC5457-159.9+89.6 & 157.0 $\pm$ 4.7 & -& 24.73 $\pm$ 0.5 & 0.349 $\pm$ 0.07 & 62.0 $\pm$ 2.6 & 89.0 $\pm$ 5.1\\ 
174 & NGC5457+133.1-126.8 & 174.0 $\pm$ 7.5 & -& 32.99 $\pm$ 0.67 & 0.32 $\pm$ 0.1 & 54.0 $\pm$ 2.8 & 32.7 $\pm$ 2.33\\ 
175 & NGC5457+177.2+76.1 & 192.5 $\pm$ 5.5 & -& 66.7 $\pm$ 1.33 & 0.669 $\pm$ 0.084 & 51.4 $\pm$ 1.9 & 76.0 $\pm$ 3.6\\ 
176 & NGC5457-120.2+146.9 & 185.0 $\pm$ 4.5 & -& 32.59 $\pm$ 0.98 & 0.503 $\pm$ 0.049 & 54.2 $\pm$ 1.67 & 88.1 $\pm$ 3.83\\ 
177 & NGC5457+130.2+157.4 & 189.0 $\pm$ 4.5 & -& 60.7 $\pm$ 1.22 & 0.443 $\pm$ 0.078 & 61.0 $\pm$ 2.4 & 63.0 $\pm$ 3.3\\ 
178 & NGC5457+129.2+161.7 & 145.0 $\pm$ 4.9 & -& 49.8 $\pm$ 1.08 & 0.538 $\pm$ 0.064 & 62.0 $\pm$ 2.3 & 64.3 $\pm$ 3.33\\ 
179 & NGC5457-145.1+146.8 & 202.9 $\pm$ 7.1 & -& 64.4 $\pm$ 1.4 & 0.63 $\pm$ 0.17 & 44.4 $\pm$ 2.05 & 65.0 $\pm$ 4.1\\ 
180 & NGC5457+103.5+192.6 & 128.0 $\pm$ 5.1 & -& 17.7 $\pm$ 2.1 & 0.72 $\pm$ 0.21 & 48.0 $\pm$ 2.5 & 67.8 $\pm$ 4.58\\ 
181 & NGC5457-205.4-98.2 & 238.5 $\pm$ 7.1 & -& 59.8 $\pm$ 1.51 & 0.63 $\pm$ 0.11 & 66.0 $\pm$ 2.9 & 98.0 $\pm$ 5.9\\ 
182 & NGC5457+17.3-235.4 & 218.5 $\pm$ 5.3 & 0.403 $\pm$ 0.057 & 152.4 $\pm$ 3.06 & 0.843 $\pm$ 0.077 & 43.3 $\pm$ 1.39 & 48.6 $\pm$ 1.85\\ 

\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{cccccccc}
\cline{1-8}
  & Line & [OII] & [OIII] & [OIII] & [SIII] & [SII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 &4959, 5007 & 6312  & 6717, 6731 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{6}{c}{I($\lambda $)$^{a}$} \\ \hline

 
 
 
183 & NGC5457+189.2-136.3 & 214.2 $\pm$ 5.1 & 0.658 $\pm$ 0.026 & 42.7 $\pm$ 1.19 & 1.11 $\pm$ 0.033 & 78.0 $\pm$ 3.1 & 52.2 $\pm$ 3.08\\ 
184 & NGC5457-183.9-179.0 & 289.2 $\pm$ 7.2 & 0.36 $\pm$ 0.078 & 69.6 $\pm$ 1.43 & 0.79 $\pm$ 0.13 & 94.0 $\pm$ 3.8 & 78.0 $\pm$ 4.0\\ 
185 & NGC5457-249.4-51.3 & 376.8 $\pm$ 8.6 & -& 131.5 $\pm$ 2.69 & 0.75 $\pm$ 0.13 & 131.0 $\pm$ 5.7 & 68.4 $\pm$ 3.89\\ 
186 & NGC5457+225.6-124.1 & 257.9 $\pm$ 9.1 & 0.658 $\pm$ 0.041 & 184.2 $\pm$ 3.72 & 1.02 $\pm$ 0.053 & 34.8 $\pm$ 1.25 & 59.8 $\pm$ 2.67\\ 
187 & NGC5457+117.9-235.0 & 167.0 $\pm$ 5.8 & 0.613 $\pm$ 0.084 & 143.4 $\pm$ 2.92 & 1.0 $\pm$ 0.22 & 46.0 $\pm$ 2.5 & 81.0 $\pm$ 5.8\\ 
188 & NGC5457-208.0-180.7 & 341.5 $\pm$ 9.6 & -& 38.93 $\pm$ 1.03 & 0.85 $\pm$ 0.11 & 79.0 $\pm$ 2.9 & 75.0 $\pm$ 3.68\\ 
189 & NGC5457-12.3-271.1 & 377.5 $\pm$ 13.9 & -& 175.7 $\pm$ 3.47 & 0.92 $\pm$ 0.27 & 83.0 $\pm$ 3.7 & 52.0 $\pm$ 3.4\\ 
190 & NGC5457-200.3-193.6 & 250.2 $\pm$ 7.1 & 0.63 $\pm$ 0.06 & 109.4 $\pm$ 2.15 & 0.75 $\pm$ 0.19 & 73.0 $\pm$ 2.8 & 65.9 $\pm$ 3.4\\ 
191 & NGC5457+96.7+266.9 & 221.9 $\pm$ 4.6 & 0.343 $\pm$ 0.068 & 338.6 $\pm$ 6.8 & 0.714 $\pm$ 0.089 & 33.8 $\pm$ 1.03 & 78.8 $\pm$ 2.46\\ 
192 & NGC5457+67.5+277.0 & 244.3 $\pm$ 7.4 & 0.963 $\pm$ 0.035 & 216.3 $\pm$ 4.3 & 1.34 $\pm$ 0.12 & 63.0 $\pm$ 2.4 & 51.5 $\pm$ 2.76\\ 
193 & NGC5457+252.2-109.8 & 161.0 $\pm$ 7.2 & 0.784 $\pm$ 0.057 & 456.9 $\pm$ 9.1 & 0.707 $\pm$ 0.099 & 26.4 $\pm$ 1.47 & 93.0 $\pm$ 8.8\\ 
194 & NGC5457+254.6-107.2 & 284.7 $\pm$ 6.5 & 1.39 $\pm$ 0.034 & 214.1 $\pm$ 4.2 & 1.54 $\pm$ 0.067 & 32.1 $\pm$ 1.22 & 68.2 $\pm$ 3.24\\ 
195 & NGC5457+281.4-71.8 & 281.4 $\pm$ 8.2 & 0.739 $\pm$ 0.055 & 113.7 $\pm$ 2.26 & 0.97 $\pm$ 0.15 & 68.0 $\pm$ 2.8 & 97.0 $\pm$ 5.6\\ 
196 & NGC5457-243.0+159.6 & 251.1 $\pm$ 5.2 & 0.291 $\pm$ 0.048 & 297.1 $\pm$ 5.9 & 0.82 $\pm$ 0.19 & 57.2 $\pm$ 1.77 & 75.0 $\pm$ 3.2\\ 
197 & NGC5457+249.3+201.9 & 301.7 $\pm$ 12.6 & 1.16 $\pm$ 0.04 & 159.0 $\pm$ 3.18 & 1.38 $\pm$ 0.15 & 64.0 $\pm$ 3.3 & 92.0 $\pm$ 6.0\\ 
198 & NGC5457-297.7+87.1 & 245.6 $\pm$ 9.8 & 0.537 $\pm$ 0.055 & 145.0 $\pm$ 2.91 & 1.42 $\pm$ 0.31 & 68.0 $\pm$ 3.0 & 86.0 $\pm$ 5.4\\ 
199 & NGC5457+354.1+71.2 & 228.1 $\pm$ 8.2 & 1.94 $\pm$ 0.057 & 325.1 $\pm$ 6.5 & 1.4 $\pm$ 0.11 & 26.0 $\pm$ 1.15 & 86.0 $\pm$ 4.6\\ 
200 & NGC5457-164.9-333.9 & 175.8 $\pm$ 6.8 & 0.864 $\pm$ 0.027 & 470.2 $\pm$ 9.4 & 1.08 $\pm$ 0.12 & 28.8 $\pm$ 1.4 & 117.0 $\pm$ 7.4\\ 
201 & NGC5457+360.9+75.3 & 574.3 $\pm$ 16.4 & 1.71 $\pm$ 0.053 & 106.0 $\pm$ 14.9 & 1.28 $\pm$ 0.12 & 78.0 $\pm$ 10.6 & 44.6 $\pm$ 11.4\\ 
202 & NGC5457-178.0+319.1 & 288.0 $\pm$ 10.1 & -& 176.3 $\pm$ 3.48 & 1.36 $\pm$ 0.41 & 73.0 $\pm$ 3.7 & 88.0 $\pm$ 5.5\\ 
203 & NGC5457-377.9-64.9 & 290.5 $\pm$ 9.2 & 0.773 $\pm$ 0.039 & 277.8 $\pm$ 7.0 & 0.88 $\pm$ 0.14 & 65.0 $\pm$ 3.3 & 100.0 $\pm$ 8.3\\ 
204 & NGC5457-99.6-388.0 & 394.6 $\pm$ 13.1 & 2.08 $\pm$ 0.044 & 201.1 $\pm$ 3.99 & 1.41 $\pm$ 0.044 & 49.4 $\pm$ 2.08 & 79.0 $\pm$ 4.5\\ 
205 & NGC5457-226.9-366.4 & 319.0 $\pm$ 11.6 & 0.888 $\pm$ 0.06 & 195.3 $\pm$ 3.88 & 1.28 $\pm$ 0.12 & 42.3 $\pm$ 2.04 & 48.0 $\pm$ 3.2\\ 
206 & NGC5457-345.5+273.8 & 236.3 $\pm$ 6.6 & 3.95 $\pm$ 0.14 & 431.4 $\pm$ 8.7 & 1.53 $\pm$ 0.24 & 38.8 $\pm$ 1.47 & 56.5 $\pm$ 3.09\\ 
207 & NGC5457-410.3-206.3 & 281.4 $\pm$ 7.3 & 0.66 $\pm$ 0.074 & 433.8 $\pm$ 8.7 & 1.2 $\pm$ 0.21 & 28.7 $\pm$ 1.01 & 43.6 $\pm$ 2.01\\ 
208 & NGC5457-371.1-280.0 & 155.0 $\pm$ 4.7 & 1.61 $\pm$ 0.036 & 497.1 $\pm$ 9.9 & 1.28 $\pm$ 0.044 & 24.3 $\pm$ 0.99 & 52.0 $\pm$ 3.08\\ 
209 & NGC5457-368.3-285.6 & 197.0 $\pm$ 4.9 & 1.64 $\pm$ 0.033 & 542.9 $\pm$ 10.8 & 1.4 $\pm$ 0.042 & 28.9 $\pm$ 1.05 & 45.8 $\pm$ 2.09\\ 
210 & NGC5457-455.7-55.8 & 275.2 $\pm$ 7.8 & 2.92 $\pm$ 0.058 & 450.9 $\pm$ 9.1 & 1.28 $\pm$ 0.12 & 38.0 $\pm$ 1.44 & 42.6 $\pm$ 2.27\\ 
211 & NGC5457-392.0-270.1 & 314.8 $\pm$ 7.7 & 2.1 $\pm$ 0.044 & 333.6 $\pm$ 6.7 & 1.31 $\pm$ 0.039 & 35.2 $\pm$ 1.07 & 37.1 $\pm$ 1.54\\ 
212 & NGC5457-414.1-253.6 & 322.9 $\pm$ 10.2 & 2.7 $\pm$ 0.12 & 363.0 $\pm$ 7.3 & 1.43 $\pm$ 0.25 & 30.6 $\pm$ 1.73 & 41.0 $\pm$ 3.17\\ 
213 & NGC5457-464.7-131.0 & 317.9 $\pm$ 10.1 & 3.54 $\pm$ 0.12 & 378.3 $\pm$ 7.6 & 1.17 $\pm$ 0.31 & 43.0 $\pm$ 2.6 & 30.96 $\pm$ 2.19\\ 
214 & NGC5457-466.1-128.2 & 265.3 $\pm$ 8.6 & 2.49 $\pm$ 0.08 & 500.2 $\pm$ 10.0 & 1.23 $\pm$ 0.14 & 34.6 $\pm$ 1.41 & 35.0 $\pm$ 1.99\\ 
215 & NGC5457-479.7-3.9 & 205.8 $\pm$ 6.8 & 2.93 $\pm$ 0.11 & 481.3 $\pm$ 9.6 & 1.22 $\pm$ 0.31 & 21.73 $\pm$ 1.01 & 62.0 $\pm$ 4.3\\ 
216 & NGC5457-481.4-0.5 & 330.6 $\pm$ 12.2 & 3.92 $\pm$ 0.078 & 357.0 $\pm$ 7.2 & 1.31 $\pm$ 0.11 & 42.5 $\pm$ 2.23 & 56.0 $\pm$ 5.1\\ 
217 & NGC5457-453.8-191.8 & 272.4 $\pm$ 10.6 & 3.64 $\pm$ 0.096 & 588.3 $\pm$ 11.7 & 1.44 $\pm$ 0.074 & 46.0 $\pm$ 2.6 & 65.0 $\pm$ 6.1\\ 
218 & NGC5457-540.5-149.9 & 321.5 $\pm$ 12.0 & 6.56 $\pm$ 0.13 & 784.6 $\pm$ 28.0 & 1.47 $\pm$ 0.14 & 49.0 $\pm$ 4.9 & 70.0 $\pm$ 20.0\\ 
219 & NGC5457+509.5+264.1 & 237.4 $\pm$ 12.1 & 3.37 $\pm$ 0.067 & 483.1 $\pm$ 9.6 & 1.53 $\pm$ 0.071 & 22.49 $\pm$ 1.33 & 48.0 $\pm$ 3.8\\ 
220 & NGC5457+667.9+174.1 & 237.9 $\pm$ 8.2 & 8.85 $\pm$ 0.027 & 356.8 $\pm$ 7.2 & 1.64 $\pm$ 0.059 & 27.5 $\pm$ 1.11 & 45.64 $\pm$ 2.75\\ 
221 & NGC5457+692.1+272.9 & 208.6 $\pm$ 7.9 & 4.11 $\pm$ 0.19 & 222.1 $\pm$ 5.4 & 1.64 $\pm$ 0.32 & 22.47 $\pm$ 1.3 & 43.0 $\pm$ 6.0\\ 
222 & N300-R20 & 190.0 $\pm$ 12.0 & 0.6 $\pm$ 0.12 & 286.0 $\pm$ 20.0 & 1.2 $\pm$ 0.2 & 27.0 $\pm$ 3.0 & 96.0 $\pm$ 7.0\\ 
223 & N300-R23 & 172.0 $\pm$ 12.0 & 0.51 $\pm$ 0.1 & 259.0 $\pm$ 18.0 & 1.02 $\pm$ 0.18 & 32.0 $\pm$ 2.0 & 91.0 $\pm$ 7.0\\ 
224 & N300-R14 & 222.0 $\pm$ 14.0 & 0.75 $\pm$ 0.09 & 240.0 $\pm$ 17.0 & 1.3 $\pm$ 0.2 & 40.0 $\pm$ 3.0 & 78.0 $\pm$ 6.0\\ 
225 & N300-R5 & 313.0 $\pm$ 19.0 & 1.1 $\pm$ 0.3 & 270.0 $\pm$ 11.0 & 1.7 $\pm$ 0.4 & 56.0 $\pm$ 6.0 & 69.0 $\pm$ 7.0\\ 
226 & N300-R2 & 203.0 $\pm$ 13.0 & 4.8 $\pm$ 0.5 & 633.0 $\pm$ 45.0 & 1.8 $\pm$ 0.4 & 24.0 $\pm$ 2.0 & 58.0 $\pm$ 4.0\\ 
227 & MWG-S83 & 90.88 $\pm$ 8.7 & 5.46 $\pm$ 0.69 & 763.4 $\pm$ 8.59 & 1.57 $\pm$ 0.09 & 6.78 $\pm$ 0.17 & 72.3 $\pm$ 0.18\\ 
228 & MWG-S132 & 411.94 $\pm$ 39.32 & -& 30.87 $\pm$ 0.67 & 0.75 $\pm$ 0.1 & 73.83 $\pm$ 0.49 & 68.11 $\pm$ 0.14\\ 
229 & MWG-S156 & 301.56 $\pm$ 24.4 & 0.43 $\pm$ 0.06 & 124.54 $\pm$ 1.17 & 1.44 $\pm$ 0.05 & 21.36 $\pm$ 0.13 & 127.55 $\pm$ 0.04\\ 
230 & MWG-S162 & 257.25 $\pm$ 8.53 & 0.7 $\pm$ 0.05 & 183.83 $\pm$ 0.66 & 1.62 $\pm$ 0.05 & 28.47 $\pm$ 0.11 & 144.75 $\pm$ 0.04\\ 
231 & MWG-S212 & 295.98 $\pm$ 20.43 & 2.28 $\pm$ 0.2 & 265.85 $\pm$ 2.05 & 1.61 $\pm$ 0.14 & 18.95 $\pm$ 0.28 & 69.28 $\pm$ 0.44\\ 
233 & LMC-30Dor & 131.0 $\pm$ 5.0 & 3.21 $\pm$ 0.05 & 674.31 $\pm$ 3.99 & 2.15 $\pm$ 0.04 & 16.9 $\pm$ 0.2 & 144.48 $\pm$ 3.44\\ 
233 & LMC-N44C & 69.0 $\pm$ 5.0 & 6.8 $\pm$ 0.5 & 936.32 $\pm$ 14.63 & 1.29 $\pm$ 0.07 & 14.7 $\pm$ 1.1 & 48.16 $\pm$ 4.97\\ 
234 & LMC-IC2111 & 277.0 $\pm$ 13.0 & 1.51 $\pm$ 0.07 & 412.3 $\pm$ 15.96 & 1.56 $\pm$ 0.08 & 24.0 $\pm$ 1.0 & 144.8 $\pm$ 10.32\\ 
235 & LMC-N11B & 224.0 $\pm$ 17.0 & 1.48 $\pm$ 0.06 & 409.64 $\pm$ 5.32 & 1.46 $\pm$ 0.07 & 24.0 $\pm$ 1.0 & 79.12 $\pm$ 4.97\\ 
236 & LMC-NGC1714 & 128.0 $\pm$ 6.0 & 2.5 $\pm$ 0.1 & 590.52 $\pm$ 23.94 & 1.55 $\pm$ 0.08 & 11.6 $\pm$ 0.6 & 141.04 $\pm$ 4.97\\ 
237 & SMC-N66A & 176.0 $\pm$ 12.0 & 5.1 $\pm$ 0.2 & 535.99 $\pm$ 7.98 & 1.79 $\pm$ 0.08 & 17.0 $\pm$ 0.9 & 79.12 $\pm$ 6.88\\ 
238 & SMC-N81 & 106.0 $\pm$ 7.0 & 6.8 $\pm$ 0.018 & 668.99 $\pm$ 10.64 & 1.76 $\pm$ 0.08 & 8.1 $\pm$ 0.4 & 48.16 $\pm$ 3.44\\ 
239 & SMC-N88A & 44.0 $\pm$ 6.0 & 13.0 $\pm$ 1.0 & 892.43 $\pm$ 17.29 & 1.8 $\pm$ 0.2 & 4.2 $\pm$ 0.5 & 48.16 $\pm$ 10.32\\ 
240 &  NGC3184-14.9-95.5                 & 125.6 $\pm$ 3.3 & -& 36.0 $\pm$ 0.8 & 0.6 $\pm$ 0.2 & 42.8 $\pm$ 0.9 & 35.3 $\pm$ 0.8\\ 
241 & NGC3184 -71.1+67.7                 & 127.8 $\pm$ 1.6 & -& 31.3 $\pm$ 0.6 & 0.4 $\pm$ 0.1 & 54.8 $\pm$ 1.0 & 69.1 $\pm$ 0.6\\ 
242 & NGC3184 +48.9+97.3                 & 178.7 $\pm$ 1.8 & -& 62.8 $\pm$ 1.7 & 0.5 $\pm$ 0.1 & 45.3 $\pm$ 0.9 & 85.9 $\pm$ 1.3\\ 
243 &  NGC3184+107.7-15.4                & 150.1 $\pm$ 1.7 & -& 26.1 $\pm$ 0.6 & 0.4 $\pm$ 0.1 & 63.7 $\pm$ 2.4 & 60.9 $\pm$ 0.7\\ 

 \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{cccccccc}
\cline{1-8}
  & Line & [OII] & [OIII] & [OIII] & [SIII] & [SII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 &4959, 5007 & 6312  & 6717, 6731 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{6}{c}{I($\lambda $)$^{a}$} \\ \hline


 
 
244 &  NGC3184-67.3+87.1                 & 150.6 $\pm$ 1.6 & -& 31.4 $\pm$ 0.5 & 0.5 $\pm$ 0.1 & 72.0 $\pm$ 1.7 & 80.1 $\pm$ 0.7\\ 
245 & NGC3184 +75.7+89.1                 & 200.9 $\pm$ 1.0 & -& 47.6 $\pm$ 0.3 & 0.7 $\pm$ 0.1 & 52.8 $\pm$ 1.1 & 126.3 $\pm$ 0.7\\ 
246 & NGC3184 -72.8+91.3                 & 182.7 $\pm$ 0.8 & -& 51.1 $\pm$ 0.4 & 0.4 $\pm$ 0.1 & 60.5 $\pm$ 0.5 & 76.3 $\pm$ 0.4\\ 
247 &  NGC3184+16.4+119.8                & 197.7 $\pm$ 1.1 & -& 112.7 $\pm$ 0.5 & 0.6 $\pm$ 0.1 & 48.4 $\pm$ 0.9 & 100.1 $\pm$ 0.4\\ 
248 &  NGC3184+110.6-52.0 & 194.1 $\pm$ 2.6 & -& 53.3 $\pm$ 0.9 & 0.6 $\pm$ 0.1 & 64.1 $\pm$ 3.9 & 69.4 $\pm$ 1.2\\ 
249 & NGC3184 -96.7+74.3                 & 233.7 $\pm$ 2.5 & -& 42.6 $\pm$ 0.9 & 0.6 $\pm$ 0.2 & 85.4 $\pm$ 1.6 & 62.6 $\pm$ 1.2\\ 
250 &  NGC3184+94.9-91.5                 & 177.1 $\pm$ 2.4 & -& 22.9 $\pm$ 1.0 & 0.4 $\pm$ 0.1 & 84.8 $\pm$ 2.5 & 58.8 $\pm$ 1.6\\ 
251 & NGC3184 +63.8+126.0 & 253.7 $\pm$ 2.1 & -& 110.3 $\pm$ 1.8 & 0.7 $\pm$ 0.3 & 78.0 $\pm$ 1.5 & 75.1 $\pm$ 1.4\\ 
252 &  NGC3184+123.8+76.5                & 255.9 $\pm$ 1.6 & -& 87.2 $\pm$ 1.4 & 0.7 $\pm$ 0.3 & 70.9 $\pm$ 0.9 & 65.1 $\pm$ 1.5\\ 
253 &  NGC3184+41.9+148.8                & 229.0 $\pm$ 1.6 & -& 89.9 $\pm$ 1.3 & 1.0 $\pm$ 0.2 & 51.7 $\pm$ 0.9 & 75.9 $\pm$ 1.1\\ 
254 & NGC3184 +80.0-148.2                & 288.0 $\pm$ 3.5 & -& 114.5 $\pm$ 3.0 & 1.0 $\pm$ 0.1 & 76.0 $\pm$ 1.6 & 80.7 $\pm$ 4.5\\ 
255 & NGC3184 -172.5-30.2 & 232.3 $\pm$ 1.8 & -& 324.4 $\pm$ 2.4 & 1.5 $\pm$ 0.3 & 43.4 $\pm$ 0.3 & 88.2 $\pm$ 1.2\\

\hline
\end{tabular}

\begin{tablenotes}
\centering
$^a$ Values normalized to I(H$\beta$)/100. 
\end{tablenotes}


\end{table*}
\newpage

==> Tables/Tabla_DHR_referencias.tex <==
\begin{table*}
\centering
    \caption{References to published data sets for objects in the DHR sub-sample of the present compilation.}
 \label{RefDHR-2}
\begin{tabular}{ccc}
\hline
ID  & Telescope+Instrument & Reference\\ \hline

1-2 & INT(2.5m)+IDS  & \citet{1987MNRAS.226...19D}\\ 
3 & INT(2.5m)+IDS  & \citet{1988MNRAS.235..633V}\\ 
4-7 & INT(2.5m)+IDS & \citet{1993MNRAS.260..177P}\\ 
8-12 & WHT(4.2m)+ISIS & \citet{1994ApJ...437..239G}\\
13 & MMT(4.5m, 6.5m)+ Blue Channel and Red Chanell Spectrograp & \citet{1994ApJ...426..123G}\\ 
14-16 & WHT(4.2m)+ISIS & \citet{1995ApJ...439..604G}\\ 
17-24 & INT(2.5m)+IDS and KPNO(2.1m)+ GoldCam CCD & \citet{1997ApJ...489...63G}\\ 
25-26 & WHT(4.2m)+ISIS & \citet{2000MNRAS.318..462D}\\ 
27-30 & WHT(4.2m)+ISIS & \citet{2002MNRAS.329..315C}\\ 
31-45 & MMT(4.5m, 6.5m)+ Blue Channel and Red Chanell Spectrograp & \citet{2003ApJ...591..801K}\\ 
46 & VLT(8.2m) + UVES & \citet{2003ApJ...584..735P}\\ 
47-52 & KeckI(10.0m)+LRIS & \citet{2004ApJ...615..228B}\\ 
53 & VLT(8.0m)+UVES & \citet{2004MNRAS.355..229E}\\ 
54 & VLT(8.0m)+UVES & \citet{2004ApJS..153..501G}\\ 
55-72 & KeckI(10.0m)+LRIS & \citet{2005AandA...441..981B}\\ 
73 & VLT(8.0m)+UVES & \citet{2005MNRAS.362..301G}\\ 
74-76 & VLT(8.0m)+UVES & \citet{2006MNRAS.368..253G}\\ 
77-78 & KeckI(10.0m)+LRIS & \citet{2007ApJ...656..186B}\\ 
79-80 & VLT(8.0m)+UVES & \citet{2007RMxAA..43....3G}\\ 
81-104 & VLT(8.0m)+FORS2 Multi-object & \citet{2009ApJ...700..309B}\\ 
105-109 & KeckI(10.0m)+LRIS & \citet{2012MNRAS.427.1463Z}\\ 
110-148 & LBT(8.4m)+MODS & \citet{2015ApJ...806...16B}\\ 
149-165 & LBT(8.4m)+MODS & \citet{2015ApJ...808...42C}\\ 
166-221 & LBT(8.4m)+MODS & \citet{2016ApJ...830....4C}\\ 
222-226 & VLT(8.2m) + UVES & \citet{2016MNRAS.458.1866T}\\ 
227-231 & WHT(4.2m)+ISIS & \citet{2017AandA...597A..84F}\\ 
232-239 & VLT(8.2m) + UVES & \citet{2017MNRAS.467.3759T}\\ 
240-255 & LBT(8.4m)+MODS & \citet{2020ApJ...893...96B}\\ 

 \hline     
\end{tabular}
\end{table*}
\newpage

==> Tables/Tabla_DHR_resultados_O.tex <==
\begin{table*}
\centering
\caption{Oxygen electron temperature and ionic abundances of objects in sub-sample DHR. Only objects with measured [ OIII] $\lambda$ 4363 \AA\ line intensities are listed.}
\label{OresDHR}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([OIII])$^a$ & 12+log(O$^{+}$/H$^{+}$)&	12+log(O$^{++}$/H$^{+}$) & 12+log(O/H)
\\ \hline


4 & 1.066 $\pm$ 0.079 & 7.72 $\pm$ 0.21 & 7.34 $\pm$ 0.09 & 7.87 $\pm$ 0.13\\ 
5 & 1.16 $\pm$ 0.103 & 8.15 $\pm$ 0.11 & 7.23 $\pm$ 0.09 & 8.19 $\pm$ 0.09\\ 
8 & 1.604 $\pm$ 0.02 & 6.75 $\pm$ 0.08 & 6.85 $\pm$ 0.01 & 7.1 $\pm$ 0.03\\ 
9 & 1.55 $\pm$ 0.044 & 7.05 $\pm$ 0.28 & 6.9 $\pm$ 0.03 & 7.28 $\pm$ 0.14\\ 
10 & 1.52 $\pm$ 0.013 & 6.77 $\pm$ 0.05 & 6.9 $\pm$ 0.01 & 7.14 $\pm$ 0.02\\ 
11 & 1.495 $\pm$ 0.028 & 6.63 $\pm$ 0.15 & 6.92 $\pm$ 0.02 & 7.1 $\pm$ 0.05\\ 
12 & 1.536 $\pm$ 0.111 & 6.52 $\pm$ 0.25 & 6.91 $\pm$ 0.06 & 7.06 $\pm$ 0.08\\ 
13 & 1.377 $\pm$ 0.063 & 7.18 $\pm$ 0.11 & 7.03 $\pm$ 0.05 & 7.41 $\pm$ 0.06\\ 
14 & 1.252 $\pm$ 0.053 & 8.47 $\pm$ 0.08 & 7.13 $\pm$ 0.04 & 8.49 $\pm$ 0.07\\ 
15 & 1.099 $\pm$ 0.051 & 7.6 $\pm$ 0.07 & 7.3 $\pm$ 0.05 & 7.78 $\pm$ 0.04\\ 
16 & 1.013 $\pm$ 0.057 & 7.82 $\pm$ 0.09 & 7.42 $\pm$ 0.07 & 7.96 $\pm$ 0.06\\ 
22 & 0.996 $\pm$ 0.052 & 8.09 $\pm$ 0.12 & 7.48 $\pm$ 0.08 & 8.19 $\pm$ 0.09\\ 
23 & 1.224 $\pm$ 0.073 & 8.04 $\pm$ 0.17 & 7.2 $\pm$ 0.07 & 8.1 $\pm$ 0.13\\ 
24 & 1.227 $\pm$ 0.08 & 7.94 $\pm$ 0.21 & 7.19 $\pm$ 0.08 & 8.02 $\pm$ 0.15\\ 
30 & 1.004 $\pm$ 0.047 & 7.9 $\pm$ 0.07 & 7.43 $\pm$ 0.06 & 8.03 $\pm$ 0.05\\ 
32 & 0.91 $\pm$ 0.016 & 8.33 $\pm$ 0.06 & 7.6 $\pm$ 0.03 & 8.4 $\pm$ 0.05\\ 
33 & 0.986 $\pm$ 0.048 & 7.98 $\pm$ 0.1 & 7.48 $\pm$ 0.06 & 8.1 $\pm$ 0.07\\ 
34 & 1.07 $\pm$ 0.039 & 8.57 $\pm$ 0.09 & 7.36 $\pm$ 0.05 & 8.6 $\pm$ 0.07\\ 
35 & 1.008 $\pm$ 0.032 & 8.07 $\pm$ 0.06 & 7.44 $\pm$ 0.05 & 8.16 $\pm$ 0.05\\ 
36 & 1.149 $\pm$ 0.03 & 7.73 $\pm$ 0.07 & 7.26 $\pm$ 0.04 & 7.86 $\pm$ 0.05\\ 
37 & 0.906 $\pm$ 0.024 & 8.08 $\pm$ 0.07 & 7.62 $\pm$ 0.05 & 8.21 $\pm$ 0.05\\ 
38 & 1.075 $\pm$ 0.053 & 8.11 $\pm$ 0.11 & 7.35 $\pm$ 0.06 & 8.18 $\pm$ 0.09\\ 
39 & 0.97 $\pm$ 0.048 & 8.11 $\pm$ 0.07 & 7.5 $\pm$ 0.07 & 8.2 $\pm$ 0.05\\ 
40 & 0.996 $\pm$ 0.024 & 8.72 $\pm$ 0.1 & 7.46 $\pm$ 0.04 & 8.74 $\pm$ 0.08\\ 
41 & 1.16 $\pm$ 0.029 & 7.98 $\pm$ 0.07 & 7.25 $\pm$ 0.03 & 8.05 $\pm$ 0.05\\ 
42 & 1.332 $\pm$ 0.039 & 7.21 $\pm$ 0.17 & 7.07 $\pm$ 0.04 & 7.45 $\pm$ 0.09\\ 
43 & 1.404 $\pm$ 0.048 & 7.46 $\pm$ 0.07 & 7.01 $\pm$ 0.04 & 7.59 $\pm$ 0.05\\ 
44 & 1.265 $\pm$ 0.036 & 7.77 $\pm$ 0.07 & 7.13 $\pm$ 0.04 & 7.86 $\pm$ 0.06\\ 
45 & 1.298 $\pm$ 0.036 & 7.72 $\pm$ 0.07 & 7.1 $\pm$ 0.04 & 7.82 $\pm$ 0.05\\ 
46 & 0.999 $\pm$ 0.004 & 7.65 $\pm$ 0.02 & 7.44 $\pm$ 0.01 & 7.85 $\pm$ 0.01\\ 
53 & 0.85 $\pm$ 0.003 & 7.53 $\pm$ 0.12 & 7.69 $\pm$ 0.01 & 7.92 $\pm$ 0.04\\ 
54 & 0.863 $\pm$ 0.003 & 7.96 $\pm$ 0.09 & 7.67 $\pm$ 0.01 & 8.14 $\pm$ 0.05\\ 
73 & 0.911 $\pm$ 0.009 & 8.27 $\pm$ 0.05 & 7.59 $\pm$ 0.02 & 8.35 $\pm$ 0.04\\ 
74 & 0.768 $\pm$ 0.014 & 8.37 $\pm$ 0.06 & 7.88 $\pm$ 0.03 & 8.49 $\pm$ 0.05\\ 
75 & 0.921 $\pm$ 0.011 & 7.59 $\pm$ 0.08 & 7.57 $\pm$ 0.02 & 7.88 $\pm$ 0.04\\ 
76 & 0.787 $\pm$ 0.021 & 8.47 $\pm$ 0.05 & 7.84 $\pm$ 0.04 & 8.56 $\pm$ 0.04\\ 
78 & 0.773 $\pm$ 0.021 & 8.49 $\pm$ 0.13 & 7.88 $\pm$ 0.05 & 8.58 $\pm$ 0.1\\ 
79 & 0.821 $\pm$ 0.008 & 8.09 $\pm$ 0.05 & 7.77 $\pm$ 0.02 & 8.25 $\pm$ 0.03\\ 
80 & 0.811 $\pm$ 0.009 & 7.98 $\pm$ 0.06 & 7.79 $\pm$ 0.02 & 8.19 $\pm$ 0.03\\ 
81 & 1.194 $\pm$ 0.034 & 7.47 $\pm$ 0.09 & 7.21 $\pm$ 0.04 & 7.66 $\pm$ 0.06\\ 
82 & 1.091 $\pm$ 0.03 & 7.81 $\pm$ 0.09 & 7.33 $\pm$ 0.04 & 7.93 $\pm$ 0.06\\ 
83 & 0.933 $\pm$ 0.028 & 8.25 $\pm$ 0.1 & 7.56 $\pm$ 0.05 & 8.33 $\pm$ 0.08\\ 
84 & 0.926 $\pm$ 0.024 & 7.88 $\pm$ 0.11 & 7.58 $\pm$ 0.04 & 8.06 $\pm$ 0.07\\ 
85 & 0.957 $\pm$ 0.028 & 8.07 $\pm$ 0.09 & 7.52 $\pm$ 0.04 & 8.18 $\pm$ 0.07\\ 
86 & 0.875 $\pm$ 0.017 & 8.2 $\pm$ 0.07 & 7.67 $\pm$ 0.04 & 8.31 $\pm$ 0.05\\ 
87 & 0.879 $\pm$ 0.016 & 8.19 $\pm$ 0.07 & 7.66 $\pm$ 0.04 & 8.3 $\pm$ 0.05\\ 
88 & 0.965 $\pm$ 0.036 & 8.1 $\pm$ 0.09 & 7.51 $\pm$ 0.05 & 8.2 $\pm$ 0.06\\ 
91 & 0.896 $\pm$ 0.017 & 8.23 $\pm$ 0.07 & 7.63 $\pm$ 0.04 & 8.33 $\pm$ 0.06\\ 
94 & 0.94 $\pm$ 0.02 & 8.15 $\pm$ 0.08 & 7.55 $\pm$ 0.04 & 8.24 $\pm$ 0.06\\ 
96 & 0.801 $\pm$ 0.127 & 8.24 $\pm$ 0.07 & 7.82 $\pm$ 0.24 & 8.38 $\pm$ 0.08\\ 
97 & 1.026 $\pm$ 0.026 & 8.13 $\pm$ 0.07 & 7.42 $\pm$ 0.04 & 8.21 $\pm$ 0.06\\ 
100 & 0.836 $\pm$ 0.021 & 8.19 $\pm$ 0.08 & 7.74 $\pm$ 0.04 & 8.32 $\pm$ 0.06\\ 
102 & 0.92 $\pm$ 0.018 & 7.98 $\pm$ 0.07 & 7.59 $\pm$ 0.04 & 8.13 $\pm$ 0.05\\ 
103 & 1.11 $\pm$ 0.029 & 7.87 $\pm$ 0.08 & 7.31 $\pm$ 0.04 & 7.98 $\pm$ 0.06\\ 
104 & 1.062 $\pm$ 0.025 & 7.99 $\pm$ 0.11 & 7.37 $\pm$ 0.04 & 8.08 $\pm$ 0.08\\ 
106 & 0.82 $\pm$ 0.017 & 8.08 $\pm$ 0.12 & 7.78 $\pm$ 0.04 & 8.26 $\pm$ 0.08\\ 
107 & 0.946 $\pm$ 0.016 & 7.87 $\pm$ 0.09 & 7.54 $\pm$ 0.03 & 8.04 $\pm$ 0.06\\ 
108 & 0.959 $\pm$ 0.025 & 7.97 $\pm$ 0.09 & 7.53 $\pm$ 0.05 & 8.11 $\pm$ 0.06\\ 
109 & 0.901 $\pm$ 0.015 & 7.69 $\pm$ 0.11 & 7.62 $\pm$ 0.03 & 7.96 $\pm$ 0.06\\  
123 & 1.083 $\pm$ 0.038 & 8.74 $\pm$ 0.08 & 7.33 $\pm$ 0.04 & 8.75 $\pm$ 0.07\\ 



 \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([OIII])$^a$ & 12+log(O$^{+}$/H$^{+}$)&	12+log(O$^{++}$/H$^{+}$) & 12+log(O/H)
\\ \hline



127 & 0.934 $\pm$ 0.047 & 8.55 $\pm$ 0.1 & 7.55 $\pm$ 0.07 & 8.59 $\pm$ 0.08\\ 
133 & 1.016 $\pm$ 0.049 & 8.56 $\pm$ 0.07 & 7.42 $\pm$ 0.06 & 8.59 $\pm$ 0.06\\ 
137 & 0.978 $\pm$ 0.043 & 8.58 $\pm$ 0.09 & 7.48 $\pm$ 0.06 & 8.61 $\pm$ 0.08\\ 
138 & 0.859 $\pm$ 0.031 & 8.41 $\pm$ 0.06 & 7.68 $\pm$ 0.05 & 8.48 $\pm$ 0.05\\ 
139 & 0.915 $\pm$ 0.03 & 8.67 $\pm$ 0.13 & 7.58 $\pm$ 0.04 & 8.7 $\pm$ 0.11\\ 
140 & 0.957 $\pm$ 0.029 & 8.76 $\pm$ 0.06 & 7.51 $\pm$ 0.04 & 8.78 $\pm$ 0.05\\ 
141 & 0.843 $\pm$ 0.016 & 8.34 $\pm$ 0.17 & 7.71 $\pm$ 0.03 & 8.43 $\pm$ 0.12\\ 
142 & 0.896 $\pm$ 0.028 & 8.47 $\pm$ 0.06 & 7.61 $\pm$ 0.04 & 8.53 $\pm$ 0.05\\ 
143 & 1.03 $\pm$ 0.085 & 8.4 $\pm$ 0.2 & 7.4 $\pm$ 0.1 & 8.44 $\pm$ 0.15\\ 
144 & 1.009 $\pm$ 0.08 & 8.45 $\pm$ 0.2 & 7.43 $\pm$ 0.1 & 8.49 $\pm$ 0.15\\ 
145 & 1.176 $\pm$ 0.077 & 8.11 $\pm$ 0.13 & 7.21 $\pm$ 0.07 & 8.16 $\pm$ 0.1\\ 
146 & 1.194 $\pm$ 0.074 & 8.05 $\pm$ 0.14 & 7.19 $\pm$ 0.07 & 8.11 $\pm$ 0.11\\ 
147 & 1.027 $\pm$ 0.018 & 7.91 $\pm$ 0.05 & 7.4 $\pm$ 0.02 & 8.03 $\pm$ 0.04\\ 
148 & 1.064 $\pm$ 0.015 & 7.68 $\pm$ 0.05 & 7.35 $\pm$ 0.02 & 7.85 $\pm$ 0.03\\ 
169 & 0.742 $\pm$ 0.019 & 8.66 $\pm$ 0.04 & 7.95 $\pm$ 0.04 & 8.74 $\pm$ 0.03\\ 
182 & 0.859 $\pm$ 0.022 & 7.98 $\pm$ 0.07 & 7.68 $\pm$ 0.04 & 8.16 $\pm$ 0.05\\ 
183 & 1.546 $\pm$ 0.036 & 7.8 $\pm$ 0.05 & 6.89 $\pm$ 0.02 & 7.85 $\pm$ 0.04\\ 
184 & 1.025 $\pm$ 0.055 & 8.54 $\pm$ 0.11 & 7.41 $\pm$ 0.06 & 8.57 $\pm$ 0.09\\ 
186 & 0.927 $\pm$ 0.012 & 8.07 $\pm$ 0.05 & 7.56 $\pm$ 0.02 & 8.18 $\pm$ 0.04\\ 
187 & 0.972 $\pm$ 0.029 & 8.14 $\pm$ 0.16 & 7.48 $\pm$ 0.04 & 8.23 $\pm$ 0.11\\ 
190 & 1.058 $\pm$ 0.027 & 8.38 $\pm$ 0.17 & 7.36 $\pm$ 0.03 & 8.42 $\pm$ 0.13\\ 
191 & 0.632 $\pm$ 0.049 & 8.51 $\pm$ 0.08 & 8.27 $\pm$ 0.15 & 8.71 $\pm$ 0.07\\ 
192 & 0.983 $\pm$ 0.009 & 7.68 $\pm$ 0.08 & 7.47 $\pm$ 0.01 & 7.89 $\pm$ 0.05\\ 
193 & 0.765 $\pm$ 0.012 & 8.49 $\pm$ 0.1 & 7.89 $\pm$ 0.03 & 8.59 $\pm$ 0.07\\ 
194 & 1.098 $\pm$ 0.01 & 7.87 $\pm$ 0.05 & 7.31 $\pm$ 0.01 & 7.98 $\pm$ 0.04\\ 
195 & 1.098 $\pm$ 0.024 & 8.53 $\pm$ 0.11 & 7.31 $\pm$ 0.03 & 8.56 $\pm$ 0.09\\ 
196 & 0.622 $\pm$ 0.042 & 8.42 $\pm$ 0.15 & 8.31 $\pm$ 0.13 & 8.67 $\pm$ 0.09\\ 
197 & 1.14 $\pm$ 0.014 & 8.24 $\pm$ 0.09 & 7.26 $\pm$ 0.02 & 8.29 $\pm$ 0.08\\ 
198 & 0.936 $\pm$ 0.02 & 8.07 $\pm$ 0.17 & 7.54 $\pm$ 0.03 & 8.19 $\pm$ 0.11\\ 
199 & 1.069 $\pm$ 0.01 & 8.05 $\pm$ 0.07 & 7.34 $\pm$ 0.01 & 8.13 $\pm$ 0.06\\ 
200 & 0.78 $\pm$ 0.006 & 8.39 $\pm$ 0.08 & 7.85 $\pm$ 0.01 & 8.5 $\pm$ 0.06\\ 
201 & 1.581 $\pm$ 0.111 & 7.97 $\pm$ 0.2 & 6.91 $\pm$ 0.08 & 8.0 $\pm$ 0.16\\ 
203 & 0.87 $\pm$ 0.009 & 8.64 $\pm$ 0.11 & 7.66 $\pm$ 0.02 & 8.69 $\pm$ 0.09\\ 
204 & 1.296 $\pm$ 0.014 & 8.21 $\pm$ 0.05 & 7.09 $\pm$ 0.01 & 8.25 $\pm$ 0.04\\ 
205 & 0.989 $\pm$ 0.016 & 7.77 $\pm$ 0.09 & 7.46 $\pm$ 0.02 & 7.95 $\pm$ 0.06\\ 
206 & 1.236 $\pm$ 0.018 & 7.63 $\pm$ 0.13 & 7.15 $\pm$ 0.02 & 7.75 $\pm$ 0.09\\ 
207 & 0.737 $\pm$ 0.02 & 7.69 $\pm$ 0.14 & 7.96 $\pm$ 0.05 & 8.15 $\pm$ 0.05\\ 
208 & 0.904 $\pm$ 0.005 & 7.53 $\pm$ 0.05 & 7.6 $\pm$ 0.01 & 7.87 $\pm$ 0.02\\ 
209 & 0.889 $\pm$ 0.005 & 7.45 $\pm$ 0.04 & 7.63 $\pm$ 0.01 & 7.85 $\pm$ 0.02\\ 
210 & 1.097 $\pm$ 0.009 & 7.61 $\pm$ 0.08 & 7.31 $\pm$ 0.01 & 7.78 $\pm$ 0.05\\ 
211 & 1.087 $\pm$ 0.009 & 7.52 $\pm$ 0.04 & 7.32 $\pm$ 0.01 & 7.74 $\pm$ 0.02\\ 
212 & 1.148 $\pm$ 0.017 & 7.55 $\pm$ 0.14 & 7.25 $\pm$ 0.02 & 7.72 $\pm$ 0.08\\ 
213 & 1.246 $\pm$ 0.018 & 7.47 $\pm$ 0.2 & 7.14 $\pm$ 0.02 & 7.64 $\pm$ 0.12\\ 
214 & 1.014 $\pm$ 0.009 & 7.45 $\pm$ 0.09 & 7.42 $\pm$ 0.01 & 7.74 $\pm$ 0.05\\ 
215 & 1.076 $\pm$ 0.012 & 7.85 $\pm$ 0.2 & 7.34 $\pm$ 0.02 & 7.96 $\pm$ 0.13\\ 
216 & 1.328 $\pm$ 0.015 & 7.9 $\pm$ 0.09 & 7.06 $\pm$ 0.01 & 7.96 $\pm$ 0.08\\ 
217 & 1.081 $\pm$ 0.01 & 7.87 $\pm$ 0.08 & 7.33 $\pm$ 0.01 & 7.98 $\pm$ 0.06\\ 
218 & 1.195 $\pm$ 0.016 & 7.99 $\pm$ 0.23 & 7.2 $\pm$ 0.02 & 8.05 $\pm$ 0.16\\ 
219 & 1.124 $\pm$ 0.009 & 7.49 $\pm$ 0.07 & 7.28 $\pm$ 0.01 & 7.7 $\pm$ 0.04\\ 
220 & 2.0 $\pm$ 0.024 & 7.39 $\pm$ 0.05 & 6.64 $\pm$ 0.01 & 7.46 $\pm$ 0.04\\ 
221 & 1.696 $\pm$ 0.046 & 7.28 $\pm$ 0.17 & 6.8 $\pm$ 0.02 & 7.4 $\pm$ 0.11\\ 
222 & 0.809 $\pm$ 0.033 & 8.19 $\pm$ 0.13 & 7.81 $\pm$ 0.07 & 8.34 $\pm$ 0.08\\ 
223 & 0.795 $\pm$ 0.032 & 8.23 $\pm$ 0.13 & 7.84 $\pm$ 0.07 & 8.38 $\pm$ 0.09\\ 
224 & 0.896 $\pm$ 0.023 & 8.02 $\pm$ 0.13 & 7.63 $\pm$ 0.05 & 8.17 $\pm$ 0.08\\ 
225 & 0.96 $\pm$ 0.056 & 7.84 $\pm$ 0.19 & 7.51 $\pm$ 0.08 & 8.0 $\pm$ 0.12\\ 
226 & 1.155 $\pm$ 0.046 & 7.45 $\pm$ 0.17 & 7.26 $\pm$ 0.05 & 7.66 $\pm$ 0.1\\ 
227 & 1.133 $\pm$ 0.044 & 7.41 $\pm$ 0.06 & 7.26 $\pm$ 0.04 & 7.64 $\pm$ 0.04\\ 



 \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([OIII])$^a$ & 12+log(O$^{+}$/H$^{+}$)&	12+log(O$^{++}$/H$^{+}$) & 12+log(O/H)
\\ \hline




228 & -& 8.63 $\pm$ 0.1 & -& -\\ 
229 & 0.919 $\pm$ 0.025 & 8.47 $\pm$ 0.04 & 7.57 $\pm$ 0.04 & 8.52 $\pm$ 0.04\\ 
230 & 0.943 $\pm$ 0.014 & 8.41 $\pm$ 0.02 & 7.52 $\pm$ 0.02 & 8.46 $\pm$ 0.02\\ 
231 & 1.207 $\pm$ 0.036 & 7.86 $\pm$ 0.07 & 7.18 $\pm$ 0.03 & 7.94 $\pm$ 0.06\\ 
233 & 1.001 $\pm$ 0.004 & 7.89 $\pm$ 0.03 & 7.43 $\pm$ 0.01 & 8.02 $\pm$ 0.02\\ 
233 & 1.139 $\pm$ 0.026 & 7.11 $\pm$ 0.09 & 7.26 $\pm$ 0.03 & 7.49 $\pm$ 0.04\\ 
234 & 0.933 $\pm$ 0.011 & 8.47 $\pm$ 0.06 & 7.56 $\pm$ 0.02 & 8.52 $\pm$ 0.05\\ 
235 & 0.93 $\pm$ 0.008 & 7.94 $\pm$ 0.07 & 7.55 $\pm$ 0.01 & 8.09 $\pm$ 0.04\\ 
236 & 0.97 $\pm$ 0.012 & 8.12 $\pm$ 0.05 & 7.5 $\pm$ 0.02 & 8.21 $\pm$ 0.04\\ 
237 & 1.254 $\pm$ 0.019 & 7.66 $\pm$ 0.08 & 7.13 $\pm$ 0.02 & 7.77 $\pm$ 0.06\\ 
238 & 1.287 $\pm$ 0.008 & 7.02 $\pm$ 0.07 & 7.1 $\pm$ 0.01 & 7.36 $\pm$ 0.03\\ 
239 & 1.504 $\pm$ 0.055 & 6.62 $\pm$ 0.18 & 6.92 $\pm$ 0.03 & 7.1 $\pm$ 0.06\\





 

 





 
 

 
 
 



\hline

\end{tabular}
\begin{tablenotes}

$^a$ In units of 10$^{4}$K.\\
    
\end{tablenotes}
\end{table*}
\newpage

==> Tables/Tabla_DHR_resultados_S.tex <==
\begin{table*}
\centering
\caption{Sulphur electron temperature and ionic abundances of objects in sub-sample DHR.}
\label{ResHDR}
\begin{tabular}{ccccc}
\hline

ID & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) & 12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline



1 & 0.700 $\pm$ 0.074 & 6.22 $\pm$ 0.14 & 7.13 $\pm$ 0.1 & 7.18 $\pm$ 0.08\\ 
2 & 0.734 $\pm$ 0.072 & 6.49 $\pm$ 0.12 & 7.09 $\pm$ 0.09 & 7.19 $\pm$ 0.07\\ 
3 & 0.724 $\pm$ 0.035 & 6.2 $\pm$ 0.06 & 6.99 $\pm$ 0.04 & 7.05 $\pm$ 0.04\\ 
4 & 1.132 $\pm$ 0.158 & 5.96 $\pm$ 0.11 & 6.19 $\pm$ 0.09 & 6.39 $\pm$ 0.06\\ 
5 & 0.941 $\pm$ 0.056 & 6.21 $\pm$ 0.06 & 6.63 $\pm$ 0.04 & 6.77 $\pm$ 0.03\\ 
6 & 0.967 $\pm$ 0.209 & 6.23 $\pm$ 0.2 & 6.58 $\pm$ 0.15 & 6.74 $\pm$ 0.11\\ 
7 & 0.921 $\pm$ 0.17 & 6.42 $\pm$ 0.18 & 6.57 $\pm$ 0.13 & 6.8 $\pm$ 0.1\\ 
8 & 1.278 $\pm$ 0.078 & 4.98 $\pm$ 0.05 & 5.96 $\pm$ 0.04 & 6.0 $\pm$ 0.03\\ 
9 & 1.518 $\pm$ 0.379 & 5.35 $\pm$ 0.16 & 5.93 $\pm$ 0.14 & 6.03 $\pm$ 0.1\\ 
10 & 1.575 $\pm$ 0.071 & 5.08 $\pm$ 0.03 & 5.88 $\pm$ 0.03 & 5.95 $\pm$ 0.02\\ 
11 & 1.544 $\pm$ 0.209 & 4.96 $\pm$ 0.08 & 5.86 $\pm$ 0.1 & 5.91 $\pm$ 0.08\\ 
12 & 1.485 $\pm$ 0.335 & 4.92 $\pm$ 0.15 & 5.94 $\pm$ 0.16 & 5.98 $\pm$ 0.13\\ 
13 & 1.614 $\pm$ 0.169 & 5.39 $\pm$ 0.08 & 5.85 $\pm$ 0.08 & 5.98 $\pm$ 0.06\\ 
14 & 0.769 $\pm$ 0.029 & 6.59 $\pm$ 0.04 & 6.83 $\pm$ 0.03 & 7.03 $\pm$ 0.03\\ 
15 & 1.198 $\pm$ 0.057 & 5.94 $\pm$ 0.04 & 6.2 $\pm$ 0.04 & 6.39 $\pm$ 0.03\\ 
16 & 1.092 $\pm$ 0.055 & 6.06 $\pm$ 0.07 & 6.21 $\pm$ 0.03 & 6.45 $\pm$ 0.03\\ 
17 & 0.862 $\pm$ 0.09 & 6.25 $\pm$ 0.14 & 6.71 $\pm$ 0.09 & 6.84 $\pm$ 0.07\\ 
18 & 0.619 $\pm$ 0.029 & 6.59 $\pm$ 0.07 & 7.15 $\pm$ 0.06 & 7.25 $\pm$ 0.05\\ 
19 & 0.726 $\pm$ 0.029 & 6.28 $\pm$ 0.05 & 6.92 $\pm$ 0.04 & 7.01 $\pm$ 0.03\\ 
20 & 0.898 $\pm$ 0.037 & 6.12 $\pm$ 0.04 & 6.62 $\pm$ 0.04 & 6.74 $\pm$ 0.03\\ 
21 & 0.828 $\pm$ 0.073 & 6.15 $\pm$ 0.1 & 6.75 $\pm$ 0.1 & 6.85 $\pm$ 0.07\\ 
22 & 0.898 $\pm$ 0.038 & 6.03 $\pm$ 0.04 & 6.66 $\pm$ 0.04 & 6.75 $\pm$ 0.03\\ 
23 & 0.915 $\pm$ 0.083 & 6.11 $\pm$ 0.09 & 6.62 $\pm$ 0.09 & 6.74 $\pm$ 0.07\\ 
24 & 0.992 $\pm$ 0.124 & 5.97 $\pm$ 0.12 & 6.59 $\pm$ 0.14 & 6.68 $\pm$ 0.1\\ 
25 & 0.761 $\pm$ 0.025 & 6.39 $\pm$ 0.04 & 6.91 $\pm$ 0.03 & 7.02 $\pm$ 0.02\\ 
26 & 0.785 $\pm$ 0.038 & 6.48 $\pm$ 0.06 & 6.72 $\pm$ 0.05 & 6.92 $\pm$ 0.04\\ 
27 & 0.726 $\pm$ 0.029 & 6.58 $\pm$ 0.05 & 6.92 $\pm$ 0.04 & 7.08 $\pm$ 0.03\\ 
28 & 0.710 $\pm$ 0.026 & 6.57 $\pm$ 0.05 & 6.98 $\pm$ 0.04 & 7.12 $\pm$ 0.03\\ 
29 & 0.570 $\pm$ 0.046 & 6.98 $\pm$ 0.13 & 7.11 $\pm$ 0.09 & 7.35 $\pm$ 0.07\\ 
30 & 1.053 $\pm$ 0.048 & 5.89 $\pm$ 0.04 & 6.35 $\pm$ 0.04 & 6.48 $\pm$ 0.03\\ 
31 & 0.668 $\pm$ 0.019 & 6.38 $\pm$ 0.04 & 7.21 $\pm$ 0.04 & 7.27 $\pm$ 0.03\\ 
32 & 0.776 $\pm$ 0.021 & 6.09 $\pm$ 0.04 & 7.02 $\pm$ 0.03 & 7.07 $\pm$ 0.03\\ 
33 & 0.922 $\pm$ 0.051 & 5.97 $\pm$ 0.06 & 6.73 $\pm$ 0.05 & 6.8 $\pm$ 0.04\\ 
34 & 0.768 $\pm$ 0.029 & 6.48 $\pm$ 0.05 & 7.16 $\pm$ 0.04 & 7.24 $\pm$ 0.03\\ 
35 & 0.845 $\pm$ 0.026 & 5.96 $\pm$ 0.04 & 6.88 $\pm$ 0.03 & 6.93 $\pm$ 0.03\\ 
36 & 0.987 $\pm$ 0.036 & 5.69 $\pm$ 0.04 & 6.6 $\pm$ 0.03 & 6.65 $\pm$ 0.03\\ 
37 & 0.827 $\pm$ 0.027 & 5.99 $\pm$ 0.04 & 6.87 $\pm$ 0.03 & 6.92 $\pm$ 0.03\\ 
38 & 0.886 $\pm$ 0.052 & 6.14 $\pm$ 0.06 & 6.75 $\pm$ 0.05 & 6.85 $\pm$ 0.04\\ 
39 & 0.88 $\pm$ 0.029 & 6.12 $\pm$ 0.04 & 6.77 $\pm$ 0.03 & 6.86 $\pm$ 0.03\\ 
40 & 0.683 $\pm$ 0.027 & 6.38 $\pm$ 0.06 & 7.02 $\pm$ 0.04 & 7.11 $\pm$ 0.04\\ 
41 & 0.968 $\pm$ 0.036 & 5.86 $\pm$ 0.05 & 6.66 $\pm$ 0.04 & 6.72 $\pm$ 0.03\\ 
42 & 1.218 $\pm$ 0.152 & 5.4 $\pm$ 0.1 & 6.29 $\pm$ 0.08 & 6.34 $\pm$ 0.06\\ 
43 & 1.266 $\pm$ 0.062 & 5.9 $\pm$ 0.04 & 6.17 $\pm$ 0.04 & 6.36 $\pm$ 0.03\\ 
44 & 0.997 $\pm$ 0.043 & 6.46 $\pm$ 0.04 & 6.49 $\pm$ 0.04 & 6.78 $\pm$ 0.03\\ 
45 & 0.969 $\pm$ 0.038 & 5.75 $\pm$ 0.04 & 6.58 $\pm$ 0.04 & 6.64 $\pm$ 0.03\\ 
46 & 0.986 $\pm$ 0.012 & 5.55 $\pm$ 0.01 & 6.65 $\pm$ 0.01 & 6.68 $\pm$ 0.01\\ 
47 & 0.641 $\pm$ 0.025 & 6.65 $\pm$ 0.06 & 6.91 $\pm$ 0.08 & 7.1 $\pm$ 0.05\\ 
48 & 0.637 $\pm$ 0.035 & 6.61 $\pm$ 0.08 & 6.94 $\pm$ 0.1 & 7.11 $\pm$ 0.07\\ 
49 & 0.706 $\pm$ 0.038 & 6.64 $\pm$ 0.08 & 6.79 $\pm$ 0.09 & 7.02 $\pm$ 0.06\\ 
50 & 0.615 $\pm$ 0.023 & 6.67 $\pm$ 0.06 & 7.06 $\pm$ 0.08 & 7.2 $\pm$ 0.06\\ 
51 & 0.677 $\pm$ 0.046 & 6.56 $\pm$ 0.09 & 6.76 $\pm$ 0.11 & 6.97 $\pm$ 0.07\\ 
52 & 0.58 $\pm$ 0.026 & 6.82 $\pm$ 0.08 & 6.96 $\pm$ 0.1 & 7.19 $\pm$ 0.06\\ 
53 & 0.958 $\pm$ 0.063 & 5.18 $\pm$ 0.07 & 6.72 $\pm$ 0.08 & 6.73 $\pm$ 0.07\\ 
54 & 0.856 $\pm$ 0.037 & 5.7 $\pm$ 0.05 & 6.87 $\pm$ 0.06 & 6.9 $\pm$ 0.05\\ 
55 & 1.061 $\pm$ 0.127 & 5.7 $\pm$ 0.11 & 6.43 $\pm$ 0.11 & 6.5 $\pm$ 0.09\\ 
56 & 0.71 $\pm$ 0.045 & 6.6 $\pm$ 0.09 & 6.95 $\pm$ 0.1 & 7.11 $\pm$ 0.07\\ 
57 & 0.67 $\pm$ 0.064 & 6.71 $\pm$ 0.13 & 6.86 $\pm$ 0.11 & 7.09 $\pm$ 0.08\\ 
58 & 0.822 $\pm$ 0.073 & 6.52 $\pm$ 0.1 & 6.67 $\pm$ 0.11 & 6.91 $\pm$ 0.07\\ 
59 & 0.66 $\pm$ 0.053 & 6.76 $\pm$ 0.11 & 6.85 $\pm$ 0.11 & 7.11 $\pm$ 0.07\\ 
60 & 0.759 $\pm$ 0.065 & 6.48 $\pm$ 0.11 & 6.76 $\pm$ 0.11 & 6.94 $\pm$ 0.07\\ 

 

\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) & 12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline   
 
61 & 0.702 $\pm$ 0.078 & 6.63 $\pm$ 0.15 & 6.75 $\pm$ 0.13 & 6.99 $\pm$ 0.09\\ 
62 & 0.739 $\pm$ 0.049 & 6.52 $\pm$ 0.09 & 7.03 $\pm$ 0.1 & 7.15 $\pm$ 0.07\\ 
63 & 0.815 $\pm$ 0.113 & 6.28 $\pm$ 0.16 & 6.68 $\pm$ 0.14 & 6.83 $\pm$ 0.1\\ 
64 & 0.787 $\pm$ 0.066 & 6.49 $\pm$ 0.11 & 6.85 $\pm$ 0.1 & 7.01 $\pm$ 0.07\\ 
65 & 0.673 $\pm$ 0.041 & 6.72 $\pm$ 0.09 & 7.02 $\pm$ 0.1 & 7.2 $\pm$ 0.07\\ 
66 & 0.751 $\pm$ 0.051 & 6.31 $\pm$ 0.11 & 6.97 $\pm$ 0.1 & 7.05 $\pm$ 0.08\\ 
67 & 0.711 $\pm$ 0.053 & 6.58 $\pm$ 0.1 & 6.92 $\pm$ 0.11 & 7.08 $\pm$ 0.07\\ 
68 & 0.573 $\pm$ 0.034 & 6.88 $\pm$ 0.1 & 7.24 $\pm$ 0.1 & 7.4 $\pm$ 0.07\\ 
69 & 0.72 $\pm$ 0.048 & 6.45 $\pm$ 0.09 & 6.96 $\pm$ 0.1 & 7.07 $\pm$ 0.07\\ 
70 & 0.667 $\pm$ 0.056 & 6.62 $\pm$ 0.12 & 7.01 $\pm$ 0.11 & 7.16 $\pm$ 0.08\\ 
71 & 0.486 $\pm$ 0.034 & 7.26 $\pm$ 0.13 & 7.68 $\pm$ 0.12 & 7.82 $\pm$ 0.08\\ 
72 & 0.557 $\pm$ 0.031 & 6.93 $\pm$ 0.1 & 7.43 $\pm$ 0.1 & 7.55 $\pm$ 0.07\\ 
73 & 0.909 $\pm$ 0.023 & 6.21 $\pm$ 0.03 & 6.68 $\pm$ 0.03 & 6.81 $\pm$ 0.02\\ 
74 & 0.822 $\pm$ 0.025 & 6.35 $\pm$ 0.04 & 6.78 $\pm$ 0.04 & 6.92 $\pm$ 0.03\\ 
75 & 0.884 $\pm$ 0.035 & 5.26 $\pm$ 0.05 & 6.88 $\pm$ 0.05 & 6.89 $\pm$ 0.04\\ 
76 & 0.81 $\pm$ 0.019 & 6.31 $\pm$ 0.03 & 6.78 $\pm$ 0.03 & 6.91 $\pm$ 0.02\\ 
77 & 0.714 $\pm$ 0.059 & 6.53 $\pm$ 0.11 & 6.55 $\pm$ 0.11 & 6.84 $\pm$ 0.07\\ 
78 & 0.75 $\pm$ 0.045 & 6.23 $\pm$ 0.08 & 6.88 $\pm$ 0.1 & 6.96 $\pm$ 0.07\\ 
79 & 0.888 $\pm$ 0.017 & 5.86 $\pm$ 0.02 & 6.73 $\pm$ 0.02 & 6.79 $\pm$ 0.02\\ 
80 & 0.791 $\pm$ 0.02 & 5.63 $\pm$ 0.04 & 6.94 $\pm$ 0.04 & 6.96 $\pm$ 0.03\\ 
81 & 1.175 $\pm$ 0.069 & 5.48 $\pm$ 0.05 & 6.36 $\pm$ 0.05 & 6.41 $\pm$ 0.04\\ 
82 & 1.103 $\pm$ 0.063 & 5.82 $\pm$ 0.05 & 6.43 $\pm$ 0.05 & 6.53 $\pm$ 0.04\\ 
83 & 0.882 $\pm$ 0.045 & 6.27 $\pm$ 0.06 & 6.75 $\pm$ 0.05 & 6.87 $\pm$ 0.04\\ 
84 & 0.998 $\pm$ 0.06 & 5.99 $\pm$ 0.06 & 6.51 $\pm$ 0.05 & 6.63 $\pm$ 0.04\\ 
85 & 0.972 $\pm$ 0.048 & 6.08 $\pm$ 0.05 & 6.54 $\pm$ 0.04 & 6.67 $\pm$ 0.03\\ 
86 & 0.808 $\pm$ 0.026 & 6.17 $\pm$ 0.04 & 6.85 $\pm$ 0.04 & 6.93 $\pm$ 0.03\\ 
87 & 0.821 $\pm$ 0.027 & 5.85 $\pm$ 0.04 & 6.82 $\pm$ 0.04 & 6.86 $\pm$ 0.03\\ 
88 & 0.919 $\pm$ 0.042 & 6.12 $\pm$ 0.05 & 6.66 $\pm$ 0.04 & 6.77 $\pm$ 0.03\\ 
89 & 0.76 $\pm$ 0.025 & 6.6 $\pm$ 0.04 & 6.82 $\pm$ 0.04 & 7.03 $\pm$ 0.03\\ 
90 & 0.87 $\pm$ 0.035 & 6.13 $\pm$ 0.05 & 6.66 $\pm$ 0.04 & 6.78 $\pm$ 0.03\\ 
91 & 0.858 $\pm$ 0.03 & 6.2 $\pm$ 0.04 & 6.82 $\pm$ 0.04 & 6.91 $\pm$ 0.03\\ 
92 & 0.802 $\pm$ 0.029 & 6.35 $\pm$ 0.05 & 6.87 $\pm$ 0.04 & 6.98 $\pm$ 0.03\\ 
93 & 0.813 $\pm$ 0.037 & 6.37 $\pm$ 0.05 & 6.79 $\pm$ 0.05 & 6.93 $\pm$ 0.04\\ 
94 & 0.865 $\pm$ 0.034 & 6.0 $\pm$ 0.05 & 6.78 $\pm$ 0.04 & 6.85 $\pm$ 0.03\\ 
95 & 0.867 $\pm$ 0.033 & 6.32 $\pm$ 0.04 & 6.75 $\pm$ 0.04 & 6.89 $\pm$ 0.03\\ 
96 & 0.815 $\pm$ 0.027 & 6.13 $\pm$ 0.04 & 6.77 $\pm$ 0.04 & 6.86 $\pm$ 0.03\\ 
97 & 0.809 $\pm$ 0.026 & 5.95 $\pm$ 0.04 & 6.87 $\pm$ 0.04 & 6.92 $\pm$ 0.03\\ 
98 & 0.793 $\pm$ 0.032 & 6.42 $\pm$ 0.05 & 6.89 $\pm$ 0.04 & 7.02 $\pm$ 0.03\\ 
99 & 0.785 $\pm$ 0.029 & 6.55 $\pm$ 0.05 & 6.79 $\pm$ 0.04 & 6.99 $\pm$ 0.03\\ 
100 & 0.816 $\pm$ 0.031 & 6.09 $\pm$ 0.05 & 6.78 $\pm$ 0.04 & 6.86 $\pm$ 0.03\\ 
101 & 0.832 $\pm$ 0.04 & 6.27 $\pm$ 0.06 & 6.77 $\pm$ 0.05 & 6.89 $\pm$ 0.04\\ 
102 & 0.881 $\pm$ 0.032 & 5.89 $\pm$ 0.04 & 6.77 $\pm$ 0.04 & 6.83 $\pm$ 0.03\\ 
103 & 1.124 $\pm$ 0.055 & 6.19 $\pm$ 0.04 & 6.34 $\pm$ 0.04 & 6.57 $\pm$ 0.03\\ 
104 & 1.02 $\pm$ 0.067 & 5.95 $\pm$ 0.06 & 6.51 $\pm$ 0.05 & 6.62 $\pm$ 0.04\\ 
105 & 0.708 $\pm$ 0.03 & 6.44 $\pm$ 0.07 & 6.92 $\pm$ 0.06 & 7.04 $\pm$ 0.05\\ 
106 & 0.823 $\pm$ 0.047 & 6.05 $\pm$ 0.08 & 6.75 $\pm$ 0.07 & 6.83 $\pm$ 0.06\\ 
107 & 0.93 $\pm$ 0.045 & 5.76 $\pm$ 0.05 & 6.59 $\pm$ 0.05 & 6.65 $\pm$ 0.04\\ 
108 & 0.958 $\pm$ 0.048 & 5.92 $\pm$ 0.06 & 6.59 $\pm$ 0.05 & 6.67 $\pm$ 0.04\\ 
109 & 1.007 $\pm$ 0.063 & 5.73 $\pm$ 0.07 & 6.52 $\pm$ 0.06 & 6.58 $\pm$ 0.05\\ 
110 & 0.644 $\pm$ 0.018 & 6.61 $\pm$ 0.04 & 7.26 $\pm$ 0.03 & 7.35 $\pm$ 0.02\\ 
111 & 0.647 $\pm$ 0.032 & 6.81 $\pm$ 0.07 & 7.0 $\pm$ 0.05 & 7.22 $\pm$ 0.04\\ 
112 & 0.613 $\pm$ 0.026 & 6.75 $\pm$ 0.06 & 7.18 $\pm$ 0.05 & 7.31 $\pm$ 0.04\\ 
113 & 0.671 $\pm$ 0.021 & 6.68 $\pm$ 0.04 & 7.14 $\pm$ 0.03 & 7.27 $\pm$ 0.02\\ 
114 & 0.559 $\pm$ 0.03 & 6.84 $\pm$ 0.09 & 7.36 $\pm$ 0.06 & 7.47 $\pm$ 0.05\\ 
115 & 0.594 $\pm$ 0.024 & 6.83 $\pm$ 0.06 & 7.28 $\pm$ 0.04 & 7.41 $\pm$ 0.04\\ 
116 & 0.581 $\pm$ 0.023 & 7.05 $\pm$ 0.06 & 7.35 $\pm$ 0.04 & 7.53 $\pm$ 0.03\\ 
117 & 0.662 $\pm$ 0.02 & 6.62 $\pm$ 0.04 & 7.18 $\pm$ 0.03 & 7.29 $\pm$ 0.02\\ 
118 & 0.645 $\pm$ 0.021 & 6.77 $\pm$ 0.05 & 7.19 $\pm$ 0.03 & 7.33 $\pm$ 0.03\\ 
119 & 0.693 $\pm$ 0.015 & 6.55 $\pm$ 0.03 & 7.24 $\pm$ 0.02 & 7.32 $\pm$ 0.02\\ 
120 & 0.637 $\pm$ 0.024 & 6.78 $\pm$ 0.05 & 7.15 $\pm$ 0.04 & 7.31 $\pm$ 0.03\\ 
121 & 0.646 $\pm$ 0.025 & 6.71 $\pm$ 0.05 & 7.11 $\pm$ 0.04 & 7.25 $\pm$ 0.03\\ 


\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) & 12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline   
 
 
122 & 0.665 $\pm$ 0.018 & 6.67 $\pm$ 0.04 & 7.22 $\pm$ 0.03 & 7.33 $\pm$ 0.02\\ 
123 & 0.674 $\pm$ 0.021 & 6.7 $\pm$ 0.04 & 7.13 $\pm$ 0.03 & 7.26 $\pm$ 0.02\\ 
124 & 0.714 $\pm$ 0.045 & 6.61 $\pm$ 0.08 & 7.02 $\pm$ 0.06 & 7.17 $\pm$ 0.05\\ 
126 & 0.766 $\pm$ 0.027 & 6.49 $\pm$ 0.04 & 6.89 $\pm$ 0.04 & 7.04 $\pm$ 0.03\\ 
127 & 0.707 $\pm$ 0.029 & 6.39 $\pm$ 0.05 & 7.23 $\pm$ 0.04 & 7.28 $\pm$ 0.03\\ 
128 & 0.7 $\pm$ 0.037 & 6.37 $\pm$ 0.07 & 7.13 $\pm$ 0.05 & 7.2 $\pm$ 0.04\\ 
129 & 0.67 $\pm$ 0.024 & 6.62 $\pm$ 0.05 & 7.08 $\pm$ 0.04 & 7.21 $\pm$ 0.03\\ 
130 & 0.65 $\pm$ 0.021 & 6.74 $\pm$ 0.05 & 7.17 $\pm$ 0.03 & 7.31 $\pm$ 0.03\\ 
131 & 0.657 $\pm$ 0.019 & 6.43 $\pm$ 0.04 & 7.2 $\pm$ 0.03 & 7.27 $\pm$ 0.03\\ 
125 & 0.69 $\pm$ 0.02 & 6.59 $\pm$ 0.04 & 7.12 $\pm$ 0.03 & 7.23 $\pm$ 0.02\\ 
132 & 0.815 $\pm$ 0.025 & 6.26 $\pm$ 0.04 & 6.83 $\pm$ 0.03 & 6.94 $\pm$ 0.02\\ 
133 & 0.71 $\pm$ 0.018 & 6.38 $\pm$ 0.03 & 7.14 $\pm$ 0.03 & 7.2 $\pm$ 0.02\\ 
134 & 0.675 $\pm$ 0.019 & 6.81 $\pm$ 0.04 & 7.18 $\pm$ 0.03 & 7.33 $\pm$ 0.02\\ 
135 & 0.798 $\pm$ 0.026 & 6.21 $\pm$ 0.04 & 6.84 $\pm$ 0.03 & 6.93 $\pm$ 0.02\\ 
136 & 0.758 $\pm$ 0.055 & 6.38 $\pm$ 0.09 & 6.87 $\pm$ 0.06 & 6.99 $\pm$ 0.05\\ 
137 & 0.715 $\pm$ 0.027 & 6.63 $\pm$ 0.05 & 6.96 $\pm$ 0.04 & 7.13 $\pm$ 0.03\\ 
138 & 0.784 $\pm$ 0.023 & 6.3 $\pm$ 0.03 & 6.92 $\pm$ 0.03 & 7.02 $\pm$ 0.02\\ 
139 & 0.707 $\pm$ 0.039 & 6.46 $\pm$ 0.07 & 7.1 $\pm$ 0.05 & 7.19 $\pm$ 0.04\\ 
140 & 0.704 $\pm$ 0.017 & 6.64 $\pm$ 0.03 & 7.16 $\pm$ 0.02 & 7.27 $\pm$ 0.02\\ 
141 & 0.761 $\pm$ 0.06 & 6.13 $\pm$ 0.09 & 7.0 $\pm$ 0.07 & 7.05 $\pm$ 0.06\\ 
142 & 0.788 $\pm$ 0.023 & 6.29 $\pm$ 0.03 & 6.91 $\pm$ 0.03 & 7.01 $\pm$ 0.02\\ 
143 & 0.781 $\pm$ 0.072 & 6.43 $\pm$ 0.11 & 6.89 $\pm$ 0.08 & 7.02 $\pm$ 0.06\\ 
144 & 0.796 $\pm$ 0.076 & 6.43 $\pm$ 0.11 & 6.84 $\pm$ 0.08 & 6.99 $\pm$ 0.06\\ 
145 & 0.963 $\pm$ 0.067 & 6.42 $\pm$ 0.07 & 6.72 $\pm$ 0.05 & 6.9 $\pm$ 0.04\\ 
146 & 0.946 $\pm$ 0.075 & 6.06 $\pm$ 0.08 & 6.68 $\pm$ 0.06 & 6.77 $\pm$ 0.05\\ 
147 & 0.904 $\pm$ 0.023 & 5.79 $\pm$ 0.03 & 6.77 $\pm$ 0.02 & 6.81 $\pm$ 0.02\\ 
148 & 0.946 $\pm$ 0.028 & 5.54 $\pm$ 0.03 & 6.65 $\pm$ 0.02 & 6.68 $\pm$ 0.02\\ 
149 & 0.743 $\pm$ 0.052 & 6.48 $\pm$ 0.09 & 6.41 $\pm$ 0.06 & 6.74 $\pm$ 0.05\\ 
150 & 0.564 $\pm$ 0.03 & 7.01 $\pm$ 0.08 & 7.32 $\pm$ 0.06 & 7.49 $\pm$ 0.05\\ 
151 & 0.545 $\pm$ 0.015 & 6.93 $\pm$ 0.05 & 7.03 $\pm$ 0.03 & 7.28 $\pm$ 0.03\\ 
152 & 0.569 $\pm$ 0.012 & 6.88 $\pm$ 0.03 & 7.23 $\pm$ 0.03 & 7.39 $\pm$ 0.02\\ 
153 & 0.743 $\pm$ 0.049 & 6.48 $\pm$ 0.08 & 6.68 $\pm$ 0.06 & 6.89 $\pm$ 0.05\\ 
154 & 0.678 $\pm$ 0.036 & 6.62 $\pm$ 0.07 & 6.76 $\pm$ 0.05 & 7.0 $\pm$ 0.04\\ 
155 & 0.679 $\pm$ 0.039 & 6.54 $\pm$ 0.08 & 6.78 $\pm$ 0.06 & 6.97 $\pm$ 0.04\\ 
156 & 0.701 $\pm$ 0.035 & 6.72 $\pm$ 0.06 & 6.6 $\pm$ 0.05 & 6.96 $\pm$ 0.04\\ 
157 & 0.626 $\pm$ 0.011 & 6.59 $\pm$ 0.03 & 7.16 $\pm$ 0.02 & 7.26 $\pm$ 0.02\\ 
158 & 0.587 $\pm$ 0.008 & 6.77 $\pm$ 0.02 & 7.17 $\pm$ 0.02 & 7.32 $\pm$ 0.01\\ 
159 & 0.643 $\pm$ 0.022 & 6.67 $\pm$ 0.05 & 6.77 $\pm$ 0.04 & 7.02 $\pm$ 0.03\\ 
160 & 0.6 $\pm$ 0.015 & 6.81 $\pm$ 0.04 & 7.13 $\pm$ 0.03 & 7.3 $\pm$ 0.02\\ 
161 & 0.633 $\pm$ 0.024 & 6.83 $\pm$ 0.06 & 7.1 $\pm$ 0.04 & 7.29 $\pm$ 0.03\\ 
162 & 0.68 $\pm$ 0.034 & 6.63 $\pm$ 0.07 & 7.08 $\pm$ 0.05 & 7.21 $\pm$ 0.04\\ 
163 & 0.661 $\pm$ 0.032 & 6.84 $\pm$ 0.07 & 7.01 $\pm$ 0.05 & 7.24 $\pm$ 0.04\\ 
164 & 0.652 $\pm$ 0.021 & 6.67 $\pm$ 0.05 & 7.09 $\pm$ 0.03 & 7.23 $\pm$ 0.03\\ 
165 & 0.731 $\pm$ 0.026 & 6.52 $\pm$ 0.04 & 6.98 $\pm$ 0.03 & 7.11 $\pm$ 0.03\\ 
166 & 0.587 $\pm$ 0.029 & 6.87 $\pm$ 0.08 & 7.05 $\pm$ 0.06 & 7.27 $\pm$ 0.04\\ 
167 & 0.665 $\pm$ 0.016 & 6.53 $\pm$ 0.04 & 7.05 $\pm$ 0.03 & 7.16 $\pm$ 0.02\\ 
168 & 0.771 $\pm$ 0.051 & 6.54 $\pm$ 0.08 & 6.59 $\pm$ 0.06 & 6.86 $\pm$ 0.05\\ 
169 & 0.685 $\pm$ 0.011 & 6.33 $\pm$ 0.03 & 7.13 $\pm$ 0.03 & 7.19 $\pm$ 0.02\\ 
170 & 0.693 $\pm$ 0.027 & 6.46 $\pm$ 0.05 & 7.15 $\pm$ 0.04 & 7.23 $\pm$ 0.03\\ 
171 & 0.752 $\pm$ 0.035 & 6.47 $\pm$ 0.06 & 6.67 $\pm$ 0.05 & 6.88 $\pm$ 0.03\\ 
172 & 0.72 $\pm$ 0.024 & 6.33 $\pm$ 0.04 & 6.74 $\pm$ 0.04 & 6.89 $\pm$ 0.03\\ 
173 & 0.602 $\pm$ 0.021 & 6.88 $\pm$ 0.05 & 7.17 $\pm$ 0.04 & 7.35 $\pm$ 0.03\\ 
174 & 0.763 $\pm$ 0.071 & 6.46 $\pm$ 0.11 & 6.45 $\pm$ 0.08 & 6.76 $\pm$ 0.07\\ 
175 & 0.739 $\pm$ 0.027 & 6.49 $\pm$ 0.05 & 6.86 $\pm$ 0.04 & 7.01 $\pm$ 0.03\\ 
176 & 0.657 $\pm$ 0.014 & 6.68 $\pm$ 0.03 & 7.06 $\pm$ 0.03 & 7.21 $\pm$ 0.02\\ 
177 & 0.693 $\pm$ 0.03 & 6.65 $\pm$ 0.06 & 6.85 $\pm$ 0.05 & 7.06 $\pm$ 0.03\\ 
178 & 0.728 $\pm$ 0.025 & 6.59 $\pm$ 0.04 & 6.8 $\pm$ 0.04 & 7.01 $\pm$ 0.03\\ 
179 & 0.761 $\pm$ 0.061 & 6.38 $\pm$ 0.1 & 6.76 $\pm$ 0.07 & 6.91 $\pm$ 0.06\\ 
180 & 0.783 $\pm$ 0.072 & 6.38 $\pm$ 0.11 & 6.74 $\pm$ 0.08 & 6.9 $\pm$ 0.06\\ 
181 & 0.677 $\pm$ 0.027 & 6.72 $\pm$ 0.06 & 7.07 $\pm$ 0.05 & 7.23 $\pm$ 0.03\\ 
182 & 0.942 $\pm$ 0.039 & 6.1 $\pm$ 0.04 & 6.41 $\pm$ 0.03 & 6.58 $\pm$ 0.03\\ 

 
 
\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) & 12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline  
 
183 & 1.033 $\pm$ 0.032 & 6.26 $\pm$ 0.03 & 6.36 $\pm$ 0.03 & 6.61 $\pm$ 0.02\\ 
184 & 0.771 $\pm$ 0.04 & 6.69 $\pm$ 0.06 & 6.82 $\pm$ 0.05 & 7.06 $\pm$ 0.04\\ 
185 & 0.792 $\pm$ 0.045 & 6.8 $\pm$ 0.07 & 6.73 $\pm$ 0.05 & 7.07 $\pm$ 0.04\\ 
186 & 0.936 $\pm$ 0.026 & 6.02 $\pm$ 0.03 & 6.51 $\pm$ 0.03 & 6.63 $\pm$ 0.02\\ 
187 & 0.825 $\pm$ 0.065 & 6.29 $\pm$ 0.09 & 6.76 $\pm$ 0.07 & 6.89 $\pm$ 0.05\\ 
188 & 0.801 $\pm$ 0.036 & 6.56 $\pm$ 0.05 & 6.76 $\pm$ 0.04 & 6.98 $\pm$ 0.03\\ 
189 & 0.95 $\pm$ 0.121 & 6.38 $\pm$ 0.12 & 6.43 $\pm$ 0.09 & 6.71 $\pm$ 0.07\\ 
190 & 0.802 $\pm$ 0.067 & 6.53 $\pm$ 0.09 & 6.7 $\pm$ 0.07 & 6.93 $\pm$ 0.05\\ 
191 & 0.745 $\pm$ 0.027 & 6.29 $\pm$ 0.04 & 6.86 $\pm$ 0.03 & 6.97 $\pm$ 0.03\\ 
192 & 1.142 $\pm$ 0.062 & 6.06 $\pm$ 0.05 & 6.26 $\pm$ 0.04 & 6.47 $\pm$ 0.03\\ 
193 & 0.708 $\pm$ 0.029 & 6.26 $\pm$ 0.06 & 6.99 $\pm$ 0.05 & 7.07 $\pm$ 0.04\\ 
194 & 1.063 $\pm$ 0.033 & 5.84 $\pm$ 0.03 & 6.45 $\pm$ 0.03 & 6.54 $\pm$ 0.02\\ 
195 & 0.768 $\pm$ 0.038 & 6.55 $\pm$ 0.06 & 6.92 $\pm$ 0.05 & 7.07 $\pm$ 0.04\\ 
196 & 0.791 $\pm$ 0.058 & 6.44 $\pm$ 0.09 & 6.77 $\pm$ 0.06 & 6.94 $\pm$ 0.05\\ 
197 & 0.888 $\pm$ 0.043 & 6.34 $\pm$ 0.05 & 6.74 $\pm$ 0.05 & 6.89 $\pm$ 0.03\\ 
198 & 0.923 $\pm$ 0.085 & 6.32 $\pm$ 0.09 & 6.68 $\pm$ 0.07 & 6.84 $\pm$ 0.05\\ 
199 & 0.917 $\pm$ 0.035 & 5.91 $\pm$ 0.04 & 6.68 $\pm$ 0.04 & 6.75 $\pm$ 0.03\\ 
200 & 0.749 $\pm$ 0.027 & 6.22 $\pm$ 0.05 & 7.03 $\pm$ 0.04 & 7.09 $\pm$ 0.03\\ 
201 & 1.204 $\pm$ 0.177 & 6.1 $\pm$ 0.12 & 6.16 $\pm$ 0.13 & 6.43 $\pm$ 0.08\\ 
202 & 0.898 $\pm$ 0.108 & 6.39 $\pm$ 0.12 & 6.71 $\pm$ 0.09 & 6.88 $\pm$ 0.07\\ 
203 & 0.739 $\pm$ 0.036 & 6.59 $\pm$ 0.06 & 6.98 $\pm$ 0.05 & 7.12 $\pm$ 0.04\\ 
204 & 0.954 $\pm$ 0.026 & 6.15 $\pm$ 0.03 & 6.61 $\pm$ 0.03 & 6.74 $\pm$ 0.02\\ 
205 & 1.157 $\pm$ 0.07 & 5.88 $\pm$ 0.05 & 6.22 $\pm$ 0.05 & 6.38 $\pm$ 0.03\\ 
206 & 1.167 $\pm$ 0.102 & 5.83 $\pm$ 0.07 & 6.28 $\pm$ 0.06 & 6.42 $\pm$ 0.04\\ 
207 & 1.177 $\pm$ 0.113 & 5.69 $\pm$ 0.08 & 6.17 $\pm$ 0.06 & 6.29 $\pm$ 0.05\\ 
208 & 1.11 $\pm$ 0.038 & 5.68 $\pm$ 0.03 & 6.29 $\pm$ 0.03 & 6.39 $\pm$ 0.03\\ 
209 & 1.246 $\pm$ 0.038 & 5.64 $\pm$ 0.03 & 6.14 $\pm$ 0.03 & 6.26 $\pm$ 0.02\\ 
210 & 1.234 $\pm$ 0.073 & 5.77 $\pm$ 0.05 & 6.12 $\pm$ 0.04 & 6.28 $\pm$ 0.03\\ 
211 & 1.355 $\pm$ 0.041 & 5.65 $\pm$ 0.02 & 5.98 $\pm$ 0.02 & 6.15 $\pm$ 0.02\\ 
212 & 1.345 $\pm$ 0.151 & 5.6 $\pm$ 0.08 & 6.03 $\pm$ 0.07 & 6.17 $\pm$ 0.05\\ 
213 & 1.411 $\pm$ 0.235 & 5.7 $\pm$ 0.11 & 5.88 $\pm$ 0.09 & 6.1 $\pm$ 0.07\\ 
214 & 1.351 $\pm$ 0.101 & 5.65 $\pm$ 0.05 & 5.96 $\pm$ 0.05 & 6.13 $\pm$ 0.03\\ 
215 & 0.996 $\pm$ 0.117 & 5.74 $\pm$ 0.11 & 6.46 $\pm$ 0.08 & 6.54 $\pm$ 0.07\\ 
216 & 1.082 $\pm$ 0.066 & 5.94 $\pm$ 0.06 & 6.34 $\pm$ 0.05 & 6.49 $\pm$ 0.04\\ 
217 & 1.053 $\pm$ 0.054 & 6.01 $\pm$ 0.05 & 6.43 $\pm$ 0.05 & 6.57 $\pm$ 0.04\\ 
218 & 1.027 $\pm$ 0.143 & 6.06 $\pm$ 0.13 & 6.49 $\pm$ 0.14 & 6.63 $\pm$ 0.1\\ 
219 & 1.276 $\pm$ 0.066 & 5.51 $\pm$ 0.05 & 6.14 $\pm$ 0.04 & 6.23 $\pm$ 0.04\\ 
220 & 1.369 $\pm$ 0.057 & 5.54 $\pm$ 0.03 & 6.07 $\pm$ 0.03 & 6.18 $\pm$ 0.03\\ 
221 & 1.419 $\pm$ 0.207 & 5.42 $\pm$ 0.1 & 6.01 $\pm$ 0.09 & 6.11 $\pm$ 0.07\\ 
222 & 0.828 $\pm$ 0.052 & 6.05 $\pm$ 0.08 & 6.83 $\pm$ 0.06 & 6.9 $\pm$ 0.05\\ 
223 & 0.798 $\pm$ 0.049 & 6.18 $\pm$ 0.07 & 6.85 $\pm$ 0.06 & 6.93 $\pm$ 0.05\\ 
224 & 0.926 $\pm$ 0.065 & 6.09 $\pm$ 0.08 & 6.63 $\pm$ 0.06 & 6.74 $\pm$ 0.05\\ 
225 & 1.111 $\pm$ 0.143 & 6.04 $\pm$ 0.11 & 6.41 $\pm$ 0.09 & 6.57 $\pm$ 0.07\\ 
226 & 1.257 $\pm$ 0.164 & 5.55 $\pm$ 0.1 & 6.24 $\pm$ 0.08 & 6.32 $\pm$ 0.06\\ 
227 & 1.043 $\pm$ 0.028 & 5.19 $\pm$ 0.03 & 6.49 $\pm$ 0.02 & 6.51 $\pm$ 0.02\\ 
228 & 0.793 $\pm$ 0.033 & 6.55 $\pm$ 0.05 & 6.73 $\pm$ 0.03 & 6.95 $\pm$ 0.03\\ 
229 & 0.799 $\pm$ 0.009 & 6.0 $\pm$ 0.01 & 6.99 $\pm$ 0.01 & 7.04 $\pm$ 0.01\\ 
230 & 0.797 $\pm$ 0.008 & 6.13 $\pm$ 0.01 & 7.05 $\pm$ 0.01 & 7.1 $\pm$ 0.01\\ 
231 & 1.078 $\pm$ 0.046 & 5.6 $\pm$ 0.04 & 6.44 $\pm$ 0.03 & 6.5 $\pm$ 0.02\\ 
233 & 0.885 $\pm$ 0.01 & 5.77 $\pm$ 0.01 & 6.94 $\pm$ 0.01 & 6.97 $\pm$ 0.01\\ 
233 & 1.16 $\pm$ 0.071 & 5.41 $\pm$ 0.06 & 6.22 $\pm$ 0.06 & 6.28 $\pm$ 0.05\\ 
234 & 0.787 $\pm$ 0.021 & 6.07 $\pm$ 0.04 & 7.07 $\pm$ 0.04 & 7.11 $\pm$ 0.03\\ 
235 & 0.968 $\pm$ 0.033 & 5.82 $\pm$ 0.04 & 6.6 $\pm$ 0.04 & 6.66 $\pm$ 0.03\\ 
236 & 0.792 $\pm$ 0.016 & 5.74 $\pm$ 0.03 & 7.05 $\pm$ 0.02 & 7.07 $\pm$ 0.02\\ 
237 & 1.064 $\pm$ 0.05 & 5.56 $\pm$ 0.05 & 6.51 $\pm$ 0.05 & 6.56 $\pm$ 0.04\\ 
238 & 1.383 $\pm$ 0.07 & 5.0 $\pm$ 0.04 & 6.08 $\pm$ 0.04 & 6.12 $\pm$ 0.04\\ 
239 & 1.402 $\pm$ 0.204 & 4.7 $\pm$ 0.11 & 6.07 $\pm$ 0.11 & 6.09 $\pm$ 0.1\\ 
240 & 0.934 $\pm$ 0.129 & 6.11 $\pm$ 0.13 & 6.28 $\pm$ 0.1 & 6.5 $\pm$ 0.07\\ 
241 & 0.66 $\pm$ 0.034 & 6.68 $\pm$ 0.07 & 6.95 $\pm$ 0.05 & 7.14 $\pm$ 0.04\\ 
242 & 0.661 $\pm$ 0.027 & 6.6 $\pm$ 0.06 & 7.04 $\pm$ 0.04 & 7.17 $\pm$ 0.03\\ 
243 & 0.681 $\pm$ 0.038 & 6.7 $\pm$ 0.07 & 6.85 $\pm$ 0.05 & 7.08 $\pm$ 0.04\\ 

 
\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) & 12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline  
 
 
244 & 0.672 $\pm$ 0.029 & 6.77 $\pm$ 0.06 & 6.99 $\pm$ 0.04 & 7.19 $\pm$ 0.03\\ 
245 & 0.653 $\pm$ 0.019 & 6.68 $\pm$ 0.04 & 7.22 $\pm$ 0.03 & 7.33 $\pm$ 0.02\\ 
246 & 0.644 $\pm$ 0.031 & 6.76 $\pm$ 0.07 & 7.02 $\pm$ 0.05 & 7.21 $\pm$ 0.04\\ 
247 & 0.665 $\pm$ 0.023 & 6.61 $\pm$ 0.05 & 7.1 $\pm$ 0.03 & 7.22 $\pm$ 0.03\\ 
248 & 0.735 $\pm$ 0.033 & 6.59 $\pm$ 0.06 & 6.82 $\pm$ 0.04 & 7.02 $\pm$ 0.03\\ 
249 & 0.758 $\pm$ 0.073 & 6.67 $\pm$ 0.11 & 6.74 $\pm$ 0.08 & 7.01 $\pm$ 0.06\\ 
250 & 0.687 $\pm$ 0.039 & 6.81 $\pm$ 0.08 & 6.83 $\pm$ 0.05 & 7.12 $\pm$ 0.04\\ 
251 & 0.751 $\pm$ 0.091 & 6.64 $\pm$ 0.14 & 6.83 $\pm$ 0.1 & 7.05 $\pm$ 0.08\\ 
252 & 0.787 $\pm$ 0.105 & 6.54 $\pm$ 0.15 & 6.72 $\pm$ 0.11 & 6.94 $\pm$ 0.08\\ 
253 & 0.844 $\pm$ 0.06 & 6.31 $\pm$ 0.08 & 6.71 $\pm$ 0.06 & 6.86 $\pm$ 0.04\\ 
254 & 0.826 $\pm$ 0.032 & 6.51 $\pm$ 0.04 & 6.76 $\pm$ 0.04 & 6.95 $\pm$ 0.03\\ 
255 & 0.934 $\pm$ 0.077 & 6.11 $\pm$ 0.08 & 6.68 $\pm$ 0.06 & 6.78 $\pm$ 0.05\\










 
 












\hline

\end{tabular}
\begin{tablenotes}

$^a$ In units of 10$^{4}$K.\\
    
\end{tablenotes}
\end{table*}
\newpage

==> Tables/Tabla_HII_lines.tex <==
\begin{table*}
\centering
\caption{Reddening corrected emission line intensities, relative to H$\beta$ = 100, for objects in the \HII Gal sub-sample.}
\label{linesHII}
\begin{tabular}{cccccccccc}
 \cline{1-10}
  & Line & [OII] & [OIII] & [ArIV] & [OIII] & [SIII] & [SII] & [ArIII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 & 4740 & 4959, 5007 & 6312  &  6717, 6731 & 7136 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{8}{c}{I($\lambda $)$^{a}$} \\ \hline



257 & IZW18NW & 26.4 $\pm$ 1.1 & 4.4 $\pm$ 0.7 & -& 259.8 $\pm$ 7.3 & 1.27 $\pm$ 0.03 & 3.58 $\pm$ 0.29 & -& 10.32 $\pm$ 0.28\\ 
258 & IZW18SE & 46.6 $\pm$ 2.2 & 6.2 $\pm$ 0.4 & -& 232.1 $\pm$ 6.7 & 0.63 $\pm$ 0.05 & 7.05 $\pm$ 0.11 & -& 13.42 $\pm$ 0.34\\ 
259 & UGC4483 & 83.5 $\pm$ 5.7 & 6.6 $\pm$ 0.4 & -& 362.8 $\pm$ 9.4 & 0.57 $\pm$ 0.05 & 12.43 $\pm$ 0.16 & -& 28.6 $\pm$ 4.3\\ 
260 & Mrk5 & 212.9 $\pm$ 3.1 & 4.4 $\pm$ 0.5 & -& 511.3 $\pm$ 6.3 & 1.39 $\pm$ 0.04 & 37.8 $\pm$ 0.45 & -& 48.1 $\pm$ 3.4\\ 
261 & 0749+568 & 166.8 $\pm$ 4.3 & 9.8 $\pm$ 1.1 & -& 655.2 $\pm$ 13.8 & 1.6 $\pm$ 0.2 & 23.4 $\pm$ 0.2 & -& 43.688 $\pm$ 4.816\\ 
262 & 0926+606 & 178.5 $\pm$ 1.2 & 8.3 $\pm$ 0.3 & -& 640.0 $\pm$ 3.6 & 2.3 $\pm$ 0.3 & 32.0 $\pm$ 0.3 & -& 48.2 $\pm$ 5.8\\ 
263 & Mrk709 & 181.6 $\pm$ 3.5 & 8.8 $\pm$ 0.5 & -& 522.6 $\pm$ 7.0 & 2.0 $\pm$ 0.1 & 62.3 $\pm$ 0.5 & -& 29.928 $\pm$ 3.44\\ 
264 & Mrk22 & 148.7 $\pm$ 2.3 & 8.2 $\pm$ 0.3 & -& 727.9 $\pm$ 5.8 & 1.4 $\pm$ 0.1 & 26.6 $\pm$ 0.4 & -& 50.912 $\pm$ 6.88\\ 
265 & Mrk1434 & 96.8 $\pm$ 0.6 & 10.4 $\pm$ 0.2 & -& 673.2 $\pm$ 2.9 & 3.0 $\pm$ 0.1 & 15.07 $\pm$ 0.5 & -& 31.648 $\pm$ 2.752\\ 
266 & MRK36 & 129.3 $\pm$ 1.5 & 9.6 $\pm$ 0.5 & -& 645.6 $\pm$ 5.8 & 1.6 $\pm$ 0.1 & 20.0 $\pm$ 0.16 & -& 41.4 $\pm$ 4.9\\ 
267 & Viizw403 & 133.3 $\pm$ 0.9 & 7.1 $\pm$ 0.2 & -& 459.8 $\pm$ 4.7 & 1.8 $\pm$ 0.2 & 13.0 $\pm$ 0.2 & -& 40.248 $\pm$ 4.472\\ 
268 & Um461 & 52.7 $\pm$ 1.5 & 13.6 $\pm$ 0.7 & -& 806.1 $\pm$ 12.4 & 1.3 $\pm$ 0.1 & 10.3 $\pm$ 0.2 & -& 34.1 $\pm$ 1.5\\ 
269 & Um462 & 174.2 $\pm$ 1.0 & 7.8 $\pm$ 0.2 & -& 659.2 $\pm$ 3.2 & 2.0 $\pm$ 0.1 & 28.3 $\pm$ 0.2 & -& 45.5 $\pm$ 5.1\\ 
270 & Mrk209 & 71.9 $\pm$ 0.2 & 12.7 $\pm$ 0.1 & -& 750.3 $\pm$ 1.1 & 2.1 $\pm$ 0.2 & 10.6 $\pm$ 0.5 & -& 41.968 $\pm$ 4.128\\ 
271 & WHT-0364 & 147.1 $\pm$ 2.2 & 7.0 $\pm$ 0.2 & 0.5 $\pm$ 0.1 & 758.0 $\pm$ 4.2 & 1.9 $\pm$ 0.1 & 23.5 $\pm$ 0.4 & 8.0 $\pm$ 0.3 & 47.1 $\pm$ 2.4\\ 
272 & WHT-0390 & 163.4 $\pm$ 1.9 & 5.6 $\pm$ 0.3 & 0.5 $\pm$ 0.1 & 586.6 $\pm$ 3.9 & 1.8 $\pm$ 0.04 & 24.3 $\pm$ 0.6 & 6.2 $\pm$ 0.2 & 35.8 $\pm$ 1.5\\ 
273 & WHT-0417 & 157.3 $\pm$ 1.4 & 6.2 $\pm$ 0.3 & 0.5 $\pm$ 0.1 & 618.9 $\pm$ 3.7 & 1.2 $\pm$ 0.1 & 29.8 $\pm$ 1.0 & 9.2 $\pm$ 0.3 & 66.2 $\pm$ 4.8\\ 
274 & NGC5253-HII-2 & 137.2 $\pm$ 4.9 & 6.46 $\pm$ 0.23 & 0.723 $\pm$ 0.059 & 783.0 $\pm$ 23.1 & 2.3 $\pm$ 0.1 & 25.81 $\pm$ 0.8 & 13.5 $\pm$ 0.56 & 96.0 $\pm$ 9.8\\ 
275 & NGC5253-HII-1 & 134.8 $\pm$ 4.8 & 3.95 $\pm$ 0.23 & 0.918 $\pm$ 0.055 & 803.2 $\pm$ 24.2 & 1.6 $\pm$ 0.1 & 22.55 $\pm$ 0.9 & 13.07 $\pm$ 0.54 & 89.3 $\pm$ 8.3\\ 
276 & NGC5253-UV-1 & 182.3 $\pm$ 6.5 & 2.61 $\pm$ 0.16 & 0.135 $\pm$ 0.033 & 620.9 $\pm$ 17.8 & 2.0 $\pm$ 0.1 & 26.07 $\pm$ 1.0 & 10.4 $\pm$ 0.44 & 72.9 $\pm$ 7.3\\ 
277 & NGC5253-UV-2 & 353.4 $\pm$ 12.5 & 2.61 $\pm$ 0.31 & -& 404.5 $\pm$ 12.6 & 1.7 $\pm$ 0.1 & 65.0 $\pm$ 1.4 & 8.89 $\pm$ 0.45 & 61.64 $\pm$ 6.02\\ 
278 & CAHA-132 & 153.2 $\pm$ 1.8 & 4.2 $\pm$ 0.21 & -& 666.9 $\pm$ 3.0 & 1.6 $\pm$ 0.1 & 34.6 $\pm$ 0.5 & -& 77.3 $\pm$ 3.8\\ 
279 & CAHA-135 & 188.3 $\pm$ 2.3 & 5.24 $\pm$ 0.24 & -& 574.1 $\pm$ 3.7 & 1.4 $\pm$ 0.1 & 38.1 $\pm$ 1.0 & -& 50.7 $\pm$ 3.6\\ 
280 & CAHA-143 & 226.9 $\pm$ 2.9 & 10.22 $\pm$ 0.35 & -& 655.6 $\pm$ 4.6 & 1.9 $\pm$ 0.1 & 33.8 $\pm$ 0.4 & -& 58.4 $\pm$ 4.2\\ 
281 & CAHA-151 & 111.5 $\pm$ 1.6 & 9.9 $\pm$ 0.6 & 1.03 $\pm$ 0.14 & 818.2 $\pm$ 4.7 & 1.8 $\pm$ 0.1 & 17.9 $\pm$ 0.6 & 6.62 $\pm$ 0.3 & 44.3 $\pm$ 2.1\\ 
282 & CAHA-049 & 217.9 $\pm$ 2.6 & 2.91 $\pm$ 0.17 & -& 414.2 $\pm$ 2.7 & 1.81 $\pm$ 0.11 & 45.3 $\pm$ 1.0 & -& 74.3 $\pm$ 3.9\\ 
283 & CAHA-052 & 84.9 $\pm$ 2.0 & 8.51 $\pm$ 0.26 & 0.69 $\pm$ 0.22 & 820.1 $\pm$ 5.2 & 1.54 $\pm$ 0.07 & 13.5 $\pm$ 0.31 & 7.36 $\pm$ 0.44 & 56.6 $\pm$ 2.1\\ 
284 & CAHA-011 & 176.2 $\pm$ 2.4 & 6.6 $\pm$ 0.24 & 0.4 $\pm$ 0.1 & 686.4 $\pm$ 5.6 & 0.9 $\pm$ 0.03 & 23.0 $\pm$ 0.53 & 8.64 $\pm$ 0.41 & 68.1 $\pm$ 3.4\\ 
285 & SBS0035-052E-1+2 & 24.84 $\pm$ 0.39 & 10.84 $\pm$ 0.16 & 0.93 $\pm$ nan & 412.68 $\pm$ 5.89 & 0.72 $\pm$ 0.04 & 3.23 $\pm$ 0.49 & 1.88 $\pm$ 0.03 & 15.93 $\pm$ 0.48\\ 
286 & SBS0035-052E-4+5 & 24.03 $\pm$ 0.44 & 11.22 $\pm$ 0.23 & 1.12 $\pm$ 0.05 & 443.62 $\pm$ 6.4 & 2.06 $\pm$ 0.04 & 2.94 $\pm$ 0.35 & 1.45 $\pm$ 0.04 & 9.63 $\pm$ 0.62\\ 
287 & SBS0035-052E-7 & 18.79 $\pm$ 0.3 & 7.55 $\pm$ 0.65 & -& 329.96 $\pm$ 5.13 & 0.77 $\pm$ 0.03 & 3.51 $\pm$ 0.56 & -& 8.05 $\pm$ 0.21\\ 
288 & Mrk59 & 113.24 $\pm$ 3.5 & 8.34 $\pm$ 0.29 & 0.71 $\pm$ 0.1 & 794.19 $\pm$ 22.79 & 1.64 $\pm$ 0.03 & 15.76 $\pm$ 0.22 & 7.87 $\pm$ 0.27 & 51.53 $\pm$ 1.86\\ 
289 & Tol2240-384 & 86.95 $\pm$ 1.45 & 14.73 $\pm$ 0.31 & -& 886.84 $\pm$ 12.76 & 0.83 $\pm$ 0.03 & 10.08 $\pm$ 0.09 & -& 24.71 $\pm$ 2.0\\ 
290 & UM283-D & 294.6 $\pm$ 5.0 & 4.1 $\pm$ 0.29 & -& 455.2 $\pm$ 7.2 & 1.49 $\pm$ 0.03 & 50.1 $\pm$ 0.18 & -& 71.2 $\pm$ 3.44\\ 
291 & UM133-H & 107.18 $\pm$ 1.7 & 7.72 $\pm$ 0.24 & -& 495.47 $\pm$ 7.34 & 2.32 $\pm$ 0.04 & 16.34 $\pm$ 0.24 & -& 25.5 $\pm$ 0.83\\ 
292 & He-10-C & 211.87 $\pm$ 3.33 & 1.96 $\pm$ 0.09 & -& 214.8 $\pm$ 3.13 & 1.98 $\pm$ 0.04 & 32.56 $\pm$ 0.42 & -& 117.6 $\pm$ 2.2\\ 
293 & He-10-E & 193.03 $\pm$ 3.09 & 0.26 $\pm$ 0.05 & -& 169.31 $\pm$ 2.5 & 1.85 $\pm$ 0.05 & 30.04 $\pm$ 0.3 & -& 95.3 $\pm$ 1.82\\ 
294 & NGC3125 & 93.12 $\pm$ 1.44 & 5.13 $\pm$ 0.08 & 0.44 $\pm$ 0.02 & 776.0 $\pm$ 11.08 & 2.53 $\pm$ 0.05 & 21.89 $\pm$ 0.24 & 13.0 $\pm$ 0.21 & 110.0 $\pm$ 2.03\\ 
295 & Mrk1259 & 170.87 $\pm$ 2.75 & 1.08 $\pm$ 0.12 & -& 216.99 $\pm$ 3.24 & 1.69 $\pm$ 0.03 & 33.88 $\pm$ 0.32 & -& 81.7 $\pm$ 1.58\\ 
296 & Pox4 & 81.26 $\pm$ 1.27 & 9.12 $\pm$ 0.13 & 0.93 $\pm$ 0.02 & 870.78 $\pm$ 12.55 & 1.38 $\pm$ 0.08 & 13.57 $\pm$ 0.72 & 5.35 $\pm$ 0.09 & 42.3 $\pm$ 0.79\\ 
297 & Tol1214-277 & 30.82 $\pm$ 0.48 & 17.29 $\pm$ 0.26 & 2.07 $\pm$ 0.05 & 683.71 $\pm$ 10.74 & 2.0 $\pm$ 0.03 & 3.63 $\pm$ 0.19 & 2.08 $\pm$ 0.04 & 9.8 $\pm$ 0.41\\ 
298 & J1253-0312 & 84.22 $\pm$ 1.3 & 10.37 $\pm$ 0.15 & 0.99 $\pm$ 0.02 & 857.88 $\pm$ 12.24 & 2.72 $\pm$ 0.05 & 11.19 $\pm$ 0.16 & 6.65 $\pm$ 0.11 & 47.3 $\pm$ 0.86\\ 
299 & NGC5253-C1 & 96.34 $\pm$ 1.5 & 7.45 $\pm$ 0.11 & 1.27 $\pm$ 0.02 & 840.87 $\pm$ 12.02 & 1.51 $\pm$ 0.03 & 15.58 $\pm$ 0.25 & 12.68 $\pm$ 0.21 & 77.2 $\pm$ 1.41\\ 
300 & NGC5253-C2 & 148.48 $\pm$ 2.32 & 3.09 $\pm$ 0.05 & 0.18 $\pm$ 0.01 & 595.11 $\pm$ 8.52 & 1.33 $\pm$ 0.03 & 27.0 $\pm$ 0.21 & 11.31 $\pm$ 0.18 & 74.2 $\pm$ 1.38\\ 
301 & NGC5253-P1 & 175.56 $\pm$ 2.77 & -& 0.14 $\pm$ 0.02 & 675.48 $\pm$ 9.63 & 1.71 $\pm$ 0.03 & 18.93 $\pm$ 0.31 & 10.85 $\pm$ 0.18 & 72.6 $\pm$ 1.34\\ 
302 & NGC5253-P2 & 106.83 $\pm$ 1.69 & 7.92 $\pm$ 0.12 & 0.97 $\pm$ 0.03 & 866.94 $\pm$ 12.36 & 2.27 $\pm$ 0.04 & 15.19 $\pm$ 0.17 & 12.88 $\pm$ 0.21 & 78.5 $\pm$ 1.44\\ 
303 & Tol89-1 & 151.6 $\pm$ 2.36 & 3.38 $\pm$ 0.07 & 0.2 $\pm$ 0.01 & 650.69 $\pm$ 9.29 & 1.27 $\pm$ 0.15 & 20.66 $\pm$ 0.52 & 10.65 $\pm$ 0.17 & 85.4 $\pm$ 1.58\\ 
304 & Tol89-2 & 157.762 $\pm$ 2.6 & 1.94 $\pm$ 0.11 & -& 507.7 $\pm$ 6.6 & 1.1 $\pm$ 0.03 & 43.17 $\pm$ 0.41 & -& 172.4 $\pm$ 3.44\\ 
305 & NGC5408-1 & 116.51 $\pm$ 1.8 & 19.77 $\pm$ 0.29 & -& 1253.69 $\pm$ 16.7 & 1.05 $\pm$ 0.18 & 11.86 $\pm$ 0.72 & -& 36.4 $\pm$ 0.65\\ 
306 & NGC5408-2 & 196.84 $\pm$ 3.04 & 11.91 $\pm$ 0.18 & -& 1020.55 $\pm$ 14.62 & 1.32 $\pm$ 0.06 & 26.83 $\pm$ 0.33 & -& 53.6 $\pm$ 1.0\\ 
307 & Tol1457-262 & 258.97 $\pm$ 4.03 & 6.8 $\pm$ 0.1 & 0.42 $\pm$ 0.02 & 839.18 $\pm$ 12.09 & 0.55 $\pm$ 0.03 & 21.02 $\pm$ 0.1 & 6.75 $\pm$ 0.11 & 47.8 $\pm$ 0.89\\ 
308 & Tol1924-416-1 & 94.48 $\pm$ 1.55 & 5.36 $\pm$ 0.09 & 0.28 $\pm$ 0.01 & 579.19 $\pm$ 8.8 & 0.64 $\pm$ 0.06 & 16.87 $\pm$ 0.08 & 4.76 $\pm$ 0.08 & 45.0 $\pm$ 0.89\\ 
309 & Tol1924-416-2 & 113.9 $\pm$ 1.79 & 6.23 $\pm$ 0.09 & 0.43 $\pm$ 0.02 & 704.82 $\pm$ 10.25 & 0.65 $\pm$ 0.02 & 19.47 $\pm$ 0.15 & 6.2 $\pm$ 0.1 & 48.1 $\pm$ 0.89\\ 
310 & NGC6822-V & 78.55 $\pm$ 1.23 & 5.18 $\pm$ 0.08 & 0.2 $\pm$ 0.01 & 716.75 $\pm$ 9.29 & 1.84 $\pm$ 0.09 & 10.65 $\pm$ 0.53 & 10.57 $\pm$ 0.17 & 88.1 $\pm$ 1.65\\ 
311 & PHL-293B & 51.16 $\pm$ 1.62 & 14.55 $\pm$ 0.27 & 1.33 $\pm$ 0.17 & 726.79 $\pm$ 10.67 & 1.5 $\pm$ 0.1 & 7.78 $\pm$ 0.2 & 3.89 $\pm$ 0.26 & 32.78 $\pm$ 1.24\\ 
312 & HG031203 & 85.8 $\pm$ 3.5 & 8.5 $\pm$ 0.6 & -& 978.8 $\pm$ 11.6 & 1.19 $\pm$ 0.04 & 15.6 $\pm$ 2.0 & -& 54.99 $\pm$ 1.0\\ 
313 & Mrk71 & 44.09 $\pm$ 1.11 & 16.32 $\pm$ 0.61 & 2.29 $\pm$ 0.22 & 966.7 $\pm$ 13.96 & 1.68 $\pm$ 0.24 & 6.42 $\pm$ 0.76 & 5.39 $\pm$ 0.31 & 31.5 $\pm$ 1.05\\ 
314 & Mrk930 & 250.96 $\pm$ 4.94 & 5.21 $\pm$ 0.51 & -& 560.92 $\pm$ 9.93 & 1.55 $\pm$ 0.09 & 46.76 $\pm$ 0.37 & -& 54.0 $\pm$ 1.64\\ 
315 & IIZW40 & 59.06 $\pm$ 2.03 & 12.77 $\pm$ 0.7 & 1.29 $\pm$ 0.2 & 963.2 $\pm$ 14.32 & 1.7 $\pm$ 0.1 & 9.02 $\pm$ 0.35 & 8.03 $\pm$ 0.29 & 39.89 $\pm$ 0.92\\ 
316 & Haro11B & 218.63 $\pm$ 3.41 & 2.45 $\pm$ 0.05 & 0.17 $\pm$ 0.02 & 490.94 $\pm$ 7.06 & 1.25 $\pm$ 0.15 & 25.88 $\pm$ 0.51 & 7.01 $\pm$ 0.12 & 71.04 $\pm$ 1.19\\ 
317 & Haro11C & 233.6 $\pm$ 3.8 & 2.96 $\pm$ 0.34 & -& 416.21 $\pm$ 6.16 & 1.41 $\pm$ 0.15 & 42.51 $\pm$ 0.63 & -& 87.85 $\pm$ 1.05\\ 


\end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{cccccccccc}
 \cline{1-10}
  & Line & [OII] & [OIII] & [ArIV] & [OIII] & [SIII] & [SII] & [ArIII] & [SIII]\\
  & $\lambda$ & 3727, 3729 & 4363 & 4740 & 4959, 5007 & 6312  &  6717, 6731 & 7136 & 9069, 9532\\\hline
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{Region} & \multicolumn{8}{c}{I($\lambda $)$^{a}$} \\ \hline
  
 
 
318 & ESO338-IG004 & 137.46 $\pm$ 2.22 & 9.59 $\pm$ 0.65 & 0.84 $\pm$ 0.07 & 684.96 $\pm$ 9.91 & 1.69 $\pm$ 0.11 & 19.37 $\pm$ 0.35 & 5.6 $\pm$ 0.11 & 55.5 $\pm$ 0.69\\ 
319 & J0908+0517-2 & 89.38 $\pm$ 2.61 & 2.4 $\pm$ 0.54 & -& 544.1 $\pm$ 9.69 & 1.18 $\pm$ 0.13 & 23.66 $\pm$ 0.32 & -& 38.91 $\pm$ 2.3\\ 
320 & J1226-0115-1 & 94.02 $\pm$ 1.91 & 12.74 $\pm$ 0.4 & 0.98 $\pm$ 0.15 & 744.12 $\pm$ 11.32 & 1.06 $\pm$ 0.14 & 17.13 $\pm$ 0.37 & 6.17 $\pm$ 0.16 & 31.34 $\pm$ 0.96\\ 
321 & J1226-0115-2 & 86.25 $\pm$ 1.77 & 10.03 $\pm$ 0.33 & 0.93 $\pm$ 0.18 & 681.15 $\pm$ 10.24 & 1.36 $\pm$ 0.16 & 17.01 $\pm$ 0.48 & 5.3 $\pm$ 0.13 & 32.13 $\pm$ 0.89\\ 
322 & J1235+2755-2 & 188.91 $\pm$ 3.61 & 5.67 $\pm$ 0.33 & -& 455.53 $\pm$ 7.11 & 0.41 $\pm$ 0.06 & 22.4 $\pm$ 0.1 & -& 42.97 $\pm$ 1.38\\ 
323 & J1235+2755-3 & 234.09 $\pm$ 4.97 & 7.23 $\pm$ 0.53 & -& 467.61 $\pm$ 7.68 & 1.929 $\pm$ 0.35 & 23.61 $\pm$ 0.77 & -& 47.3 $\pm$ 1.65\\ 
324 & J1241-0340 & 127.94 $\pm$ 2.28 & 11.96 $\pm$ 0.32 & -& 670.42 $\pm$ 9.96 & 1.954 $\pm$ 0.12 & 17.51 $\pm$ 0.28 & -& 35.05 $\pm$ 0.93\\ 
325 & SBS1420+544 & 57.64 $\pm$ 1.58 & 15.48 $\pm$ 0.46 & 1.67 $\pm$ 0.24 & 882.1 $\pm$ 13.77 & 1.893 $\pm$ 0.18 & 8.95 $\pm$ 0.57 & 4.38 $\pm$ 0.15 & 35.09 $\pm$ 1.34\\ 
326 & PHL-293B & 108.65 $\pm$ 2.41 & 11.93 $\pm$ 0.4 & -& 621.67 $\pm$ 9.5 & 1.785 $\pm$ 0.045 & 12.03 $\pm$ 0.51 & -& 19.37 $\pm$ 0.86\\ 
327 & NGC5408 & 88.0 $\pm$ 4.0 & 12.0 $\pm$ 0.5 & 1.2 $\pm$ 0.05 & 761.0 $\pm$ 21.0 & 0.63 $\pm$ 0.04 & 13.3 $\pm$ 0.12 & 7.4 $\pm$ 0.4 & 45.0 $\pm$ 3.0\\ 
328 & Tol1924-416 & 133.0 $\pm$ 6.0 & 9.4 $\pm$ 0.4 & 0.74 $\pm$ 0.05 & 810.0 $\pm$ 29.0 & 0.78 $\pm$ 0.04 & 19.0 $\pm$ 0.15 & 6.7 $\pm$ 0.4 & 47.0 $\pm$ 4.0\\ 
329 & NGC3125 & 154.0 $\pm$ 9.0 & 3.7 $\pm$ 0.2 & 0.27 $\pm$ 0.03 & 693.0 $\pm$ 28.0 & 0.5 $\pm$ 0.03 & 24.8 $\pm$ 0.1 & 8.8 $\pm$ 0.6 & 60.0 $\pm$ 6.0\\ 
330 & Mrk271 & 138.0 $\pm$ 7.0 & 9.3 $\pm$ 0.4 & 0.76 $\pm$ 0.08 & 844.0 $\pm$ 32.0 & 1.7 $\pm$ 0.26 & 25.7 $\pm$ 1.7 & 7.8 $\pm$ 0.5 & 39.0 $\pm$ 3.0\\ 
331 & Pox4 & 95.0 $\pm$ 4.0 & 9.9 $\pm$ 0.4 & 0.98 $\pm$ 0.07 & 922.0 $\pm$ 32.0 & 1.72 $\pm$ 0.04 & 15.2 $\pm$ 0.7 & 6.8 $\pm$ 0.4 & 45.0 $\pm$ 4.0\\ 
332 & J1253-0312 & 79.0 $\pm$ 4.0 & 9.7 $\pm$ 0.5 & 0.91 $\pm$ 0.08 & 866.0 $\pm$ 35.0 & 1.44 $\pm$ 0.09 & 14.2 $\pm$ 1.0 & 7.5 $\pm$ 0.5 & 50.0 $\pm$ 4.0\\ 
333 & Tol1457-262 & 178.0 $\pm$ 9.0 & 5.2 $\pm$ 0.2 & 4.3 $\pm$ 0.09 & 710.0 $\pm$ 25.0 & 1.5 $\pm$ 0.1 & 36.8 $\pm$ 1.6 & 8.3 $\pm$ 0.5 & 67.0 $\pm$ 5.0\\ 
334 & He2-10 & 215.0 $\pm$ 10.0 & 0.4 $\pm$ 0.06 & -& 180.0 $\pm$ 7.0 & 1.6 $\pm$ 0.1 & 39.0 $\pm$ 1.6 & 6.8 $\pm$ 0.4 & 90.0 $\pm$ 0.7\\ 
335 & NGC6822-V & 114.0 $\pm$ 6.0 & 5.5 $\pm$ 0.2 & 0.24 $\pm$ 0.02 & 722.0 $\pm$ 29.0 & 2.1 $\pm$ 0.1 & 13.7 $\pm$ 0.8 & 10.8 $\pm$ 0.7 & 52.0 $\pm$ 5.0\\ 
336 & KISSR0242 & 281.6 $\pm$ 11.5 & 5.1 $\pm$ 0.1 & -& 544.82 $\pm$ 11.4 & 1.6 $\pm$ 0.1 & 36.1 $\pm$ 0.9 & -& 50.3 $\pm$ 4.0\\ 
337 & KISSR0451 & 390.8 $\pm$ 16.4 & 2.8 $\pm$ 0.2 & -& 382.5 $\pm$ 8.3 & 1.6 $\pm$ 0.2 & 54.6 $\pm$ 1.8 & -& 62.2 $\pm$ 5.1\\ 
338 & KISSR0475 & 358.2 $\pm$ 14.7 & 1.8 $\pm$ 0.2 & -& 209.1 $\pm$ 6.0 & 0.94 $\pm$ 0.07 & 61.0 $\pm$ 2.0 & -& 57.8 $\pm$ 4.5\\ 
339 & KISSR0590 & 250.1 $\pm$ 14.6 & 3.0 $\pm$ 0.3 & -& 352.7 $\pm$ 7.9 & 2.1 $\pm$ 0.1 & 65.3 $\pm$ 0.9 & -& 56.4 $\pm$ 4.5\\ 
340 & KISSR0653 & 293.9 $\pm$ 12.2 & 1.3 $\pm$ 0.2 & -& 236.6 $\pm$ 5.1 & 2.51 $\pm$ 0.14 & 55.2 $\pm$ 1.06 & -& 83.9 $\pm$ 6.5\\ 
341 & KISSR1379 & 302.2 $\pm$ 12.5 & 1.9 $\pm$ 0.2 & -& 319.2 $\pm$ 6.8 & 2.43 $\pm$ 0.13 & 49.3 $\pm$ 0.92 & -& 36.3 $\pm$ 2.9\\ 
342 & KISSR1734 & 180.6 $\pm$ 7.3 & 7.6 $\pm$ 0.2 & 0.4 $\pm$ 0.1 & 663.5 $\pm$ 14.0 & 1.705 $\pm$ 0.099 & 31.2 $\pm$ 1.07 & 5.3 $\pm$ 0.3 & 42.0 $\pm$ 3.1\\ 
343 & KISSR2117 & 346.6 $\pm$ 14.2 & 1.5 $\pm$ 0.1 & -& 345.2 $\pm$ 7.5 & 1.53 $\pm$ 0.26 & 52.5 $\pm$ 2.8 & -& 67.3 $\pm$ 5.2\\ 
344 & KISSR2125 & 349.0 $\pm$ 15.6 & -& -& 99.7 $\pm$ 2.2 & 1.2 $\pm$ 0.1 & 72.9 $\pm$ 1.7 & -& 41.4 $\pm$ 3.7\\ 
345 & J0159+0751 & 16.15 $\pm$ 0.55 & 22.9 $\pm$ 0.68 & 3.62 $\pm$ 0.14 & 843.26 $\pm$ 24.17 & 1.0 $\pm$ 0.1 & 2.82 $\pm$ 2.6 & 1.83 $\pm$ 0.07 & 9.942 $\pm$ 0.516\\ 
346 & J1032+4919 & 27.86 $\pm$ 0.89 & 20.85 $\pm$ 0.61 & 2.37 $\pm$ 0.08 & 886.9 $\pm$ 25.31 & 1.0 $\pm$ 0.1 & 4.25 $\pm$ 2.8 & 2.54 $\pm$ 0.09 & 13.59 $\pm$ 0.54\\ 
347 & J1205+4551 & 18.26 $\pm$ 0.59 & 12.87 $\pm$ 0.38 & 1.2 $\pm$ 0.06 & 553.78 $\pm$ 15.88 & 1.3 $\pm$ 0.2 & 2.65 $\pm$ 3.1 & 1.03 $\pm$ 0.05 & 7.052 $\pm$ 0.344\\ 
348 & J0811+4730 & 16.75 $\pm$ 0.4 & 6.26 $\pm$ 0.2 & 0.58 $\pm$ 0.11 & 217.2 $\pm$ 3.29 & 0.9 $\pm$ 0.1 & 2.28 $\pm$ 2.6 & 0.84 $\pm$ 0.05 & 6.23 $\pm$ 0.52\\ 
349 & SHOC592 & 168.8 $\pm$ 16.88 & 3.63 $\pm$ 0.033 & 0.4305 $\pm$ 0.22 & 638.8 $\pm$ 1.96 & 1.1 $\pm$ 0.1 & 47.68 $\pm$ 2.3 & 9.923 $\pm$ 0.31 & 107.5 $\pm$ 2.32\\ 
350 & SHOC588 & 144.7 $\pm$ 14.7 & 3.822 $\pm$ 0.022 & 0.3647 $\pm$ 0.11 & 659.3 $\pm$ 6.7 & 1.5 $\pm$ 0.1 & 32.68 $\pm$ 1.4 & 8.14 $\pm$ 0.15 & 67.79 $\pm$ 1.07\\ 
351 & SHOC575 & 123.8 $\pm$ 2.5 & 4.22 $\pm$ 0.039 & -& 692.9 $\pm$ 4.61 & 0.9 $\pm$ 0.1 & 23.96 $\pm$ 2.4 & -& 75.23 $\pm$ 0.112\\ 
352 & SHOC579 & 77.1 $\pm$ 1.56 & 7.723 $\pm$ 0.078 & 0.6469 $\pm$ 0.066 & 825.6 $\pm$ 0.62 & 0.5 $\pm$ 0.1 & 19.29 $\pm$ 3.8 & 8.486 $\pm$ 0.056 & 55.62 $\pm$ 0.73\\








\hline                                                                             
\end{tabular}
\begin{tablenotes}
\centering
$^a$ Values normalized to I(H$\beta$)/100. 
\end{tablenotes}

\end{table*}
\newpage

==> Tables/Tabla_HII_referencias.tex <==
\begin{table*}
\centering
    \caption{References to published data sets for objects in the \HII Gal sub-sample of the present compilation.}
 \label{RefHII-2}
\begin{tabular}{cccc}
\hline
ID & Telescope+Instrument & Reference\\ \hline

257-258 & Large Cass  McDonal(2.7m)+MMT(6.2m) Spectrograph & \citet{1993ApJ...411..655S}\\ 
259 & ISIS+WHT (4.2m) + MMT(6.2m) & \citet{1994ApJ...431..172S}\\ 
260-270 & IDS+INT(2.5m) & \citet{2003MNRAS.346..105P}\\ 
271-273 & ISIS+WHT(4.2m) & \citet{2006MNRAS.372..293H}\\ 
274-277 & UVES+VLT(8.2m) & \citet{2007ApJ...656..168L}\\ 
278-284 & ISIS+WHT(4.2m) & \citet{2008MNRAS.383..209H}\\ 
285-287 & FORS+UVES+VLT(8.2m) & \citet{2009AandA...503...61I}\\ 
288 & TRIPLESPEC+APO Telescope (3.5m)+SDSS & \citet{2009ApJ...703.1984I}\\ 
289 & FORS+UVES+VLT(8.2m) & \citet{2010AandA...517A..90I}\\ 
290-311 & FORS+UVES+VLT(8.2m) & \citet{2011AandA...529A.149G}\\ 
312 & FORS+UVES+VLT(8.2m) & \citet{2011AandA...534A..84G}\\ 
313-315 & DIS + TRIPLESPEC+APO Telescope (3.5m) & \citet{2011ApJ...734...82I}\\ 
316-318 & XSHOOTER+VLT(8.2m) & \citet{2012AandA...541A.115G}\\ 
319-326 & DIS +APO Telescope (3.5m)+MMT(6.2m) Spectrograph & \citet{2012AandA...546A.122I}\\ 
327-335 & UVES+VLT(8.2m) & \citet{2014MNRAS.443..624E}\\ 
336-344 & LRIS+Keck(10m) & \citet{2015AJ....150...71H}\\ 
345-347 & LBT(8.4m)+MODS & \citet{2017MNRAS.471..548I}\\ 
348 & LBT(8.4m)+MODS & \citet{2018MNRAS.473.1956I}\\ 
349-352 & ISIS+WHT(4.2m) & \citet{2018MNRAS.478.5301F}\\ 



 \hline     
\end{tabular}
\end{table*}
\newpage

==> Tables/Tabla_HII_resultados_O.tex <==
\begin{table*}
\centering
\caption{Oxygen electron temperature and ionic abundances of objects in sub-sample \HII Gal.}
\label{OresHII}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([OIII])$^a$ & 12+log(O$^{+}$/H$^{+}$)&	12+log(O$^{++}$/H$^{+}$) & 12+log(O/H)
\\ \hline


257 & 1.62 $\pm$ 0.133 & 6.0 $\pm$ 0.06 & 7.25 $\pm$ 0.07 & 7.27 $\pm$ 0.06\\ 
258 & 2.092 $\pm$ 0.091 & 6.54 $\pm$ 0.07 & 6.95 $\pm$ 0.03 & 7.09 $\pm$ 0.03\\ 
259 & 1.681 $\pm$ 0.058 & 6.75 $\pm$ 0.11 & 7.35 $\pm$ 0.03 & 7.45 $\pm$ 0.03\\ 
260 & 1.208 $\pm$ 0.05 & 7.41 $\pm$ 0.11 & 7.88 $\pm$ 0.04 & 8.01 $\pm$ 0.04\\ 
261 & 1.524 $\pm$ 0.083 & 6.92 $\pm$ 0.11 & 7.71 $\pm$ 0.05 & 7.78 $\pm$ 0.04\\ 
262 & 1.426 $\pm$ 0.023 & 7.14 $\pm$ 0.09 & 7.78 $\pm$ 0.01 & 7.87 $\pm$ 0.02\\ 
263 & 1.615 $\pm$ 0.048 & 7.05 $\pm$ 0.09 & 7.55 $\pm$ 0.02 & 7.67 $\pm$ 0.03\\ 
264 & 1.342 $\pm$ 0.021 & 6.78 $\pm$ 0.09 & 7.9 $\pm$ 0.01 & 7.93 $\pm$ 0.01\\ 
265 & 1.548 $\pm$ 0.015 & 6.71 $\pm$ 0.07 & 7.71 $\pm$ 0.01 & 7.75 $\pm$ 0.01\\ 
266 & 1.519 $\pm$ 0.038 & 6.96 $\pm$ 0.11 & 7.71 $\pm$ 0.02 & 7.78 $\pm$ 0.02\\ 
267 & 1.547 $\pm$ 0.023 & 7.23 $\pm$ 0.1 & 7.54 $\pm$ 0.01 & 7.71 $\pm$ 0.03\\ 
268 & 1.617 $\pm$ 0.044 & 6.33 $\pm$ 0.04 & 7.74 $\pm$ 0.02 & 7.76 $\pm$ 0.02\\ 
269 & 1.37 $\pm$ 0.015 & 7.04 $\pm$ 0.1 & 7.84 $\pm$ 0.01 & 7.9 $\pm$ 0.02\\ 
270 & 1.62 $\pm$ 0.007 & 6.67 $\pm$ 0.08 & 7.71 $\pm$ 0.0 & 7.75 $\pm$ 0.01\\ 
271 & 1.24 $\pm$ 0.014 & 7.13 $\pm$ 0.04 & 8.02 $\pm$ 0.01 & 8.07 $\pm$ 0.01\\ 
272 & 1.256 $\pm$ 0.026 & 7.28 $\pm$ 0.07 & 7.89 $\pm$ 0.02 & 7.99 $\pm$ 0.02\\ 
273 & 1.279 $\pm$ 0.025 & 7.24 $\pm$ 0.06 & 7.89 $\pm$ 0.02 & 7.98 $\pm$ 0.02\\ 
274 & 1.19 $\pm$ 0.02 & 7.43 $\pm$ 0.09 & 8.08 $\pm$ 0.02 & 8.17 $\pm$ 0.02\\ 
275 & 1.011 $\pm$ 0.019 & 7.38 $\pm$ 0.08 & 8.32 $\pm$ 0.03 & 8.37 $\pm$ 0.02\\ 
276 & 0.968 $\pm$ 0.018 & 7.65 $\pm$ 0.09 & 8.28 $\pm$ 0.03 & 8.37 $\pm$ 0.03\\ 
277 & 1.096 $\pm$ 0.043 & 7.88 $\pm$ 0.15 & 7.91 $\pm$ 0.05 & 8.2 $\pm$ 0.07\\ 
278 & 1.087 $\pm$ 0.017 & 7.68 $\pm$ 0.06 & 8.14 $\pm$ 0.02 & 8.27 $\pm$ 0.02\\ 
279 & 1.235 $\pm$ 0.021 & 7.21 $\pm$ 0.06 & 7.9 $\pm$ 0.02 & 7.98 $\pm$ 0.02\\ 
280 & 1.554 $\pm$ 0.027 & 7.55 $\pm$ 0.07 & 7.69 $\pm$ 0.01 & 7.93 $\pm$ 0.03\\ 
281 & 1.383 $\pm$ 0.036 & 7.05 $\pm$ 0.06 & 7.92 $\pm$ 0.02 & 7.97 $\pm$ 0.02\\ 
282 & 1.126 $\pm$ 0.022 & 7.91 $\pm$ 0.07 & 7.88 $\pm$ 0.02 & 8.2 $\pm$ 0.03\\ 
283 & 1.297 $\pm$ 0.016 & 7.0 $\pm$ 0.05 & 8.0 $\pm$ 0.01 & 8.04 $\pm$ 0.01\\ 
284 & 1.259 $\pm$ 0.018 & 7.52 $\pm$ 0.06 & 7.95 $\pm$ 0.01 & 8.09 $\pm$ 0.02\\ 
285 & 2.071 $\pm$ 0.026 & 6.44 $\pm$ 0.05 & 7.21 $\pm$ 0.01 & 7.28 $\pm$ 0.01\\ 
286 & 2.024 $\pm$ 0.031 & 5.89 $\pm$ 0.07 & 7.26 $\pm$ 0.01 & 7.28 $\pm$ 0.01\\ 
287 & 1.908 $\pm$ 0.097 & 5.64 $\pm$ 0.02 & 7.19 $\pm$ 0.04 & 7.2 $\pm$ 0.03\\ 
288 & 1.304 $\pm$ 0.024 & 7.07 $\pm$ 0.05 & 7.98 $\pm$ 0.02 & 8.03 $\pm$ 0.02\\ 
289 & 1.604 $\pm$ 0.021 & 6.7 $\pm$ 0.06 & 7.79 $\pm$ 0.01 & 7.82 $\pm$ 0.01\\ 
290 & 1.228 $\pm$ 0.033 & 7.78 $\pm$ 0.06 & 7.81 $\pm$ 0.03 & 8.1 $\pm$ 0.03\\ 
291 & 1.554 $\pm$ 0.026 & 6.62 $\pm$ 0.04 & 7.57 $\pm$ 0.02 & 7.62 $\pm$ 0.01\\ 
292 & 1.234 $\pm$ 0.022 & 8.61 $\pm$ 0.03 & 7.48 $\pm$ 0.02 & 8.64 $\pm$ 0.02\\ 
293 & 0.739 $\pm$ 0.045 & 8.58 $\pm$ 0.04 & 8.17 $\pm$ 0.1 & 8.72 $\pm$ 0.04\\ 
294 & 1.104 $\pm$ 0.007 & 7.55 $\pm$ 0.02 & 8.18 $\pm$ 0.01 & 8.27 $\pm$ 0.01\\ 
295 & 1.014 $\pm$ 0.032 & 8.36 $\pm$ 0.03 & 7.75 $\pm$ 0.04 & 8.46 $\pm$ 0.02\\ 
296 & 1.302 $\pm$ 0.011 & 6.86 $\pm$ 0.02 & 8.02 $\pm$ 0.01 & 8.05 $\pm$ 0.01\\ 
297 & 2.024 $\pm$ 0.026 & 5.82 $\pm$ 0.03 & 7.45 $\pm$ 0.01 & 7.46 $\pm$ 0.01\\ 
298 & 1.383 $\pm$ 0.012 & 7.05 $\pm$ 0.02 & 7.94 $\pm$ 0.01 & 7.99 $\pm$ 0.01\\ 
299 & 1.221 $\pm$ 0.009 & 7.15 $\pm$ 0.02 & 8.08 $\pm$ 0.01 & 8.13 $\pm$ 0.01\\ 
300 & 1.026 $\pm$ 0.006 & 7.44 $\pm$ 0.02 & 8.17 $\pm$ 0.01 & 8.24 $\pm$ 0.01\\ 
301 & - & 7.55 $\pm$ 0.03 & - & -\\ 
302 & 1.235 $\pm$ 0.01 & 7.13 $\pm$ 0.02 & 8.08 $\pm$ 0.01 & 8.13 $\pm$ 0.01\\ 
303 & 1.026 $\pm$ 0.007 & 7.71 $\pm$ 0.02 & 8.21 $\pm$ 0.01 & 8.33 $\pm$ 0.01\\ 
304 & 0.944 $\pm$ 0.014 & 8.45 $\pm$ 0.04 & 8.23 $\pm$ 0.02 & 8.65 $\pm$ 0.03\\ 
305 & 1.563 $\pm$ 0.015 & 6.73 $\pm$ 0.02 & 7.97 $\pm$ 0.01 & 7.99 $\pm$ 0.01\\ 
306 & 1.362 $\pm$ 0.012 & 7.02 $\pm$ 0.02 & 8.03 $\pm$ 0.01 & 8.07 $\pm$ 0.01\\ 
307 & 1.182 $\pm$ 0.009 & 7.54 $\pm$ 0.02 & 8.12 $\pm$ 0.01 & 8.22 $\pm$ 0.01\\ 
308 & 1.241 $\pm$ 0.011 & 7.16 $\pm$ 0.02 & 7.9 $\pm$ 0.01 & 7.97 $\pm$ 0.01\\ 
309 & 1.22 $\pm$ 0.009 & 7.08 $\pm$ 0.02 & 8.01 $\pm$ 0.01 & 8.05 $\pm$ 0.01\\ 
310 & 1.137 $\pm$ 0.008 & 7.2 $\pm$ 0.02 & 8.11 $\pm$ 0.01 & 8.16 $\pm$ 0.01\\ 
311 & 1.769 $\pm$ 0.023 & 6.66 $\pm$ 0.09 & 7.6 $\pm$ 0.01 & 7.65 $\pm$ 0.01\\ 
312 & 1.212 $\pm$ 0.032 & 7.18 $\pm$ 0.06 & 8.16 $\pm$ 0.03 & 8.2 $\pm$ 0.02\\ 
313 & 1.617 $\pm$ 0.033 & 6.5 $\pm$ 0.09 & 7.82 $\pm$ 0.02 & 7.84 $\pm$ 0.02\\ 
314 & 1.243 $\pm$ 0.047 & 7.53 $\pm$ 0.12 & 7.88 $\pm$ 0.04 & 8.04 $\pm$ 0.04\\ 
315 & 1.44 $\pm$ 0.037 & 6.81 $\pm$ 0.03 & 7.94 $\pm$ 0.02 & 7.97 $\pm$ 0.02\\ 
316 & 1.015 $\pm$ 0.007 & 8.08 $\pm$ 0.02 & 8.1 $\pm$ 0.01 & 8.39 $\pm$ 0.01\\ 

 
  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID & t$_e$([OIII])$^a$ & 12+log(O$^{+}$/H$^{+}$)&	12+log(O$^{++}$/H$^{+}$) & 12+log(O/H)
\\ \hline 
 
317 & 1.131 $\pm$ 0.043 & 8.32 $\pm$ 0.12 & 7.88 $\pm$ 0.04 & 8.45 $\pm$ 0.08\\ 
318 & 1.477 $\pm$ 0.048 & 7.51 $\pm$ 0.04 & 7.77 $\pm$ 0.03 & 7.96 $\pm$ 0.02\\ 
319 & 0.981 $\pm$ 0.06 & 6.81 $\pm$ 0.11 & 8.2 $\pm$ 0.08 & 8.22 $\pm$ 0.07\\ 
320 & 1.629 $\pm$ 0.029 & 6.72 $\pm$ 0.05 & 7.7 $\pm$ 0.02 & 7.74 $\pm$ 0.01\\ 
321 & 1.512 $\pm$ 0.026 & 6.63 $\pm$ 0.04 & 7.74 $\pm$ 0.02 & 7.77 $\pm$ 0.01\\ 
322 & 1.4 $\pm$ 0.037 & 7.47 $\pm$ 0.09 & 7.65 $\pm$ 0.02 & 7.87 $\pm$ 0.04\\ 
323 & 1.548 $\pm$ 0.057 & 7.54 $\pm$ 0.08 & 7.55 $\pm$ 0.03 & 7.85 $\pm$ 0.04\\ 
324 & 1.664 $\pm$ 0.027 & 6.87 $\pm$ 0.05 & 7.63 $\pm$ 0.01 & 7.7 $\pm$ 0.01\\ 
325 & 1.65 $\pm$ 0.029 & 6.83 $\pm$ 0.09 & 7.76 $\pm$ 0.02 & 7.81 $\pm$ 0.02\\ 
326 & 1.729 $\pm$ 0.034 & 6.7 $\pm$ 0.09 & 7.56 $\pm$ 0.02 & 7.61 $\pm$ 0.02\\ 
327 & 1.563 $\pm$ 0.038 & 6.9 $\pm$ 0.05 & 7.75 $\pm$ 0.02 & 7.81 $\pm$ 0.02\\ 
328 & 1.359 $\pm$ 0.032 & 7.27 $\pm$ 0.08 & 7.93 $\pm$ 0.03 & 8.02 $\pm$ 0.03\\ 
329 & 1.035 $\pm$ 0.02 & 7.51 $\pm$ 0.09 & 8.22 $\pm$ 0.03 & 8.3 $\pm$ 0.03\\ 
330 & 1.33 $\pm$ 0.031 & 7.04 $\pm$ 0.07 & 7.98 $\pm$ 0.03 & 8.03 $\pm$ 0.03\\ 
331 & 1.316 $\pm$ 0.029 & 6.77 $\pm$ 0.07 & 8.03 $\pm$ 0.03 & 8.05 $\pm$ 0.02\\ 
332 & 1.339 $\pm$ 0.036 & 7.01 $\pm$ 0.08 & 7.98 $\pm$ 0.03 & 8.03 $\pm$ 0.03\\ 
333 & 1.142 $\pm$ 0.02 & 7.62 $\pm$ 0.11 & 8.1 $\pm$ 0.02 & 8.22 $\pm$ 0.03\\ 
334 & 0.821 $\pm$ 0.034 & 8.38 $\pm$ 0.06 & 8.01 $\pm$ 0.06 & 8.54 $\pm$ 0.04\\ 
335 & 1.157 $\pm$ 0.021 & 6.97 $\pm$ 0.08 & 8.09 $\pm$ 0.03 & 8.12 $\pm$ 0.02\\ 
336 & 1.246 $\pm$ 0.014 & 7.82 $\pm$ 0.09 & 7.87 $\pm$ 0.01 & 8.14 $\pm$ 0.04\\ 
337 & 1.142 $\pm$ 0.029 & 8.3 $\pm$ 0.1 & 7.83 $\pm$ 0.03 & 8.43 $\pm$ 0.07\\ 
338 & 1.208 $\pm$ 0.05 & 8.2 $\pm$ 0.1 & 7.49 $\pm$ 0.04 & 8.28 $\pm$ 0.07\\ 
339 & 1.203 $\pm$ 0.045 & 7.8 $\pm$ 0.13 & 7.72 $\pm$ 0.04 & 8.06 $\pm$ 0.07\\ 
340 & 1.043 $\pm$ 0.048 & 8.5 $\pm$ 0.1 & 7.74 $\pm$ 0.05 & 8.57 $\pm$ 0.07\\ 
341 & 1.069 $\pm$ 0.035 & 7.64 $\pm$ 0.09 & 7.84 $\pm$ 0.04 & 8.05 $\pm$ 0.04\\ 
342 & 1.351 $\pm$ 0.019 & 7.27 $\pm$ 0.07 & 7.85 $\pm$ 0.02 & 7.96 $\pm$ 0.02\\ 
343 & 0.977 $\pm$ 0.019 & 8.4 $\pm$ 0.1 & 8.01 $\pm$ 0.03 & 8.55 $\pm$ 0.07\\ 
345 & 2.114 $\pm$ 0.054 & 5.76 $\pm$ 0.05 & 7.51 $\pm$ 0.02 & 7.51 $\pm$ 0.02\\ 
346 & 1.938 $\pm$ 0.046 & 6.07 $\pm$ 0.04 & 7.6 $\pm$ 0.02 & 7.62 $\pm$ 0.02\\ 
347 & 1.925 $\pm$ 0.046 & 5.72 $\pm$ 0.05 & 7.41 $\pm$ 0.02 & 7.41 $\pm$ 0.02\\ 
348 & 2.194 $\pm$ 0.049 & 5.74 $\pm$ 0.1 & 6.88 $\pm$ 0.02 & 6.91 $\pm$ 0.02\\ 
349 & 1.054 $\pm$ 0.003 & 7.84 $\pm$ 0.14 & 8.16 $\pm$ 0.0 & 8.33 $\pm$ 0.04\\ 
350 & 1.06 $\pm$ 0.004 & 7.36 $\pm$ 0.06 & 8.17 $\pm$ 0.01 & 8.23 $\pm$ 0.01\\ 
351 & 1.076 $\pm$ 0.004 & 7.41 $\pm$ 0.07 & 8.17 $\pm$ 0.0 & 8.24 $\pm$ 0.01\\ 
352 & 1.246 $\pm$ 0.005 & 7.0 $\pm$ 0.02 & 8.05 $\pm$ 0.0 & 8.09 $\pm$ 0.0\\







 

 





 
 

 
 
 



\hline

\end{tabular}
\begin{tablenotes}

$^a$ In units of 10$^{4}$K.\\
    
\end{tablenotes}
\end{table*}
\newpage

==> Tables/Tabla_HII_resultados_S.tex <==
\begin{table*}
\centering
\caption{Sulphur electron temperature and ionic abundances of objects in sub-sample \HII Gal.}
\label{SresHII}
\begin{tabular}{ccccc}
\hline

ID  & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) &  12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline

257 & 1.94 $\pm$ 0.116 & 4.39 $\pm$ 0.03 & 5.18 $\pm$ 0.03 & 5.25 $\pm$ 0.02\\ 
258 & 1.518 $\pm$ 0.088 & 4.86 $\pm$ 0.04 & 5.46 $\pm$ 0.03 & 5.56 $\pm$ 0.03\\ 
259 & 1.562 $\pm$ 0.154 & 5.08 $\pm$ 0.06 & 5.77 $\pm$ 0.08 & 5.85 $\pm$ 0.06\\ 
260 & 1.308 $\pm$ 0.109 & 5.71 $\pm$ 0.06 & 6.12 $\pm$ 0.05 & 6.27 $\pm$ 0.04\\ 
261 & 1.749 $\pm$ 0.204 & 5.27 $\pm$ 0.06 & 5.88 $\pm$ 0.07 & 5.97 $\pm$ 0.05\\ 
262 & 1.495 $\pm$ 0.123 & 5.53 $\pm$ 0.05 & 6.03 $\pm$ 0.06 & 6.15 $\pm$ 0.05\\ 
263 & 1.616 $\pm$ 0.144 & 5.76 $\pm$ 0.05 & 5.76 $\pm$ 0.06 & 6.06 $\pm$ 0.04\\ 
264 & 1.892 $\pm$ 0.186 & 5.28 $\pm$ 0.05 & 5.89 $\pm$ 0.07 & 5.99 $\pm$ 0.05\\ 
265 & 1.702 $\pm$ 0.123 & 5.1 $\pm$ 0.04 & 5.75 $\pm$ 0.05 & 5.84 $\pm$ 0.04\\ 
266 & 1.541 $\pm$ 0.161 & 5.3 $\pm$ 0.06 & 5.94 $\pm$ 0.07 & 6.03 $\pm$ 0.05\\ 
267 & 1.286 $\pm$ 0.1 & 5.26 $\pm$ 0.06 & 6.06 $\pm$ 0.06 & 6.12 $\pm$ 0.05\\ 
268 & 1.886 $\pm$ 0.089 & 4.87 $\pm$ 0.03 & 5.72 $\pm$ 0.03 & 5.78 $\pm$ 0.02\\ 
269 & 1.602 $\pm$ 0.154 & 5.42 $\pm$ 0.06 & 5.95 $\pm$ 0.07 & 6.06 $\pm$ 0.05\\ 
270 & 1.581 $\pm$ 0.115 & 5.0 $\pm$ 0.05 & 5.93 $\pm$ 0.05 & 5.98 $\pm$ 0.05\\ 
271 & 1.421 $\pm$ 0.048 & 5.44 $\pm$ 0.02 & 6.05 $\pm$ 0.03 & 6.15 $\pm$ 0.02\\ 
272 & 1.314 $\pm$ 0.071 & 5.52 $\pm$ 0.04 & 5.99 $\pm$ 0.03 & 6.12 $\pm$ 0.03\\ 
273 & 1.342 $\pm$ 0.067 & 5.59 $\pm$ 0.04 & 6.24 $\pm$ 0.04 & 6.33 $\pm$ 0.03\\ 
274 & 1.145 $\pm$ 0.07 & 5.67 $\pm$ 0.05 & 6.53 $\pm$ 0.06 & 6.59 $\pm$ 0.05\\ 
275 & 1.17 $\pm$ 0.067 & 5.59 $\pm$ 0.05 & 6.48 $\pm$ 0.05 & 6.53 $\pm$ 0.04\\ 
276 & 1.082 $\pm$ 0.062 & 5.73 $\pm$ 0.05 & 6.46 $\pm$ 0.06 & 6.53 $\pm$ 0.04\\ 
277 & 1.115 $\pm$ 0.112 & 6.1 $\pm$ 0.08 & 6.36 $\pm$ 0.07 & 6.55 $\pm$ 0.05\\ 
278 & 1.02 $\pm$ 0.038 & 5.92 $\pm$ 0.03 & 6.54 $\pm$ 0.03 & 6.63 $\pm$ 0.03\\ 
279 & 1.449 $\pm$ 0.078 & 5.63 $\pm$ 0.04 & 6.07 $\pm$ 0.04 & 6.2 $\pm$ 0.03\\ 
280 & 1.213 $\pm$ 0.062 & 5.73 $\pm$ 0.04 & 6.27 $\pm$ 0.04 & 6.38 $\pm$ 0.03\\ 
281 & 1.373 $\pm$ 0.065 & 5.35 $\pm$ 0.03 & 6.05 $\pm$ 0.03 & 6.13 $\pm$ 0.03\\ 
282 & 0.977 $\pm$ 0.039 & 6.08 $\pm$ 0.04 & 6.56 $\pm$ 0.04 & 6.68 $\pm$ 0.03\\ 
283 & 1.315 $\pm$ 0.049 & 5.26 $\pm$ 0.03 & 6.19 $\pm$ 0.03 & 6.24 $\pm$ 0.02\\ 
284 & 1.152 $\pm$ 0.045 & 5.62 $\pm$ 0.03 & 6.38 $\pm$ 0.03 & 6.45 $\pm$ 0.03\\ 
285 & 1.337 $\pm$ 0.049 & 4.63 $\pm$ 0.03 & 5.63 $\pm$ 0.02 & 5.67 $\pm$ 0.02\\ 
286 & 2.063 $\pm$ 0.172 & 4.26 $\pm$ 0.04 & 5.12 $\pm$ 0.04 & 5.17 $\pm$ 0.04\\ 
287 & 2.387 $\pm$ 0.074 & 4.25 $\pm$ 0.02 & 4.95 $\pm$ 0.02 & 5.03 $\pm$ 0.01\\ 
288 & 1.364 $\pm$ 0.049 & 5.3 $\pm$ 0.03 & 6.12 $\pm$ 0.02 & 6.18 $\pm$ 0.02\\ 
289 & 1.647 $\pm$ 0.096 & 4.95 $\pm$ 0.09 & 5.67 $\pm$ 0.04 & 5.74 $\pm$ 0.04\\ 
290 & 1.129 $\pm$ 0.045 & 5.97 $\pm$ 0.03 & 6.41 $\pm$ 0.03 & 6.55 $\pm$ 0.02\\ 
291 & 1.925 $\pm$ 0.077 & 5.05 $\pm$ 0.02 & 5.58 $\pm$ 0.02 & 5.69 $\pm$ 0.02\\ 
292 & 0.709 $\pm$ 0.008 & 6.35 $\pm$ 0.02 & 7.09 $\pm$ 0.01 & 7.16 $\pm$ 0.01\\ 
293 & 0.707 $\pm$ 0.011 & 6.32 $\pm$ 0.02 & 7.0 $\pm$ 0.02 & 7.09 $\pm$ 0.01\\ 
294 & 0.974 $\pm$ 0.012 & 5.77 $\pm$ 0.01 & 6.73 $\pm$ 0.01 & 6.78 $\pm$ 0.01\\ 
295 & 0.754 $\pm$ 0.01 & 6.28 $\pm$ 0.02 & 6.86 $\pm$ 0.01 & 6.96 $\pm$ 0.01\\ 
296 & 1.433 $\pm$ 0.023 & 5.19 $\pm$ 0.01 & 6.0 $\pm$ 0.01 & 6.06 $\pm$ 0.01\\ 
297 & 2.477 $\pm$ 0.106 & 4.24 $\pm$ 0.02 & 5.02 $\pm$ 0.02 & 5.09 $\pm$ 0.02\\ 
298 & 1.268 $\pm$ 0.02 & 5.21 $\pm$ 0.01 & 6.14 $\pm$ 0.01 & 6.19 $\pm$ 0.01\\ 
299 & 1.235 $\pm$ 0.017 & 5.38 $\pm$ 0.01 & 6.37 $\pm$ 0.01 & 6.42 $\pm$ 0.01\\ 
300 & 1.158 $\pm$ 0.017 & 5.68 $\pm$ 0.01 & 6.41 $\pm$ 0.01 & 6.48 $\pm$ 0.01\\ 
301 & 1.13 $\pm$ 0.019 & 5.55 $\pm$ 0.02 & 6.42 $\pm$ 0.01 & 6.48 $\pm$ 0.01\\ 
302 & 1.284 $\pm$ 0.02 & 5.33 $\pm$ 0.01 & 6.35 $\pm$ 0.01 & 6.39 $\pm$ 0.01\\ 
303 & 0.999 $\pm$ 0.012 & 5.72 $\pm$ 0.01 & 6.6 $\pm$ 0.01 & 6.65 $\pm$ 0.01\\ 
304 & 0.718 $\pm$ 0.013 & 6.45 $\pm$ 0.02 & 7.24 $\pm$ 0.02 & 7.31 $\pm$ 0.02\\ 
305 & 1.801 $\pm$ 0.029 & 4.96 $\pm$ 0.01 & 5.78 $\pm$ 0.01 & 5.84 $\pm$ 0.01\\ 
306 & 1.706 $\pm$ 0.03 & 5.35 $\pm$ 0.01 & 5.98 $\pm$ 0.01 & 6.07 $\pm$ 0.01\\ 
307 & 1.27 $\pm$ 0.02 & 5.49 $\pm$ 0.01 & 6.14 $\pm$ 0.01 & 6.23 $\pm$ 0.01\\ 
308 & 1.223 $\pm$ 0.02 & 5.42 $\pm$ 0.01 & 6.15 $\pm$ 0.01 & 6.22 $\pm$ 0.01\\ 
309 & 1.36 $\pm$ 0.021 & 5.39 $\pm$ 0.01 & 6.09 $\pm$ 0.01 & 6.17 $\pm$ 0.01\\ 
310 & 1.136 $\pm$ 0.015 & 5.29 $\pm$ 0.01 & 6.5 $\pm$ 0.01 & 6.53 $\pm$ 0.01\\ 
311 & 1.433 $\pm$ 0.109 & 4.95 $\pm$ 0.06 & 5.89 $\pm$ 0.04 & 5.94 $\pm$ 0.04\\ 
312 & 1.171 $\pm$ 0.043 & 5.43 $\pm$ 0.03 & 6.27 $\pm$ 0.02 & 6.33 $\pm$ 0.02\\ 
313 & 1.534 $\pm$ 0.12 & 4.81 $\pm$ 0.06 & 5.82 $\pm$ 0.04 & 5.86 $\pm$ 0.04\\ 
314 & 1.267 $\pm$ 0.112 & 5.83 $\pm$ 0.07 & 6.2 $\pm$ 0.05 & 6.35 $\pm$ 0.04\\ 
315 & 1.344 $\pm$ 0.029 & 5.07 $\pm$ 0.03 & 6.02 $\pm$ 0.02 & 6.07 $\pm$ 0.01\\ 
316 & 0.899 $\pm$ 0.012 & 5.93 $\pm$ 0.01 & 6.62 $\pm$ 0.01 & 6.7 $\pm$ 0.01\\ 




 \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccc}
\hline
ID  & t$_e$([SIII])$^a$ & 12+log(S$^{+}$/H$^{+}$)&	12+log(S$^{++}$/H$^{+}$) &  12+log((S$^{+}$+S$^{++}$)/H$^{+}$)
\\ \hline 
 
317 & 0.815 $\pm$ 0.049 & 6.27 $\pm$ 0.07 & 6.81 $\pm$ 0.05 & 6.92 $\pm$ 0.04\\ 
318 & 1.091 $\pm$ 0.026 & 5.6 $\pm$ 0.02 & 6.33 $\pm$ 0.02 & 6.41 $\pm$ 0.01\\ 
319 & 1.534 $\pm$ 0.152 & 5.38 $\pm$ 0.06 & 5.91 $\pm$ 0.05 & 6.03 $\pm$ 0.04\\ 
320 & 1.677 $\pm$ 0.074 & 5.17 $\pm$ 0.03 & 5.76 $\pm$ 0.02 & 5.86 $\pm$ 0.02\\ 
321 & 1.755 $\pm$ 0.078 & 5.13 $\pm$ 0.03 & 5.74 $\pm$ 0.02 & 5.84 $\pm$ 0.02\\ 
322 & 1.213 $\pm$ 0.083 & 5.56 $\pm$ 0.05 & 6.13 $\pm$ 0.04 & 6.24 $\pm$ 0.03\\ 
323 & 1.229 $\pm$ 0.076 & 5.57 $\pm$ 0.05 & 6.17 $\pm$ 0.04 & 6.26 $\pm$ 0.03\\ 
324 & 1.648 $\pm$ 0.077 & 5.19 $\pm$ 0.03 & 5.82 $\pm$ 0.02 & 5.91 $\pm$ 0.02\\ 
325 & 1.316 $\pm$ 0.089 & 5.08 $\pm$ 0.05 & 5.98 $\pm$ 0.04 & 6.03 $\pm$ 0.04\\ 
70 & 1.796 $\pm$ 0.173 & 4.97 $\pm$ 0.05 & 5.51 $\pm$ 0.05 & 5.62 $\pm$ 0.04\\ 
327 & 1.421 $\pm$ 0.061 & 5.19 $\pm$ 0.04 & 6.03 $\pm$ 0.04 & 6.09 $\pm$ 0.03\\ 
328 & 1.248 $\pm$ 0.074 & 5.46 $\pm$ 0.05 & 6.15 $\pm$ 0.05 & 6.23 $\pm$ 0.04\\ 
73 & 1.119 $\pm$ 0.069 & 5.68 $\pm$ 0.06 & 6.35 $\pm$ 0.06 & 6.43 $\pm$ 0.05\\ 
330 & 1.485 $\pm$ 0.093 & 5.44 $\pm$ 0.05 & 5.94 $\pm$ 0.05 & 6.06 $\pm$ 0.03\\ 
75 & 1.613 $\pm$ 0.107 & 5.15 $\pm$ 0.04 & 5.94 $\pm$ 0.05 & 6.01 $\pm$ 0.04\\ 
76 & 1.279 $\pm$ 0.074 & 5.31 $\pm$ 0.05 & 6.16 $\pm$ 0.05 & 6.22 $\pm$ 0.04\\ 
77 & 1.093 $\pm$ 0.08 & 5.87 $\pm$ 0.06 & 6.41 $\pm$ 0.06 & 6.52 $\pm$ 0.04\\ 
334 & 0.779 $\pm$ 0.019 & 6.29 $\pm$ 0.04 & 6.87 $\pm$ 0.02 & 6.97 $\pm$ 0.02\\ 
79 & 1.47 $\pm$ 0.099 & 5.17 $\pm$ 0.05 & 6.07 $\pm$ 0.05 & 6.12 $\pm$ 0.04\\ 
336 & 1.093 $\pm$ 0.063 & 5.86 $\pm$ 0.05 & 6.29 $\pm$ 0.05 & 6.43 $\pm$ 0.04\\ 
337 & 0.913 $\pm$ 0.049 & 6.24 $\pm$ 0.06 & 6.55 $\pm$ 0.05 & 6.72 $\pm$ 0.04\\ 
338 & 0.941 $\pm$ 0.051 & 6.25 $\pm$ 0.06 & 6.49 $\pm$ 0.05 & 6.69 $\pm$ 0.04\\ 
339 & 1.074 $\pm$ 0.092 & 6.14 $\pm$ 0.08 & 6.35 $\pm$ 0.06 & 6.56 $\pm$ 0.05\\ 
340 & 0.786 $\pm$ 0.035 & 6.43 $\pm$ 0.05 & 6.83 $\pm$ 0.05 & 6.98 $\pm$ 0.04\\ 
341 & 1.24 $\pm$ 0.084 & 5.88 $\pm$ 0.05 & 6.04 $\pm$ 0.05 & 6.27 $\pm$ 0.04\\ 
342 & 1.364 $\pm$ 0.081 & 5.59 $\pm$ 0.04 & 6.03 $\pm$ 0.04 & 6.17 $\pm$ 0.03\\ 
343 & 0.849 $\pm$ 0.043 & 6.31 $\pm$ 0.06 & 6.65 $\pm$ 0.05 & 6.82 $\pm$ 0.04\\ 
344 & 0.818 $\pm$ 0.063 & 6.5 $\pm$ 0.09 & 6.48 $\pm$ 0.07 & 6.79 $\pm$ 0.05\\ 
345 & 1.993 $\pm$ 0.118 & 4.27 $\pm$ 0.03 & 5.15 $\pm$ 0.03 & 5.2 $\pm$ 0.03\\ 
346 & 1.857 $\pm$ 0.085 & 4.49 $\pm$ 0.03 & 5.33 $\pm$ 0.03 & 5.39 $\pm$ 0.02\\ 
347 & 2.164 $\pm$ 0.124 & 4.19 $\pm$ 0.03 & 4.95 $\pm$ 0.03 & 5.02 $\pm$ 0.03\\ 
348 & 2.048 $\pm$ 0.252 & 4.16 $\pm$ 0.06 & 4.93 $\pm$ 0.06 & 5.0 $\pm$ 0.05\\ 
349 & 0.956 $\pm$ 0.076 & 6.13 $\pm$ 0.08 & 6.74 $\pm$ 0.06 & 6.83 $\pm$ 0.05\\ 
350 & 1.207 $\pm$ 0.042 & 5.72 $\pm$ 0.03 & 6.34 $\pm$ 0.02 & 6.43 $\pm$ 0.02\\ 
351 & 1.123 $\pm$ 0.055 & 5.66 $\pm$ 0.04 & 6.44 $\pm$ 0.03 & 6.51 $\pm$ 0.03\\ 
352 & 1.281 $\pm$ 0.021 & 5.44 $\pm$ 0.02 & 6.2 $\pm$ 0.01 & 6.27 $\pm$ 0.01\\








 
 


\hline

\end{tabular}
\begin{tablenotes}

$^a$ In units of 10$^{4}$K.\\
    
\end{tablenotes}
\end{table*}
\newpage

==> Tables/Tabla_resultados_ICF.tex <==
\begin{table*}
\centering
\caption{Ionisation correction factors and total S/H abundance for the objects in the general sample. Only objects with ICF > 1.1 are listed (see text for dateils).}
\label{ICF}
\begin{tabular}{cccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline



4 & - & - & - & -& 1.17 $\pm$ 0.01 & 6.46 $\pm$ 0.07\\ 
8 & - & - & - & -& 1.82 $\pm$ 0.08 & 6.26 $\pm$ 0.05\\ 
9 & - & - & - & -& 1.38 $\pm$ 0.16 & 6.18 $\pm$ 0.15\\ 
10 & - & - & - & -& 1.48 $\pm$ 0.04 & 6.12 $\pm$ 0.04\\
11 & - & - & - & -& 1.64 $\pm$ 0.22 & 6.12 $\pm$ 0.14\\
12 & - & - & - & -& 1.71 $\pm$ 0.34 & 6.21 $\pm$ 0.21\\
13 & - & - & - & -& 1.16 $\pm$ 0.07 & 6.05 $\pm$ 0.08\\
15 & - & - & - & -& 1.3 $\pm$ 0.03 & 6.51 $\pm$ 0.04\\
16 & - & - & - & -& 1.22 $\pm$ 0.07 & 6.53 $\pm$ 0.06\\
36 & - & - & - & -& 1.11 $\pm$ 0.03 & 6.7 $\pm$ 0.04\\
42 & - & - & - & -& 1.29 $\pm$ 0.07 & 6.45 $\pm$ 0.09\\
43 & - & - & - & -& 1.39 $\pm$ 0.1 & 6.5 $\pm$ 0.06\\
44 & - & - & - & -& 1.94 $\pm$ 0.18 & 7.06 $\pm$ 0.07\\
45 & - & - & - & -& 1.2 $\pm$ 0.05 & 6.72 $\pm$ 0.05\\
46 & 6.06 $\pm$ 0.01 & 4.53 $\pm$ 0.01 & 2.03 $\pm$ 0.21 & 1.01 $\pm$ 0.01 & 1.09 $\pm$ 0.01 & 6.69 $\pm$ 0.01\\
53 & 6.22 $\pm$ 0.06 & 4.89 $\pm$ 0.01 & 1.08 $\pm$ 0.06 & 1.08 $\pm$ 0.02 & 1.03 $\pm$ 0.01 & 6.76 $\pm$ 0.08\\
54 & 6.33 $\pm$ 0.05 & 4.49 $\pm$ 0.01 & 1.52 $\pm$ 0.05 & 1.03 $\pm$ 0.02 & 1.04 $\pm$ 0.01 & 6.91 $\pm$ 0.06\\
55 & - & - & - & -& 1.11 $\pm$ 0.05 & 6.55 $\pm$ 0.11\\
75 & 6.36 $\pm$ 0.05 & 4.98 $\pm$ 0.02 & 1.13 $\pm$ 0.06 & 1.07 $\pm$ 0.01 & 1.05 $\pm$ 0.01 & 6.92 $\pm$ 0.05\\
79 & 6.1 $\pm$ 0.02 & 3.98 $\pm$ 0.02 & 1.75 $\pm$ 0.03 & 1.02 $\pm$ 0.02 & 1.01 $\pm$ 0.0 & 6.79 $\pm$ 0.03\\
81 & - & - & - & -& 1.13 $\pm$ 0.04 & 6.46 $\pm$ 0.06\\
99 & - & - & - & -& 1.11 $\pm$ 0.03 & 7.03 $\pm$ 0.04\\
103 & - & - & - & -& 1.11 $\pm$ 0.03 & 6.62 $\pm$ 0.04\\
192 & - & - & - & -& 1.13 $\pm$ 0.02 & 6.53 $\pm$ 0.04\\
196 & - & - & - & -& 1.11 $\pm$ 0.01 & 6.98 $\pm$ 0.05\\
206 & - & - & - & -& 1.16 $\pm$ 0.03 & 6.48 $\pm$ 0.05\\
207 & - & - & - & -& 1.12 $\pm$ 0.02 & 6.34 $\pm$ 0.05\\
208 & - & - & - & -& 1.2 $\pm$ 0.03 & 6.46 $\pm$ 0.04\\
209 & - & - & - & -& 1.24 $\pm$ 0.03 & 6.35 $\pm$ 0.03\\
210 & - & - & - & -& 1.19 $\pm$ 0.03 & 6.35 $\pm$ 0.04\\
211 & - & - & - & -& 1.12 $\pm$ 0.02 & 6.2 $\pm$ 0.02\\
213 & - & - & - & -& 1.22 $\pm$ 0.05 & 6.19 $\pm$ 0.08\\
214 & - & - & - & -& 1.26 $\pm$ 0.04 & 6.23 $\pm$ 0.05\\
217 & - & - & - & -& 1.2 $\pm$ 0.05 & 6.65 $\pm$ 0.05\\
218 & - & - & - & -& 1.23 $\pm$ 0.11 & 6.72 $\pm$ 0.13\\
219 & - & - & - & -& 1.12 $\pm$ 0.03 & 6.28 $\pm$ 0.05\\
220 & - & - & - & -& 1.11 $\pm$ 0.02 & 6.22 $\pm$ 0.03\\
226 & - & - & - & -& 1.17 $\pm$ 0.06 & 6.38 $\pm$ 0.09\\
233 & - & - & - & -& 1.67 $\pm$ 0.2 & 6.5 $\pm$ 0.1\\
238 & - & - & - & -& 1.13 $\pm$ 0.04 & 6.17 $\pm$ 0.05\\
239 & - & - & - & -& 1.24 $\pm$ 0.15 & 6.18 $\pm$ 0.15\\
257 & - & - & - & -& 1.53 $\pm$ 0.08 & 5.43 $\pm$ 0.05\\ 
258 & - & - & - & -& 1.38 $\pm$ 0.06 & 5.7 $\pm$ 0.04\\ 
259 & - & - & - & -& 1.26 $\pm$ 0.08 & 5.95 $\pm$ 0.09\\ 
260 & - & - & - & -& 1.26 $\pm$ 0.03 & 6.37 $\pm$ 0.05\\ 
261 & - & - & - & -& 1.3 $\pm$ 0.06 & 6.09 $\pm$ 0.07\\ 
262 & - & - & - & -& 1.34 $\pm$ 0.06 & 6.27 $\pm$ 0.07\\ 
263 & - & - & - & -& 2.03 $\pm$ 0.18 & 6.37 $\pm$ 0.08\\ 
264 & - & - & - & -& 1.37 $\pm$ 0.07 & 6.12 $\pm$ 0.08\\ 
265 & - & - & - & -& 1.51 $\pm$ 0.06 & 6.02 $\pm$ 0.06\\ 
266 & - & - & - & -& 1.35 $\pm$ 0.06 & 6.16 $\pm$ 0.07\\ 
267 & - & - & - & -& 1.14 $\pm$ 0.02 & 6.18 $\pm$ 0.06\\ 
268 & - & - & - & -& 1.76 $\pm$ 0.09 & 6.02 $\pm$ 0.05\\ 
269 & - & - & - & -& 1.34 $\pm$ 0.05 & 6.19 $\pm$ 0.07\\ 
270 & - & - & - & -& 1.39 $\pm$ 0.06 & 6.12 $\pm$ 0.06\\ 
271 & 5.54 $\pm$ 0.03 & 4.96 $\pm$ 0.08 & 0.48 $\pm$ 0.09 & 1.27 $\pm$ 0.1 & 1.38 $\pm$ 0.04 & 6.25 $\pm$ 0.06\\ 
272 & 5.49 $\pm$ 0.04 & 4.94 $\pm$ 0.08 & 0.46 $\pm$ 0.1 & 1.26 $\pm$ 0.14 & 1.35 $\pm$ 0.04 & 6.22 $\pm$ 0.07\\ 
273 & 5.65 $\pm$ 0.03 & 4.92 $\pm$ 0.08 & 0.61 $\pm$ 0.1 & 1.2 $\pm$ 0.1 & 1.24 $\pm$ 0.03 & 6.41 $\pm$ 0.07\\ 
274 & 5.95 $\pm$ 0.05 & 5.17 $\pm$ 0.04 & 0.65 $\pm$ 0.08 & 1.2 $\pm$ 0.07 & 1.2 $\pm$ 0.05 & 6.66 $\pm$ 0.07\\ 
275 & 5.92 $\pm$ 0.04 & 5.51 $\pm$ 0.04 & 0.33 $\pm$ 0.07 & 1.41 $\pm$ 0.1 & 1.2 $\pm$ 0.04 & 6.68 $\pm$ 0.07\\ 
276 & 5.89 $\pm$ 0.05 & 4.74 $\pm$ 0.1 & 0.97 $\pm$ 0.13 & 1.09 $\pm$ 0.08 & 1.15 $\pm$ 0.04 & 6.57 $\pm$ 0.07\\ 



  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 
 
277 & 5.8 $\pm$ 0.08 & - & - & -& 1.15 $\pm$ 0.04 & 6.61 $\pm$ 0.07\\ 
278 & - & - & - & -& 1.27 $\pm$ 0.03 & 6.73 $\pm$ 0.04\\ 
279 & - & - & - & -& 1.33 $\pm$ 0.04 & 6.33 $\pm$ 0.04\\ 
280 & - & - & - & -& 1.23 $\pm$ 0.03 & 6.47 $\pm$ 0.04\\ 
281 & 5.49 $\pm$ 0.04 & 4.13 $\pm$ 0.37 & 0.28 $\pm$ 0.08 & 1.44 $\pm$ 0.13 & 1.45 $\pm$ 0.05 & 6.29 $\pm$ 0.06\\ 
282 & - & - & - & -& 1.15 $\pm$ 0.02 & 6.74 $\pm$ 0.03\\
283 & 5.57 $\pm$ 0.04 & 5.04 $\pm$ 0.12 & 0.43 $\pm$ 0.13 & 1.33 $\pm$ 0.13 & 1.33 $\pm$ 0.04 & 6.36 $\pm$ 0.06\\ 
284 & 5.75 $\pm$ 0.04 & 4.84 $\pm$ 0.1 & 0.77 $\pm$ 0.12 & 1.15 $\pm$ 0.07 & 1.17 $\pm$ 0.02 & 6.51 $\pm$ 0.05\\ 
285 & 4.96 $\pm$ 0.02 & 4.66 $\pm$ 0.02 & 0.24 $\pm$ 0.03 & 1.53 $\pm$ 0.05 & 1.52 $\pm$ 0.06 & 5.85 $\pm$ 0.04\\ 
286 & 4.54 $\pm$ 0.04 & 4.76 $\pm$ 0.02 & -0.21 $\pm$ 0.05 & 2.44 $\pm$ 0.23 & 1.96 $\pm$ 0.14 & 5.56 $\pm$ 0.08\\ 
287 & - & - & - & -& 2.39 $\pm$ 0.16 & 5.41 $\pm$ 0.04\\
288 & 5.57 $\pm$ 0.03 & 5.04 $\pm$ 0.06 & 0.43 $\pm$ 0.08 & 1.32 $\pm$ 0.08 & 1.3 $\pm$ 0.05 & 6.3 $\pm$ 0.05\\ 
289 & - & - & - & -& 1.67 $\pm$ 0.22 & 5.97 $\pm$ 0.09\\ 
290 & - & - & - & -& 1.13 $\pm$ 0.02 & 6.6 $\pm$ 0.03\\ 
291 & - & - & - & -& 1.45 $\pm$ 0.04 & 5.85 $\pm$ 0.03\\ 
294 & 6.1 $\pm$ 0.01 & 5.06 $\pm$ 0.02 & 0.87 $\pm$ 0.03 & 1.12 $\pm$ 0.02 & 1.22 $\pm$ 0.02 & 6.83 $\pm$ 0.02\\ 
296 & 5.36 $\pm$ 0.01 & 5.16 $\pm$ 0.01 & 0.15 $\pm$ 0.02 & 1.62 $\pm$ 0.04 & 1.53 $\pm$ 0.04 & 6.27 $\pm$ 0.02\\ 
297 & 4.59 $\pm$ 0.02 & 5.02 $\pm$ 0.02 & -0.4 $\pm$ 0.03 & 3.15 $\pm$ 0.19 & 2.51 $\pm$ 0.17 & 5.58 $\pm$ 0.05\\ 
298 & 5.56 $\pm$ 0.01 & 5.12 $\pm$ 0.01 & 0.36 $\pm$ 0.02 & 1.39 $\pm$ 0.03 & 1.35 $\pm$ 0.03 & 6.33 $\pm$ 0.02\\ 
299 & 5.86 $\pm$ 0.01 & 5.38 $\pm$ 0.01 & 0.39 $\pm$ 0.02 & 1.37 $\pm$ 0.02 & 1.24 $\pm$ 0.02 & 6.55 $\pm$ 0.02\\ 
300 & 5.87 $\pm$ 0.01 & 4.78 $\pm$ 0.02 & 0.92 $\pm$ 0.03 & 1.1 $\pm$ 0.02 & 1.19 $\pm$ 0.01 & 6.53 $\pm$ 0.02\\ 
301 & 5.87 $\pm$ 0.01 & - & - & -& 1.12 $\pm$ 0.01 & 6.53 $\pm$ 0.02\\ 
302 & 5.83 $\pm$ 0.01 & 5.25 $\pm$ 0.02 & 0.48 $\pm$ 0.02 & 1.3 $\pm$ 0.02 & 1.21 $\pm$ 0.02 & 6.51 $\pm$ 0.02\\ 
303 & 5.98 $\pm$ 0.01 & 4.82 $\pm$ 0.02 & 0.98 $\pm$ 0.03 & 1.09 $\pm$ 0.01 & 1.13 $\pm$ 0.01 & 6.69 $\pm$ 0.02\\ 
305 & - & - & - & -& 1.55 $\pm$ 0.04 & 6.03 $\pm$ 0.02\\ 
306 & - & - & - & -& 1.38 $\pm$ 0.02 & 6.21 $\pm$ 0.02\\ 
307 & 5.56 $\pm$ 0.01 & 4.95 $\pm$ 0.02 & 0.51 $\pm$ 0.03 & 1.25 $\pm$ 0.03 & 1.19 $\pm$ 0.01 & 6.33 $\pm$ 0.02\\ 
308 & 5.44 $\pm$ 0.01 & 4.7 $\pm$ 0.02 & 0.61 $\pm$ 0.03 & 1.2 $\pm$ 0.03 & 1.33 $\pm$ 0.02 & 6.3 $\pm$ 0.02\\ 
309 & 5.47 $\pm$ 0.01 & 4.91 $\pm$ 0.02 & 0.46 $\pm$ 0.03 & 1.29 $\pm$ 0.03 & 1.36 $\pm$ 0.03 & 6.28 $\pm$ 0.02\\ 
310 & 5.85 $\pm$ 0.01 & 4.68 $\pm$ 0.02 & 0.99 $\pm$ 0.03 & 1.1 $\pm$ 0.01 & 1.14 $\pm$ 0.01 & 6.57 $\pm$ 0.01\\ 
311 & 5.22 $\pm$ 0.05 & 4.96 $\pm$ 0.05 & 0.19 $\pm$ 0.09 & 1.57 $\pm$ 0.16 & 1.52 $\pm$ 0.09 & 6.13 $\pm$ 0.08\\ 
312 & - & - & - & -& 1.5 $\pm$ 0.05 & 6.5 $\pm$ 0.03\\
313 & 5.31 $\pm$ 0.05 & 5.3 $\pm$ 0.05 & -0.01 $\pm$ 0.08 & 1.94 $\pm$ 0.22 & 1.73 $\pm$ 0.12 & 6.15 $\pm$ 0.08\\ 
314 & - & - & - & -& 1.27 $\pm$ 0.03 & 6.46 $\pm$ 0.05\\
315 & 5.59 $\pm$ 0.02 & 5.18 $\pm$ 0.07 & 0.33 $\pm$ 0.08 & 1.42 $\pm$ 0.09 & 1.58 $\pm$ 0.08 & 6.22 $\pm$ 0.04\\ 
316 & 5.92 $\pm$ 0.01 & 4.77 $\pm$ 0.05 & 0.96 $\pm$ 0.05 & 1.09 $\pm$ 0.03 & 1.1 $\pm$ 0.01 & 6.74 $\pm$ 0.02\\ 
318 & 5.62 $\pm$ 0.02 & 4.96 $\pm$ 0.05 & 0.54 $\pm$ 0.06 & 1.25 $\pm$ 0.06 & 1.24 $\pm$ 0.02 & 6.5 $\pm$ 0.03\\ 
319 & - & - & - & -& 1.58 $\pm$ 0.09 & 6.22 $\pm$ 0.07\\
320 & 5.31 $\pm$ 0.03 & 4.92 $\pm$ 0.06 & 0.31 $\pm$ 0.08 & 1.39 $\pm$ 0.12 & 1.7 $\pm$ 0.07 & 6.0 $\pm$ 0.06\\ 
321 & 5.21 $\pm$ 0.02 & 4.98 $\pm$ 0.08 & 0.17 $\pm$ 0.09 & 1.54 $\pm$ 0.17 & 1.67 $\pm$ 0.07 & 6.02 $\pm$ 0.06\\ 
322 & - & - & - & -& 1.16 $\pm$ 0.02 & 6.3 $\pm$ 0.04\\ 
323 & - & - & - & -& 1.12 $\pm$ 0.01 & 6.31 $\pm$ 0.04\\ 
324 & - & - & - & -& 1.38 $\pm$ 0.04 & 6.05 $\pm$ 0.03\\ 
325 & 5.34 $\pm$ 0.05 & 5.14 $\pm$ 0.06 & 0.15 $\pm$ 0.09 & 1.63 $\pm$ 0.18 & 1.62 $\pm$ 0.08 & 6.25 $\pm$ 0.08\\ 
326 & - & - & - & -& 1.55 $\pm$ 0.07 & 5.81 $\pm$ 0.06\\
327 & 5.51 $\pm$ 0.03 & 5.05 $\pm$ 0.03 & 0.37 $\pm$ 0.06 & 1.38 $\pm$ 0.08 & 1.37 $\pm$ 0.08 & 6.23 $\pm$ 0.06\\ 
328 & 5.57 $\pm$ 0.05 & 5.01 $\pm$ 0.04 & 0.46 $\pm$ 0.08 & 1.29 $\pm$ 0.11 & 1.36 $\pm$ 0.09 & 6.34 $\pm$ 0.07\\ 
329 & 5.79 $\pm$ 0.05 & 4.94 $\pm$ 0.05 & 0.71 $\pm$ 0.09 & 1.16 $\pm$ 0.1 & 1.26 $\pm$ 0.08 & 6.5 $\pm$ 0.08\\ 
330 & 5.5 $\pm$ 0.05 & 5.05 $\pm$ 0.05 & 0.36 $\pm$ 0.08 & 1.33 $\pm$ 0.15 & 1.64 $\pm$ 0.17 & 6.18 $\pm$ 0.08\\ 
331 & 5.38 $\pm$ 0.04 & 5.17 $\pm$ 0.04 & 0.15 $\pm$ 0.07 & 1.61 $\pm$ 0.15 & 1.5 $\pm$ 0.12 & 6.21 $\pm$ 0.08\\ 
332 & 5.6 $\pm$ 0.05 & 5.12 $\pm$ 0.05 & 0.39 $\pm$ 0.08 & 1.36 $\pm$ 0.11 & 1.47 $\pm$ 0.12 & 6.35 $\pm$ 0.07\\ 
333 & 5.79 $\pm$ 0.06 & 6.0 $\pm$ 0.02 & -0.21 $\pm$ 0.07 & 2.25 $\pm$ 0.36 & 1.31 $\pm$ 0.07 & 6.88 $\pm$ 0.11\\ 
334 & 6.07 $\pm$ 0.04 & - & - & -& 1.04 $\pm$ 0.01 & 6.99 $\pm$ 0.02\\ 
335 & 5.65 $\pm$ 0.05 & 4.73 $\pm$ 0.04 & 0.77 $\pm$ 0.08 & 1.03 $\pm$ 0.04 & 1.22 $\pm$ 0.06 & 6.13 $\pm$ 0.06\\ 
336 & - & - & - & -& 1.18 $\pm$ 0.04 & 6.5 $\pm$ 0.05\\ 
339 & - & - & - & -& 1.22 $\pm$ 0.05 & 6.65 $\pm$ 0.06\\ 
341 & - & - & - & -& 1.19 $\pm$ 0.04 & 6.34 $\pm$ 0.05\\ 
342 & 5.4 $\pm$ 0.04 & 4.75 $\pm$ 0.1 & 0.53 $\pm$ 0.12 & 1.21 $\pm$ 0.16 & 1.4 $\pm$ 0.08 & 6.25 $\pm$ 0.09\\ 
345 & 4.66 $\pm$ 0.03 & 5.23 $\pm$ 0.03 & -0.51 $\pm$ 0.05 & 3.88 $\pm$ 0.42 & 4.05 $\pm$ 0.55 & 5.79 $\pm$ 0.07\\ 
346 & 4.85 $\pm$ 0.03 & 5.12 $\pm$ 0.03 & -0.26 $\pm$ 0.05 & 2.6 $\pm$ 0.22 & 2.9 $\pm$ 0.3 & 5.8 $\pm$ 0.06\\ 
347 & 4.36 $\pm$ 0.03 & 4.84 $\pm$ 0.03 & -0.43 $\pm$ 0.06 & 3.32 $\pm$ 0.37 & 3.23 $\pm$ 0.38 & 5.54 $\pm$ 0.07\\ 


  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 




348 & 4.31 $\pm$ 0.06 & 4.4 $\pm$ 0.08 & -0.11 $\pm$ 0.12 & 2.09 $\pm$ 0.4 & 1.78 $\pm$ 0.15 & 5.32 $\pm$ 0.13\\ 
349 & 6.0 $\pm$ 0.07 & 5.12 $\pm$ 0.18 & 0.74 $\pm$ 0.22 & 1.15 $\pm$ 0.17 & 1.23 $\pm$ 0.04 & 6.89 $\pm$ 0.1\\ 
350 & 5.69 $\pm$ 0.03 & 5.04 $\pm$ 0.11 & 0.54 $\pm$ 0.12 & 1.23 $\pm$ 0.11 & 1.31 $\pm$ 0.05 & 6.52 $\pm$ 0.05\\ 
351 & - & - & - & -& 1.24 $\pm$ 0.01 & 6.6 $\pm$ 0.03\\ 
352 & 5.65 $\pm$ 0.01 & 5.06 $\pm$ 0.04 & 0.49 $\pm$ 0.05 & 1.28 $\pm$ 0.05 & 1.58 $\pm$ 0.04 & 6.38 $\pm$ 0.02\\






 

 

 









 
 

 
 
 



\hline
\end{tabular}

\end{table*}
\newpage

==> Tables/Tabla_resultados_ICF_IR.tex <==
\begin{table*}
\centering
\caption{IR derived ionisation correction factors (ICF).}
\label{ICF-IR}
\begin{tabular}{cccccccc}
\hline
ID & [SIV]10.54$\mu$m & [SIII]18.71$\mu$m & log(S$^{++}$/S$^{3+}$) & ICF$_{IR}$ 
\\ \hline

32$^a$ & 28.39 $\pm$ 0.81 & 60.56 $\pm$ 3.94 & 1.05 $\pm$ 1.05 & 1.077 $\pm$ 0.038\\ 
35$^a$ & 2.75 $\pm$ 1.21 & 7.46 $\pm$ 1.49 & 1.17 $\pm$ 1.17 & 1.059 $\pm$ 0.049\\ 
38$^a$ & 3.33 $\pm$ 0.1 & 5.41 $\pm$ 0.64 & 0.91 $\pm$ 0.91 & 1.097 $\pm$ 0.087\\ 
40$^a$ & 3.08 $\pm$ 0.09 & 7.93 $\pm$ 1.68 & 1.17 $\pm$ 1.17 & 1.054 $\pm$ 0.076\\ 
45$^a$ & 12.92 $\pm$ 0.73 & 8.47 $\pm$ 1.38 & 0.56 $\pm$ 0.56 & 1.239 $\pm$ 0.078\\ 
173$^a$ & 0.18 $\pm$ 0.05 & 4.01 $\pm$ 0.18 & 2.0 $\pm$ 2.0 & 1.006 $\pm$ 0.137\\ 
257$^b$  & 0.48 $\pm$ 0.03 & 0.23 $\pm$ 0.02 & 0.3 $\pm$ 0.3 & 1.435 $\pm$ 0.095\\ 
257$^c$  & 0.431 $\pm$ 0.0429 & 0.525 $\pm$ 0.0851 & 0.7 $\pm$ 0.7 & 1.171 $\pm$ 0.063\\ 
268$^b$  & 4.58 $\pm$ 0.04 & 0.812 $\pm$ 0.03 & -0.13 $\pm$ -0.13 & 2.179 $\pm$ 0.125\\ 
269$^c$ & 6.38 $\pm$ 0.338 & 51.1 $\pm$ 0.286 & 1.54 $\pm$ 1.54 & 1.022 $\pm$ 0.09\\ 
285$^c$ & 1.71 $\pm$ 0.0952 & 0.466 $\pm$ 0.167 & 0.18 $\pm$ 0.18 & 1.599 $\pm$ 0.22\\ 
286$^b$  & 1.56 $\pm$ 0.03 & 0.43 $\pm$ 0.03 & 0.19 $\pm$ 0.19 & 1.592 $\pm$ 0.07\\ 
292$^c$ & 36.6 $\pm$ 1.84 & 363.0 $\pm$ 18.2 & 1.79 $\pm$ 1.79 & 1.013 $\pm$ 0.014\\ 
294$^c$ & 5.53 $\pm$ 2.78 & 54.5 $\pm$ 2.76 & 1.66 $\pm$ 1.66 & 1.018 $\pm$ 0.07\\ 
296$^c$ & 19.3 $\pm$ 0.967 & 5.18 $\pm$ 0.278 & 0.05 $\pm$ 0.05 & 1.761 $\pm$ 0.143\\ 
314$^c$ & 11.3 $\pm$ 0.591 & 8.83 $\pm$ 0.491 & 0.56 $\pm$ 0.56 & 1.188 $\pm$ 0.167\\ 
315$^b$  & 185.72 $\pm$ 1.73 & 45.8 $\pm$ 0.21 & 0.08 $\pm$ 0.08 & 1.752 $\pm$ 0.042\\ 
315$^c$ & 159.0 $\pm$ 7.96 & 61.3 $\pm$ 3.08 & 0.27 $\pm$ 0.27 & 1.481 $\pm$ 0.053\\ 
315$^d$ & 14.06565 $\pm$ 0.3036 & 3.88125 $\pm$ 0.1518 & 0.12 $\pm$ 0.12 & 1.672 $\pm$ 0.053\\ 
316$^b$  & 43.95 $\pm$ 0.14 & 45.24 $\pm$ 0.25 & 0.72 $\pm$ 0.72 & 1.156 $\pm$ 0.018\\ 
317$^c$ & 58.2 $\pm$ 2.92 & 59.4 $\pm$ 3.03 & 0.76 $\pm$ 0.76 & 1.133 $\pm$ 0.107\\ 


\hline
\end{tabular}
\vspace{0.3cm}

\begin{tablenotes}

{\it Notes:}
$^a$ \cite{2008ApJ...682..336G};
$^b$ \cite{2008ApJ...673..193W};
$^c$ \cite{2008ApJ...678..804E};
$^d$ \cite{2011ApJ...734...82I}.
\end{tablenotes}
\end{table*}
\newpage

==> Tables/Tabla_resultados_ICF_all.tex <==
\begin{table*}
\centering
\caption{Ionisation correction factors (ICF) for all the objects in the general sample.}
\label{ICF-all}
\begin{tabular}{cccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline



1 & - & - & - & -& 1.04 $\pm$ 0.01 & 7.2 $\pm$ 0.08\\ 
2 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.2 $\pm$ 0.07\\ 
3 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.06 $\pm$ 0.04\\ 
4 & - & - & - & -& 1.17 $\pm$ 0.01 & 6.46 $\pm$ 0.07\\ 
5 & - & - & - & -& 1.08 $\pm$ 0.01 & 6.8 $\pm$ 0.04\\ 
6 & - & - & - & -& 1.08 $\pm$ 0.01 & 6.77 $\pm$ 0.11\\ 
7 & - & - & - & -& 1.07 $\pm$ 0.01 & 6.83 $\pm$ 0.1\\ 
8 & - & - & - & -& 1.82 $\pm$ 0.08 & 6.26 $\pm$ 0.05\\ 
9 & - & - & - & -& 1.38 $\pm$ 0.16 & 6.18 $\pm$ 0.15\\ 
10 & - & - & - & -& 1.48 $\pm$ 0.04 & 6.12 $\pm$ 0.04\\
11 & - & - & - & -& 1.64 $\pm$ 0.22 & 6.12 $\pm$ 0.14\\
12 & - & - & - & -& 1.71 $\pm$ 0.34 & 6.21 $\pm$ 0.21\\
13 & - & - & - & -& 1.16 $\pm$ 0.07 & 6.05 $\pm$ 0.08\\
14 & - & - & - & -& 1.08 $\pm$ 0.0 & 7.06 $\pm$ 0.03\\
15 & - & - & - & -& 1.3 $\pm$ 0.03 & 6.51 $\pm$ 0.04\\
16 & - & - & - & -& 1.22 $\pm$ 0.07 & 6.53 $\pm$ 0.06\\
17 & - & - & - & -& 1.05 $\pm$ 0.03 & 6.86 $\pm$ 0.08\\
18 & - & - & - & -& 1.03 $\pm$ 0.01 & 7.26 $\pm$ 0.05\\
19 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.02 $\pm$ 0.04\\
20 & - & - & - & -& 1.04 $\pm$ 0.02 & 6.76 $\pm$ 0.04\\
21 & - & - & - & -& 1.05 $\pm$ 0.03 & 6.87 $\pm$ 0.09\\
22 & - & - & - & -& 1.04 $\pm$ 0.02 & 6.77 $\pm$ 0.04\\
23 & - & - & - & -& 1.1 $\pm$ 0.04 & 6.78 $\pm$ 0.08\\
24 & - & - & - & -& 1.09 $\pm$ 0.05 & 6.72 $\pm$ 0.12\\
25 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.04 $\pm$ 0.03\\
26 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.94 $\pm$ 0.04\\
27 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.09 $\pm$ 0.03\\
28 & - & - & - & -& 1.04 $\pm$ 0.01 & 7.14 $\pm$ 0.03\\
29 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.36 $\pm$ 0.07\\
30 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.5 $\pm$ 0.03\\
31 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.28 $\pm$ 0.03\\
32 & - & - & - & -& 1.05 $\pm$ 0.01 & 7.09 $\pm$ 0.03\\
33 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.83 $\pm$ 0.05\\
34 & - & - & - & -& 1.03 $\pm$ 0.01 & 7.25 $\pm$ 0.04\\
35 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.96 $\pm$ 0.04\\
36 & - & - & - & -& 1.11 $\pm$ 0.03 & 6.7 $\pm$ 0.04\\
37 & - & - & - & -& 1.09 $\pm$ 0.02 & 6.96 $\pm$ 0.04\\
38 & - & - & - & -& 1.09 $\pm$ 0.02 & 6.89 $\pm$ 0.05\\
39 & - & - & - & -& 1.09 $\pm$ 0.02 & 6.89 $\pm$ 0.04\\
40 & - & - & - & -& 1.09 $\pm$ 0.02 & 7.15 $\pm$ 0.05\\
41 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.75 $\pm$ 0.04\\
42 & - & - & - & -& 1.29 $\pm$ 0.07 & 6.45 $\pm$ 0.09\\
43 & - & - & - & -& 1.39 $\pm$ 0.1 & 6.5 $\pm$ 0.06\\
44 & - & - & - & -& 1.94 $\pm$ 0.18 & 7.06 $\pm$ 0.07\\
45 & - & - & - & -& 1.2 $\pm$ 0.05 & 6.72 $\pm$ 0.05\\
46 & 6.06 $\pm$ 0.01 & 4.53 $\pm$ 0.01 & 2.03 $\pm$ 0.21 & 1.01 $\pm$ 0.01 & 1.09 $\pm$ 0.01 & 6.69 $\pm$ 0.01\\
47 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.11 $\pm$ 0.05\\
48 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.12 $\pm$ 0.07\\
49 & - & - & - & -& 1.06 $\pm$ 0.02 & 7.05 $\pm$ 0.07\\
50 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.21 $\pm$ 0.06\\
51 & - & - & - & -& 1.02 $\pm$ 0.01 & 6.98 $\pm$ 0.07\\
52 & - & - & - & -& 1.01 $\pm$ 0.01 & 7.2 $\pm$ 0.06\\
53 & 6.22 $\pm$ 0.06 & 4.89 $\pm$ 0.01 & 1.08 $\pm$ 0.06 & 1.08 $\pm$ 0.02 & 1.03 $\pm$ 0.01 & 6.76 $\pm$ 0.08\\
54 & 6.33 $\pm$ 0.05 & 4.49 $\pm$ 0.01 & 1.52 $\pm$ 0.05 & 1.03 $\pm$ 0.02 & 1.04 $\pm$ 0.01 & 6.91 $\pm$ 0.06\\
55 & - & - & - & -& 1.11 $\pm$ 0.05 & 6.55 $\pm$ 0.11\\
56 & - & - & - & -& 1.04 $\pm$ 0.02 & 7.13 $\pm$ 0.07\\
57 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.1 $\pm$ 0.08\\
58 & - & - & - & -& 1.04 $\pm$ 0.02 & 6.93 $\pm$ 0.08\\
59 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.12 $\pm$ 0.07\\
60 & - & - & - & -& 1.04 $\pm$ 0.02 & 6.96 $\pm$ 0.08\\

  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 
 
 
61 & - & - & - & -& 1.03 $\pm$ 0.01 & 7.01 $\pm$ 0.09\\
62 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.16 $\pm$ 0.08\\
63 & - & - & - & -& 1.03 $\pm$ 0.02 & 6.84 $\pm$ 0.1\\
64 & - & - & - & -& 1.04 $\pm$ 0.02 & 7.03 $\pm$ 0.08\\
65 & - & - & - & -& 1.04 $\pm$ 0.02 & 7.21 $\pm$ 0.07\\
66 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.06 $\pm$ 0.08\\
67 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.09 $\pm$ 0.08\\
68 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.4 $\pm$ 0.07\\
69 & - & - & - & -& 1.04 $\pm$ 0.02 & 7.09 $\pm$ 0.08\\
70 & - & - & - & -& 1.01 $\pm$ 0.01 & 7.16 $\pm$ 0.08\\
71 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.82 $\pm$ 0.09\\
72 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.56 $\pm$ 0.07\\
73 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.82 $\pm$ 0.02\\
74 & - & - & - & -& 1.02 $\pm$ 0.01 & 6.93 $\pm$ 0.03\\
75 & 6.36 $\pm$ 0.05 & 4.98 $\pm$ 0.02 & 1.13 $\pm$ 0.06 & 1.07 $\pm$ 0.01 & 1.05 $\pm$ 0.01 & 6.92 $\pm$ 0.05\\
76 & - & - & - & -& 1.01 $\pm$ 0.0 & 6.91 $\pm$ 0.03\\
77 & - & - & - & -& 1.02 $\pm$ 0.01 & 6.85 $\pm$ 0.07\\
78 & - & - & - & -& 1.02 $\pm$ 0.01 & 6.97 $\pm$ 0.08\\
79 & 6.1 $\pm$ 0.02 & 3.98 $\pm$ 0.02 & 1.75 $\pm$ 0.03 & 1.02 $\pm$ 0.02 & 1.01 $\pm$ 0.0 & 6.79 $\pm$ 0.03\\
80 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.98 $\pm$ 0.04\\
81 & - & - & - & -& 1.13 $\pm$ 0.04 & 6.46 $\pm$ 0.06\\
82 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.55 $\pm$ 0.04\\
83 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.9 $\pm$ 0.04\\
84 & - & - & - & -& 1.09 $\pm$ 0.03 & 6.67 $\pm$ 0.05\\
85 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.69 $\pm$ 0.04\\
86 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.96 $\pm$ 0.04\\
87 & - & - & - & -& 1.03 $\pm$ 0.01 & 6.88 $\pm$ 0.04\\
88 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.79 $\pm$ 0.04\\
89 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.03 $\pm$ 0.03\\
90 & - & - & - & -& 1.03 $\pm$ 0.01 & 6.79 $\pm$ 0.04\\
91 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.93 $\pm$ 0.04\\
92 & - & - & - & -& 1.03 $\pm$ 0.01 & 7.0 $\pm$ 0.03\\
93 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.96 $\pm$ 0.04\\
94 & - & - & - & -& 1.02 $\pm$ 0.01 & 6.85 $\pm$ 0.04\\
95 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.92 $\pm$ 0.04\\
96 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.88 $\pm$ 0.04\\
97 & - & - & - & -& 1.02 $\pm$ 0.0 & 6.93 $\pm$ 0.03\\
98 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.03 $\pm$ 0.04\\
99 & - & - & - & -& 1.11 $\pm$ 0.03 & 7.03 $\pm$ 0.04\\
100 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.88 $\pm$ 0.04\\
101 & - & - & - & -& 1.03 $\pm$ 0.01 & 6.91 $\pm$ 0.04\\
102 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.85 $\pm$ 0.04\\
103 & - & - & - & -& 1.11 $\pm$ 0.03 & 6.62 $\pm$ 0.04\\
104 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.64 $\pm$ 0.05\\
105 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.05 $\pm$ 0.05\\
106 & - & - & - & -& 1.04 $\pm$ 0.02 & 6.85 $\pm$ 0.06\\
107 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.68 $\pm$ 0.05\\
108 & - & - & - & -& 1.05 $\pm$ 0.02 & 6.7 $\pm$ 0.05\\
109 & - & - & - & -& 1.1 $\pm$ 0.04 & 6.63 $\pm$ 0.06\\
110 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.36 $\pm$ 0.02\\
111 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.22 $\pm$ 0.04\\
112 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.32 $\pm$ 0.04\\
113 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.28 $\pm$ 0.03\\
114 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.47 $\pm$ 0.05\\
115 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.41 $\pm$ 0.04\\
116 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.53 $\pm$ 0.04\\
117 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.29 $\pm$ 0.03\\
118 & - & - & - & -& 1.04 $\pm$ 0.0 & 7.35 $\pm$ 0.03\\
119 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.33 $\pm$ 0.02\\
120 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.31 $\pm$ 0.03\\
121 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.26 $\pm$ 0.03\\

  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 
 
 
122 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.34 $\pm$ 0.02\\
123 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.28 $\pm$ 0.03\\
124 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.18 $\pm$ 0.05\\
126 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.05 $\pm$ 0.03\\
127 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.3 $\pm$ 0.04\\
128 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.21 $\pm$ 0.04\\
129 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.22 $\pm$ 0.03\\
130 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.32 $\pm$ 0.03\\
131 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.28 $\pm$ 0.03\\
125 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.24 $\pm$ 0.02\\
132 & - & - & - & -& 1.02 $\pm$ 0.0 & 6.94 $\pm$ 0.02\\
133 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.22 $\pm$ 0.02\\
134 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.35 $\pm$ 0.02\\
135 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.94 $\pm$ 0.02\\
136 & - & - & - & -& 1.05 $\pm$ 0.01 & 7.01 $\pm$ 0.05\\
137 & - & - & - & -& 1.09 $\pm$ 0.02 & 7.16 $\pm$ 0.03\\
138 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.03 $\pm$ 0.02\\
139 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.2 $\pm$ 0.04\\
140 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.29 $\pm$ 0.02\\
141 & - & - & - & -& 1.06 $\pm$ 0.01 & 7.07 $\pm$ 0.06\\
142 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.02 $\pm$ 0.02\\
143 & - & - & - & -& 1.08 $\pm$ 0.01 & 7.06 $\pm$ 0.06\\
144 & - & - & - & -& 1.04 $\pm$ 0.01 & 7.0 $\pm$ 0.06\\
145 & - & - & - & -& 1.08 $\pm$ 0.02 & 6.93 $\pm$ 0.05\\
146 & - & - & - & -& 1.06 $\pm$ 0.01 & 6.8 $\pm$ 0.05\\
147 & - & - & - & -& 1.08 $\pm$ 0.01 & 6.84 $\pm$ 0.02\\
148 & - & - & - & -& 1.1 $\pm$ 0.01 & 6.73 $\pm$ 0.02\\
149 & - & - & - & -& 1.06 $\pm$ 0.01 & 6.77 $\pm$ 0.05\\
150 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.5 $\pm$ 0.05\\
151 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.29 $\pm$ 0.03\\
152 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.39 $\pm$ 0.02\\
153 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.9 $\pm$ 0.05\\
154 & - & - & - & -& 1.04 $\pm$ 0.0 & 7.01 $\pm$ 0.04\\
155 & - & - & - & -& 1.02 $\pm$ 0.0 & 6.98 $\pm$ 0.04\\
156 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.98 $\pm$ 0.04\\
157 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.26 $\pm$ 0.02\\
158 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.32 $\pm$ 0.02\\
159 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.03 $\pm$ 0.03\\
160 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.3 $\pm$ 0.02\\
161 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.3 $\pm$ 0.03\\
162 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.22 $\pm$ 0.04\\
163 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.24 $\pm$ 0.04\\
164 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.24 $\pm$ 0.03\\
165 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.12 $\pm$ 0.03\\
166 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.28 $\pm$ 0.05\\
167 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.17 $\pm$ 0.02\\
168 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.87 $\pm$ 0.05\\
169 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.2 $\pm$ 0.03\\
170 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.24 $\pm$ 0.04\\
171 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.9 $\pm$ 0.04\\
172 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.9 $\pm$ 0.03\\
173 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.36 $\pm$ 0.03\\
174 & - & - & - & -& 1.03 $\pm$ 0.01 & 6.77 $\pm$ 0.07\\
175 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.02 $\pm$ 0.03\\
176 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.21 $\pm$ 0.02\\
177 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.07 $\pm$ 0.04\\
178 & - & - & - & -& 1.03 $\pm$ 0.01 & 7.02 $\pm$ 0.03\\
179 & - & - & - & -& 1.02 $\pm$ 0.0 & 6.92 $\pm$ 0.06\\
180 & - & - & - & -& 1.01 $\pm$ 0.0 & 6.9 $\pm$ 0.06\\
181 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.24 $\pm$ 0.04\\
182 & - & - & - & -& 1.07 $\pm$ 0.01 & 6.61 $\pm$ 0.03\\

 
  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 
 
183 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.62 $\pm$ 0.02\\
184 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.07 $\pm$ 0.04\\
185 & - & - & - & -& 1.08 $\pm$ 0.01 & 7.1 $\pm$ 0.05\\
186 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.65 $\pm$ 0.02\\
187 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.91 $\pm$ 0.06\\
188 & - & - & - & -& 1.01 $\pm$ 0.0 & 6.98 $\pm$ 0.03\\
189 & - & - & - & -& 1.09 $\pm$ 0.02 & 6.74 $\pm$ 0.08\\
190 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.95 $\pm$ 0.06\\
191 & - & - & - & -& 1.07 $\pm$ 0.01 & 7.0 $\pm$ 0.03\\
192 & - & - & - & -& 1.13 $\pm$ 0.02 & 6.53 $\pm$ 0.04\\
193 & - & - & - & -& 1.09 $\pm$ 0.02 & 7.1 $\pm$ 0.05\\
194 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.56 $\pm$ 0.03\\
195 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.09 $\pm$ 0.04\\
196 & - & - & - & -& 1.11 $\pm$ 0.01 & 6.98 $\pm$ 0.05\\
197 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.91 $\pm$ 0.04\\
198 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.86 $\pm$ 0.06\\
199 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.77 $\pm$ 0.03\\
200 & - & - & - & -& 1.07 $\pm$ 0.01 & 7.12 $\pm$ 0.04\\
201 & - & - & - & -& 1.03 $\pm$ 0.02 & 6.45 $\pm$ 0.09\\
202 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.9 $\pm$ 0.07\\
203 & - & - & - & -& 1.07 $\pm$ 0.01 & 7.15 $\pm$ 0.05\\
204 & - & - & - & -& 1.03 $\pm$ 0.01 & 6.75 $\pm$ 0.03\\
205 & - & - & - & -& 1.06 $\pm$ 0.01 & 6.41 $\pm$ 0.04\\
206 & - & - & - & -& 1.16 $\pm$ 0.03 & 6.48 $\pm$ 0.05\\
207 & - & - & - & -& 1.12 $\pm$ 0.02 & 6.34 $\pm$ 0.05\\
208 & - & - & - & -& 1.2 $\pm$ 0.03 & 6.46 $\pm$ 0.04\\
209 & - & - & - & -& 1.24 $\pm$ 0.03 & 6.35 $\pm$ 0.03\\
210 & - & - & - & -& 1.19 $\pm$ 0.03 & 6.35 $\pm$ 0.04\\
211 & - & - & - & -& 1.12 $\pm$ 0.02 & 6.2 $\pm$ 0.02\\
212 & - & - & - & -& 1.1 $\pm$ 0.02 & 6.21 $\pm$ 0.06\\
213 & - & - & - & -& 1.22 $\pm$ 0.05 & 6.19 $\pm$ 0.08\\
214 & - & - & - & -& 1.26 $\pm$ 0.04 & 6.23 $\pm$ 0.05\\
215 & - & - & - & -& 1.1 $\pm$ 0.02 & 6.58 $\pm$ 0.08\\
216 & - & - & - & -& 1.1 $\pm$ 0.02 & 6.53 $\pm$ 0.05\\
217 & - & - & - & -& 1.2 $\pm$ 0.05 & 6.65 $\pm$ 0.05\\
218 & - & - & - & -& 1.23 $\pm$ 0.11 & 6.72 $\pm$ 0.13\\
219 & - & - & - & -& 1.12 $\pm$ 0.03 & 6.28 $\pm$ 0.05\\
220 & - & - & - & -& 1.11 $\pm$ 0.02 & 6.22 $\pm$ 0.03\\
221 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.14 $\pm$ 0.08\\
222 & - & - & - & -& 1.04 $\pm$ 0.02 & 6.92 $\pm$ 0.06\\
223 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.96 $\pm$ 0.06\\
224 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.77 $\pm$ 0.05\\
225 & - & - & - & -& 1.08 $\pm$ 0.03 & 6.6 $\pm$ 0.08\\
226 & - & - & - & -& 1.17 $\pm$ 0.06 & 6.38 $\pm$ 0.09\\
227 & - & - & - & -& 1.09 $\pm$ 0.01 & 6.55 $\pm$ 0.02\\
228 & - & - & - & -& 1.01 $\pm$ 0.0 & 6.95 $\pm$ 0.03\\
229 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.04 $\pm$ 0.01\\
230 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.11 $\pm$ 0.01\\
231 & - & - & - & -& 1.02 $\pm$ 0.0 & 6.51 $\pm$ 0.02\\
233 & - & - & - & -& 1.07 $\pm$ 0.01 & 7.0 $\pm$ 0.01\\
233 & - & - & - & -& 1.67 $\pm$ 0.2 & 6.5 $\pm$ 0.1\\
234 & - & - & - & -& 1.02 $\pm$ 0.01 & 7.12 $\pm$ 0.04\\
235 & - & - & - & -& 1.06 $\pm$ 0.02 & 6.69 $\pm$ 0.04\\
236 & - & - & - & -& 1.04 $\pm$ 0.01 & 7.08 $\pm$ 0.02\\
237 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.59 $\pm$ 0.05\\
238 & - & - & - & -& 1.13 $\pm$ 0.04 & 6.17 $\pm$ 0.05\\
239 & - & - & - & -& 1.24 $\pm$ 0.15 & 6.18 $\pm$ 0.15\\
240 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.52 $\pm$ 0.07\\
241 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.14 $\pm$ 0.04\\
242 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.18 $\pm$ 0.03\\
243 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.09 $\pm$ 0.04\\

  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 
 
 
244 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.2 $\pm$ 0.03\\
245 & - & - & - & -& 1.01 $\pm$ 0.0 & 7.34 $\pm$ 0.02\\
246 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.22 $\pm$ 0.04\\
247 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.23 $\pm$ 0.03\\
248 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.03 $\pm$ 0.03\\
249 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.02 $\pm$ 0.06\\
250 & - & - & - & -& 1.02 $\pm$ 0.0 & 7.13 $\pm$ 0.04\\
251 & - & - & - & -& 1.05 $\pm$ 0.0 & 7.07 $\pm$ 0.08\\
252 & - & - & - & -& 1.04 $\pm$ 0.0 & 6.96 $\pm$ 0.08\\
253 & - & - & - & -& 1.03 $\pm$ 0.0 & 6.87 $\pm$ 0.04\\
254 & - & - & - & -& 1.04 $\pm$ 0.01 & 6.97 $\pm$ 0.03\\
255 & - & - & - & -& 1.08 $\pm$ 0.0 & 6.81 $\pm$ 0.05\\
257 & - & - & - & -& 1.53 $\pm$ 0.08 & 5.43 $\pm$ 0.05\\ 
258 & - & - & - & -& 1.38 $\pm$ 0.06 & 5.7 $\pm$ 0.04\\ 
259 & - & - & - & -& 1.26 $\pm$ 0.08 & 5.95 $\pm$ 0.09\\ 
260 & - & - & - & -& 1.26 $\pm$ 0.03 & 6.37 $\pm$ 0.05\\ 
261 & - & - & - & -& 1.3 $\pm$ 0.06 & 6.09 $\pm$ 0.07\\ 
262 & - & - & - & -& 1.34 $\pm$ 0.06 & 6.27 $\pm$ 0.07\\ 
263 & - & - & - & -& 2.03 $\pm$ 0.18 & 6.37 $\pm$ 0.08\\ 
264 & - & - & - & -& 1.37 $\pm$ 0.07 & 6.12 $\pm$ 0.08\\ 
265 & - & - & - & -& 1.51 $\pm$ 0.06 & 6.02 $\pm$ 0.06\\ 
266 & - & - & - & -& 1.35 $\pm$ 0.06 & 6.16 $\pm$ 0.07\\ 
267 & - & - & - & -& 1.14 $\pm$ 0.02 & 6.18 $\pm$ 0.06\\ 
268 & - & - & - & -& 1.76 $\pm$ 0.09 & 6.02 $\pm$ 0.05\\ 
269 & - & - & - & -& 1.34 $\pm$ 0.05 & 6.19 $\pm$ 0.07\\ 
270 & - & - & - & -& 1.39 $\pm$ 0.06 & 6.12 $\pm$ 0.06\\ 
271 & 5.54 $\pm$ 0.03 & 4.96 $\pm$ 0.08 & 0.48 $\pm$ 0.09 & 1.27 $\pm$ 0.1 & 1.38 $\pm$ 0.04 & 6.25 $\pm$ 0.06\\ 
272 & 5.49 $\pm$ 0.04 & 4.94 $\pm$ 0.08 & 0.46 $\pm$ 0.1 & 1.26 $\pm$ 0.14 & 1.35 $\pm$ 0.04 & 6.22 $\pm$ 0.07\\ 
273 & 5.65 $\pm$ 0.03 & 4.92 $\pm$ 0.08 & 0.61 $\pm$ 0.1 & 1.2 $\pm$ 0.1 & 1.24 $\pm$ 0.03 & 6.41 $\pm$ 0.07\\ 
274 & 5.95 $\pm$ 0.05 & 5.17 $\pm$ 0.04 & 0.65 $\pm$ 0.08 & 1.2 $\pm$ 0.07 & 1.2 $\pm$ 0.05 & 6.66 $\pm$ 0.07\\ 
275 & 5.92 $\pm$ 0.04 & 5.51 $\pm$ 0.04 & 0.33 $\pm$ 0.07 & 1.41 $\pm$ 0.1 & 1.2 $\pm$ 0.04 & 6.68 $\pm$ 0.07\\ 
276 & 5.89 $\pm$ 0.05 & 4.74 $\pm$ 0.1 & 0.97 $\pm$ 0.13 & 1.09 $\pm$ 0.08 & 1.15 $\pm$ 0.04 & 6.57 $\pm$ 0.07\\ 
277 & 5.8 $\pm$ 0.08 & - & - & -& 1.15 $\pm$ 0.04 & 6.61 $\pm$ 0.07\\ 
278 & - & - & - & -& 1.27 $\pm$ 0.03 & 6.73 $\pm$ 0.04\\ 
279 & - & - & - & -& 1.33 $\pm$ 0.04 & 6.33 $\pm$ 0.04\\ 
280 & - & - & - & -& 1.23 $\pm$ 0.03 & 6.47 $\pm$ 0.04\\ 
281 & 5.49 $\pm$ 0.04 & 4.13 $\pm$ 0.37 & 0.28 $\pm$ 0.08 & 1.44 $\pm$ 0.13 & 1.45 $\pm$ 0.05 & 6.29 $\pm$ 0.06\\ 
282 & - & - & - & -& 1.15 $\pm$ 0.02 & 6.74 $\pm$ 0.03\\
283 & 5.57 $\pm$ 0.04 & 5.04 $\pm$ 0.12 & 0.43 $\pm$ 0.13 & 1.33 $\pm$ 0.13 & 1.33 $\pm$ 0.04 & 6.36 $\pm$ 0.06\\ 
284 & 5.75 $\pm$ 0.04 & 4.84 $\pm$ 0.1 & 0.77 $\pm$ 0.12 & 1.15 $\pm$ 0.07 & 1.17 $\pm$ 0.02 & 6.51 $\pm$ 0.05\\ 
285 & 4.96 $\pm$ 0.02 & 4.66 $\pm$ 0.02 & 0.24 $\pm$ 0.03 & 1.53 $\pm$ 0.05 & 1.52 $\pm$ 0.06 & 5.85 $\pm$ 0.04\\ 
286 & 4.54 $\pm$ 0.04 & 4.76 $\pm$ 0.02 & -0.21 $\pm$ 0.05 & 2.44 $\pm$ 0.23 & 1.96 $\pm$ 0.14 & 5.56 $\pm$ 0.08\\ 
287 & - & - & - & -& 2.39 $\pm$ 0.16 & 5.41 $\pm$ 0.04\\
288 & 5.57 $\pm$ 0.03 & 5.04 $\pm$ 0.06 & 0.43 $\pm$ 0.08 & 1.32 $\pm$ 0.08 & 1.3 $\pm$ 0.05 & 6.3 $\pm$ 0.05\\ 
289 & - & - & - & -& 1.67 $\pm$ 0.22 & 5.97 $\pm$ 0.09\\ 
290 & - & - & - & -& 1.13 $\pm$ 0.02 & 6.6 $\pm$ 0.03\\ 
291 & - & - & - & -& 1.45 $\pm$ 0.04 & 5.85 $\pm$ 0.03\\ 
292 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.17 $\pm$ 0.01\\ 
293 & - & - & - & -& 1.03 $\pm$ 0.0 & 7.1 $\pm$ 0.02\\
294 & 6.1 $\pm$ 0.01 & 5.06 $\pm$ 0.02 & 0.87 $\pm$ 0.03 & 1.12 $\pm$ 0.02 & 1.22 $\pm$ 0.02 & 6.83 $\pm$ 0.02\\ 
295 & - & - & - & -& 1.06 $\pm$ 0.0 & 6.99 $\pm$ 0.01\\
296 & 5.36 $\pm$ 0.01 & 5.16 $\pm$ 0.01 & 0.15 $\pm$ 0.02 & 1.62 $\pm$ 0.04 & 1.53 $\pm$ 0.04 & 6.27 $\pm$ 0.02\\ 
297 & 4.59 $\pm$ 0.02 & 5.02 $\pm$ 0.02 & -0.4 $\pm$ 0.03 & 3.15 $\pm$ 0.19 & 2.51 $\pm$ 0.17 & 5.58 $\pm$ 0.05\\ 
298 & 5.56 $\pm$ 0.01 & 5.12 $\pm$ 0.01 & 0.36 $\pm$ 0.02 & 1.39 $\pm$ 0.03 & 1.35 $\pm$ 0.03 & 6.33 $\pm$ 0.02\\ 
299 & 5.86 $\pm$ 0.01 & 5.38 $\pm$ 0.01 & 0.39 $\pm$ 0.02 & 1.37 $\pm$ 0.02 & 1.24 $\pm$ 0.02 & 6.55 $\pm$ 0.02\\ 
300 & 5.87 $\pm$ 0.01 & 4.78 $\pm$ 0.02 & 0.92 $\pm$ 0.03 & 1.1 $\pm$ 0.02 & 1.19 $\pm$ 0.01 & 6.53 $\pm$ 0.02\\ 
301 & 5.87 $\pm$ 0.01 & - & - & -& 1.12 $\pm$ 0.01 & 6.53 $\pm$ 0.02\\ 
302 & 5.83 $\pm$ 0.01 & 5.25 $\pm$ 0.02 & 0.48 $\pm$ 0.02 & 1.3 $\pm$ 0.02 & 1.21 $\pm$ 0.02 & 6.51 $\pm$ 0.02\\ 
303 & 5.98 $\pm$ 0.01 & 4.82 $\pm$ 0.02 & 0.98 $\pm$ 0.03 & 1.09 $\pm$ 0.01 & 1.13 $\pm$ 0.01 & 6.69 $\pm$ 0.02\\ 
304 & - & - & - & -& 1.09 $\pm$ 0.01 & 7.35 $\pm$ 0.02\\ 
305 & - & - & - & -& 1.55 $\pm$ 0.04 & 6.03 $\pm$ 0.02\\ 


  \end{tabular}
\end{table*}

\begin{table*}
\centering
\contcaption{}
\begin{tabular}{ccccccc}
\hline
ID & 12+log(Ar$^{++}$/H$^{+}$)&	12+log(Ar$^{3+}$/H$^{+}$) & log(S$^{3+}$/S$^{++}$) & ICF(Ar) & ICF($\eta$')& 12+log(S/H)
\\ \hline 
 


306 & - & - & - & -& 1.38 $\pm$ 0.02 & 6.21 $\pm$ 0.02\\ 
307 & 5.56 $\pm$ 0.01 & 4.95 $\pm$ 0.02 & 0.51 $\pm$ 0.03 & 1.25 $\pm$ 0.03 & 1.19 $\pm$ 0.01 & 6.33 $\pm$ 0.02\\ 
308 & 5.44 $\pm$ 0.01 & 4.7 $\pm$ 0.02 & 0.61 $\pm$ 0.03 & 1.2 $\pm$ 0.03 & 1.33 $\pm$ 0.02 & 6.3 $\pm$ 0.02\\ 
309 & 5.47 $\pm$ 0.01 & 4.91 $\pm$ 0.02 & 0.46 $\pm$ 0.03 & 1.29 $\pm$ 0.03 & 1.36 $\pm$ 0.03 & 6.28 $\pm$ 0.02\\ 
310 & 5.85 $\pm$ 0.01 & 4.68 $\pm$ 0.02 & 0.99 $\pm$ 0.03 & 1.1 $\pm$ 0.01 & 1.14 $\pm$ 0.01 & 6.57 $\pm$ 0.01\\ 
311 & 5.22 $\pm$ 0.05 & 4.96 $\pm$ 0.05 & 0.19 $\pm$ 0.09 & 1.57 $\pm$ 0.16 & 1.52 $\pm$ 0.09 & 6.13 $\pm$ 0.08\\ 
312 & - & - & - & -& 1.5 $\pm$ 0.05 & 6.5 $\pm$ 0.03\\
313 & 5.31 $\pm$ 0.05 & 5.3 $\pm$ 0.05 & -0.01 $\pm$ 0.08 & 1.94 $\pm$ 0.22 & 1.73 $\pm$ 0.12 & 6.15 $\pm$ 0.08\\ 
314 & - & - & - & -& 1.27 $\pm$ 0.03 & 6.46 $\pm$ 0.05\\
315 & 5.59 $\pm$ 0.02 & 5.18 $\pm$ 0.07 & 0.33 $\pm$ 0.08 & 1.42 $\pm$ 0.09 & 1.58 $\pm$ 0.08 & 6.22 $\pm$ 0.04\\ 
316 & 5.92 $\pm$ 0.01 & 4.77 $\pm$ 0.05 & 0.96 $\pm$ 0.05 & 1.09 $\pm$ 0.03 & 1.1 $\pm$ 0.01 & 6.74 $\pm$ 0.02\\ 
317 & - & - & - & -& 1.1 $\pm$ 0.01 & 6.96 $\pm$ 0.04\\ 
318 & 5.62 $\pm$ 0.02 & 4.96 $\pm$ 0.05 & 0.54 $\pm$ 0.06 & 1.25 $\pm$ 0.06 & 1.24 $\pm$ 0.02 & 6.5 $\pm$ 0.03\\ 
319 & - & - & - & -& 1.58 $\pm$ 0.09 & 6.22 $\pm$ 0.07\\
320 & 5.31 $\pm$ 0.03 & 4.92 $\pm$ 0.06 & 0.31 $\pm$ 0.08 & 1.39 $\pm$ 0.12 & 1.7 $\pm$ 0.07 & 6.0 $\pm$ 0.06\\ 
321 & 5.21 $\pm$ 0.02 & 4.98 $\pm$ 0.08 & 0.17 $\pm$ 0.09 & 1.54 $\pm$ 0.17 & 1.67 $\pm$ 0.07 & 6.02 $\pm$ 0.06\\ 
322 & - & - & - & -& 1.16 $\pm$ 0.02 & 6.3 $\pm$ 0.04\\ 
323 & - & - & - & -& 1.12 $\pm$ 0.01 & 6.31 $\pm$ 0.04\\ 
324 & - & - & - & -& 1.38 $\pm$ 0.04 & 6.05 $\pm$ 0.03\\ 
325 & 5.34 $\pm$ 0.05 & 5.14 $\pm$ 0.06 & 0.15 $\pm$ 0.09 & 1.63 $\pm$ 0.18 & 1.62 $\pm$ 0.08 & 6.25 $\pm$ 0.08\\ 
70 & - & - & - & -& 1.55 $\pm$ 0.07 & 5.81 $\pm$ 0.06\\
327 & 5.51 $\pm$ 0.03 & 5.05 $\pm$ 0.03 & 0.37 $\pm$ 0.06 & 1.38 $\pm$ 0.08 & 1.37 $\pm$ 0.08 & 6.23 $\pm$ 0.06\\ 
328 & 5.57 $\pm$ 0.05 & 5.01 $\pm$ 0.04 & 0.46 $\pm$ 0.08 & 1.29 $\pm$ 0.11 & 1.36 $\pm$ 0.09 & 6.34 $\pm$ 0.07\\ 
73 & 5.79 $\pm$ 0.05 & 4.94 $\pm$ 0.05 & 0.71 $\pm$ 0.09 & 1.16 $\pm$ 0.1 & 1.26 $\pm$ 0.08 & 6.5 $\pm$ 0.08\\ 
330 & 5.5 $\pm$ 0.05 & 5.05 $\pm$ 0.05 & 0.36 $\pm$ 0.08 & 1.33 $\pm$ 0.15 & 1.64 $\pm$ 0.17 & 6.18 $\pm$ 0.08\\ 
75 & 5.38 $\pm$ 0.04 & 5.17 $\pm$ 0.04 & 0.15 $\pm$ 0.07 & 1.61 $\pm$ 0.15 & 1.5 $\pm$ 0.12 & 6.21 $\pm$ 0.08\\ 
76 & 5.6 $\pm$ 0.05 & 5.12 $\pm$ 0.05 & 0.39 $\pm$ 0.08 & 1.36 $\pm$ 0.11 & 1.47 $\pm$ 0.12 & 6.35 $\pm$ 0.07\\ 
77 & 5.79 $\pm$ 0.06 & 6.0 $\pm$ 0.02 & -0.21 $\pm$ 0.07 & 2.25 $\pm$ 0.36 & 1.31 $\pm$ 0.07 & 6.88 $\pm$ 0.11\\ 
334 & 6.07 $\pm$ 0.04 & - & - & -& 1.04 $\pm$ 0.01 & 6.99 $\pm$ 0.02\\ 
79 & 5.65 $\pm$ 0.05 & 4.73 $\pm$ 0.04 & 0.77 $\pm$ 0.08 & 1.03 $\pm$ 0.04 & 1.22 $\pm$ 0.06 & 6.13 $\pm$ 0.06\\ 
336 & - & - & - & -& 1.18 $\pm$ 0.04 & 6.5 $\pm$ 0.05\\ 
337 & - & - & - & -& 1.1 $\pm$ 0.02 & 6.76 $\pm$ 0.05\\ 
338 & - & - & - & -& 1.07 $\pm$ 0.02 & 6.71 $\pm$ 0.04\\ 
339 & - & - & - & -& 1.22 $\pm$ 0.05 & 6.65 $\pm$ 0.06\\ 
340 & - & - & - & -& 1.06 $\pm$ 0.01 & 7.0 $\pm$ 0.04\\ 
341 & - & - & - & -& 1.19 $\pm$ 0.04 & 6.34 $\pm$ 0.05\\ 
342 & 5.4 $\pm$ 0.04 & 4.75 $\pm$ 0.1 & 0.53 $\pm$ 0.12 & 1.21 $\pm$ 0.16 & 1.4 $\pm$ 0.08 & 6.25 $\pm$ 0.09\\ 
343 & - & - & - & -& 1.09 $\pm$ 0.02 & 6.85 $\pm$ 0.05\\ 
344 & - & - & - & -& 1.05 $\pm$ 0.01 & 6.81 $\pm$ 0.06\\ 
345 & 4.66 $\pm$ 0.03 & 5.23 $\pm$ 0.03 & -0.51 $\pm$ 0.05 & 3.88 $\pm$ 0.42 & 4.05 $\pm$ 0.55 & 5.79 $\pm$ 0.07\\ 
346 & 4.85 $\pm$ 0.03 & 5.12 $\pm$ 0.03 & -0.26 $\pm$ 0.05 & 2.6 $\pm$ 0.22 & 2.9 $\pm$ 0.3 & 5.8 $\pm$ 0.06\\ 
347 & 4.36 $\pm$ 0.03 & 4.84 $\pm$ 0.03 & -0.43 $\pm$ 0.06 & 3.32 $\pm$ 0.37 & 3.23 $\pm$ 0.38 & 5.54 $\pm$ 0.07\\ 
348 & 4.31 $\pm$ 0.06 & 4.4 $\pm$ 0.08 & -0.11 $\pm$ 0.12 & 2.09 $\pm$ 0.4 & 1.78 $\pm$ 0.15 & 5.32 $\pm$ 0.13\\ 
349 & 6.0 $\pm$ 0.07 & 5.12 $\pm$ 0.18 & 0.74 $\pm$ 0.22 & 1.15 $\pm$ 0.17 & 1.23 $\pm$ 0.04 & 6.89 $\pm$ 0.1\\ 
350 & 5.69 $\pm$ 0.03 & 5.04 $\pm$ 0.11 & 0.54 $\pm$ 0.12 & 1.23 $\pm$ 0.11 & 1.31 $\pm$ 0.05 & 6.52 $\pm$ 0.05\\ 
351 & - & - & - & -& 1.24 $\pm$ 0.01 & 6.6 $\pm$ 0.03\\ 
352 & 5.65 $\pm$ 0.01 & 5.06 $\pm$ 0.04 & 0.49 $\pm$ 0.05 & 1.28 $\pm$ 0.05 & 1.58 $\pm$ 0.04 & 6.38 $\pm$ 0.02\\




 

 

 









 
 

 
 
 



\hline
\end{tabular}

\end{table*}
\newpage
